Faster or Slower? Performance Mystery of Python Idioms Unveiled with Empirical Evidence

The usage of Python idioms is popular among Python developers in a formative study of 101 performance-related questions of Python idioms on Stack Overflow, we find that developers often get confused about the performance impact of Python idioms and use anecdotal toy code or rely on personal project experience which is often contradictory in performance outcomes. There has been no large-scale, systematic empirical evidence to reconcile these performance debates. In the paper, we create a large synthetic dataset with 24,126 pairs of non-idiomatic and functionally-equivalent idiomatic code for the nine unique Python idioms identified in Zhang et al., and reuse a large real-project dataset of 54,879 such code pairs provided by Zhang et al. We develop a reliable performance measurement method to compare the speedup or slowdown by idiomatic code against non-idiomatic counterpart, and analyze the performance discrepancies between the synthetic and real-project code, the relationships between code features and performance changes, and the root causes of performance changes at the bytecode level. We summarize our findings as some actionable suggestions for using Python idioms.

==> motiv.tex <==


%Python developers usually use Python idioms to write code because of the conciseness and performance~\cite{}. Although previous studies or online resources~\cite{} stated that the Python idioms may speed up the programs, we find there is no quantitative analysis study on performance of Python idioms, and there are arguments about the performance of Python idioms on StackOverflow. Based on the previous studies~\cite{}, we focus on nine Python idioms: list comprehension, set comprehension, dictionary comprehension, chain comparison, truth value test, loop else, assignment multiple targets, star in function calls and for multiple targets. 

To understand the opinions and arguments on the performance of Python idioms, we examine Stack Overflow questions for the nine Python idioms identified by Zhang et al.~\cite{zhang2022making}. 
We search python-tagged questions for each python idiom with the idiom name and performance-related keywords such as ``slow'', ``fast'', ``performance'', ``speed'' or ``time'' by using Stack Overflow search interface~\cite{stack_overflow}. 
For each idiom, we check the returned top-30 questions and finally collect 101 questions that discuss the performance of these nine Python idioms. Table~\ref{tab:motivation_soposts} shows some representative examples. 
\#N represents the number of questions we find for each Python idiom and blue text represents the view times that more than 1k times indicates the questions are popular.
Our key findings are: Python developers are concerned with the performance of Python idioms. 
However, their evidences of performance improvement or regression are generally anecdotal based on either toy code or individual project experience. 
This leads to many controversies about if and when developers should or should not use Python idioms.
\zejun{Detailed discussions with examples can be found in our \href{https://anonymous.4open.science/r/PerformanceMysteryPythonIdioms-315B/performance_python_idioms_supplementary_document.pdf}{supplementary document} (see in APPENDIX A).}
%Finallysummarize the interests and confusions about the performance of Python idioms. There are  

\zc{Put the following content in the supplementary document. Use the same section heading consistently in the supplementary document so the reader can easily link the content there to the main paper. Other content should put in the supplementary doc: 1) Fig. 2 with the explanation for set/dict comprehension. 2) Non-idiomatic and idiomatic code pairs like Fig. 3 with the explanation for the code differences. 3) Complete dataset summary for each number.}
\textbf{(1) Developers are concerned with the performance of Python idioms.} First, developers ask whether idiomatic code is faster or slower than non-idiomatic code. For example, for the star-in-func-call in Table~\ref{tab:motivation_soposts}, developers are interested in whether the  star operator affects the performance. Furthermore, developers would like to know how many times idiomatic code may be faster or slower than the non-idiomatic code. For example, for the list-comprehension in Table~\ref{tab:motivation_soposts}, a developer states that the list comprehension is 50\% faster than appending to a list with for loop. Finally, developers want to know the reasons why Python idioms causes the performance change. For example, for the for-multiple-targets in Table~\ref{tab:motivation_soposts}, a developer ask why accessing by index slow things down compared to for-multiple-targets.%there is no a large-scale code pairs of idiomatic code and non-idiomatic code and quantitative study to support  analysis  propose  are ver Python developers usually use Python idioms to write  are highly valued by Python developersPrevious researchers Python Compared with other mainstream programming languages, Python developers

\textbf{(2) Many questions lack clear evidence of the performance impact of Python idioms.} Only 49.5\% questions list code fragments and corresponding execution time to illustrate the performance of Python idioms. For example, for the chain-comparison in Table~\ref{tab:motivation_soposts}, developers write a toy code pair of \textsf{x<y<z} and \textsf{x<y and y<z} to compare their execution time. Furthermore, for the two questions regarding loop-else and star-in-func-call, they lack code fragments or execution time, but provide only natural language descriptions for the performance of the idioms. 
For example, for the loop-else in Table~\ref{tab:motivation_soposts}, a developer say ``I was introduced to a wonderful idiom in which you can use a for/break/else scheme with an iterator to save both time and lines of code''.%%And 即使是toy code他们也意见不一致

%%人们对性能的探索还很有限，有很多还有争议，甚至还是空白。
\textbf{(3) Developers are often confused by the controversial descriptions or evidences of the performance of Python idioms.} 
33 out of 101 question threads present some contradictory performance results.
Among the nine examples in Table~\ref{tab:motivation_soposts}, six questions discuss the contradictory performance results, annotated with a *.
%\zc{The questions for the six Python idioms in Table~\ref{tab:motivation_soposts} demonstrate the contradictory performance results. ??among 110 \zejun{33 among 101}or just the examples in Table II? If in Table II, annotate these six by *?} \zejun{Among nine Python idioms, questions of six Python idioms demonstrate the contradictory performance result, where the percentage is about 32.7\%. We annotate these six by * in Table~\ref{tab:motivation_soposts}}
For example, for the assign-multi-targets in Table~\ref{tab:motivation_soposts}, a developer states that multiple assignment perform at least 30\% better than the individual assignment. However, the developer shows that the \href{https://wiki.python.org/moin/PythonSpeed}{Python official wiki} states that multiple assignment is slower than of individual assignment. 
Similarly, for the chain-comparison in Table~\ref{tab:motivation_soposts}, a developer finds the chain comparison is slower, but another developer states that the \href{https://wiki.python.org/moin/PythonSpeed}{Python official wiki} claims that chained comparisons are faster than using ``and'' operator.
As another example, for the truth-value-test in Table~\ref{tab:motivation_soposts}, it is generally understood that this idiom does not impact the performance largely. However, the developer encounter a scenario that the truth-value-test can shave 30\% off runtime.
%in the developer surprisingly 
%finds that the truth-value-test make her code almost 6 times faster.  
%\zc{do we have an example where idiom in toy code is faster but slower in real project? if so, discuss this example here ...}
%https://stackoverflow.com/questions/53513/how-do-i-check-if-a-list-is-empty/45778282#45778282 maybe  if xpath\_results == [] 

\vspace{0.1cm}
\noindent\fcolorbox{red}{white}{\begin{minipage}{8.6cm} \emph{Python developers are concerned with the performance of Python idioms. 
However, their evidences of performance improvement or regression are generally anecdotal based on either toy code or individual project experience. 
This leads to many controversies about if and when developers should or should not use Python idioms.} \end{minipage}}

%\noindent\textbf{Summary:}


%For another example, for the truth-value-test, the developer is shock that the Python idioms could improve performance by more than 5 times (5th-to-last row in Table~\ref{tab:motivation_soposts}).
\begin{table}[tbp]
\vspace{-0.1cm}
\scriptsize\caption{Python Idiom Performance Related SO Questions }%\zc{add question view counts. 2) If the content is from question body, indent the content. 3) Truth-value-test seems no need the code snippet? 4) Anything to highlight for the loop-else and star-in-func-call examples? 5) For for-multi-targets, no content to quote? If not, please highlight the key information in the question title.}
  \label{tab:motivation_soposts}
  \vspace{-0.3cm}
\centering
\begin{tabular}{|p{0.7cm}<{\centering}|p{0.10cm}<{\centering}|p{2.66in}|} 
\hline
Idiom          &\#N& Question \\ 
\hline
%https://stackoverflow.com/questions/31343643/why-list-comprehension-can-be-faster-than-map-in-python 用这个
%https://stackoverflow.com/questions/51105841/faster-python-list-comprehension
\begin{tabular}[c]{@{}l@{}}List-\\Compre\\hension*\end{tabular}      & 26    &\begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/19273256/how-to-speed-up-list-comprehension}{\textbf{Question: }}How to speed up list comprehension?\\
\ \ my understanding is that \textcolor{red}{for-loop is faster than} \textcolor{red}{list comprehension}.
\\\textbf{Comments: }
In all cases I've measured the time \textcolor{red}{a list  comp}\\\textcolor{red}{rehension was always faster than a standard for loop}. (\textcolor{blue}{2k times}) 
%\\table = ''\\for index in xrange(256):\\ \hspace{0.075cm} if index in ords\_to\_keep:\\ \hspace{0.15cm} table += chr(index)\\ \hspace{0.075cm} else:\\ \hspace{0.15cm} table += replace\_with\\
           \end{tabular}  \\ 
\hline
% \begin{tabular}[c]{@{}l@{}}set-com\\prehensi\\on*\end{tabular}       & 12    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/53720541/set-comprehension-vs-for-loop-vs-set-difference}{\textbf{Question: }}Set comprehension VS. For Loop VS .... \\\ \ Which one of the following do you think would faster?\\
% \textbf{Comments: }I did, but \textcolor{red}{results are quite unstable}. I'd like to know \\which one of them is really faster from a design point.
% \end{tabular}  \\ 

\begin{tabular}[c]{@{}l@{}}Set-\\Compre\\hension*\end{tabular}       & 12    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/20496536/how-do-python-set-comprehensions-work/20497109#20497109}{\textbf{Question: }}How do python Set Comprehensions work?\\ \ \ I tried timeit for speed comparisons, there is quite some difference.\\
\textbf{Answer: } List/Dict/Set comprehensions tend to be faster than\\ anything else. (\textcolor{blue}{2k times}) 
\end{tabular}  \\ 
% \begin{tabular}[c]{@{}l@{}}Set Com-\\prehension\end{tabular}       & (3)    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/38558834/use-list-set-comprehension-merely-as-a-for-loop}{\fbox{\textbf{Question: }}}Use set comprehension merely as a "for" loop?\\
% record\_key\_list = \{(choice(tuple(studentID\_list)), ...,\\
%                   choice(grades)[0]) 
%                   for no\_use in range(NUM\_RECORDS)\}\\
% I timed the two code snippets and \textbf{they are roughly the} \\\textbf{same as} fast for 20000 records.
% \end{tabular}            \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Dict-\\Compre\\hension*\end{tabular}      & \begin{tabular}[c]{@{}l@{}}15\end{tabular}   & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/52542742/why-is-this-loop-faster-than-a-dictionary-comprehension-for-creating-a-dictionar/52542927#52542927}{\textbf{Question: }}Why is \textcolor{red}{this loop faster than a dictionary} \textcolor{red}{comprehension}?\\
% \texttt{a = \{'a':'hi','b':'hey','c':'yo'\}}\\
% \texttt{b = \{v: k for k, v in a.items()\}}\\
\textbf{Comment:} ... I do this with a dictionary with 1000 random keys \\and values, \textcolor{red}{the dictcomp is marginally slightly} \textcolor{red}{faster}. (\textcolor{blue}{9k times}) 
\end{tabular}            \\ 
\hline
% \begin{tabular}[c]{@{}l@{}}chain-co\\mpare*\end{tabular}        & \begin{tabular}[c]{@{}l@{}}6 \end{tabular}    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/48375753/why-are-chained-operator-expressions-slower-than-their-expanded-equivalent}{\textbf{Question: }}Why are \textcolor{red}{chained operator expressions slower}\\ \textcolor{red}{than their expanded equivalent}?\\\textbf{Answer: }In \href{https://wiki.python.org/moin/PythonSpeed}{Python wiki page}, it states that \textcolor{red}{chained}\\ \textcolor{red}{comparisons are faster than using the "and" operator}.
% \end{tabular}    \\ 
% \hline
\begin{tabular}[c]{@{}l@{}}Chain-\\Compa\\rison*\end{tabular}        & \begin{tabular}[c]{@{}l@{}}6 \end{tabular}    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/34014906/is-x-y-z-faster-than-x-y-and-y-z?noredirect=1&lq=1}{\textbf{Question: }}Is "x < y < z" \textcolor{red}{faster than} "x < y and y < z"?\\
\ \ \href{https://wiki.python.org/moin/PythonSpeed}{In this page}, we know that chained comparisons are \textcolor{red}{faster than} u-\\sing the "and" operator. However, I got \textcolor{red}{a different result}... It seems \\that \texttt{x < y} and \texttt{y < z} is faster than \texttt{x < y < z}. (\textcolor{blue}{11k times})
\end{tabular}    \\ 
\hline
% \begin{tabular}[c]{@{}l@{}}truth-\\value-\\-test* \end{tabular}       & 17    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/67747896/why-is-if-x-significantly-faster-than-if-x0-conways-game-of-life/67748136#67748136}{\textbf{Question: }}why is ``if x:'' significantly faster than ``if x>0''?\\
% \ \ ... how this one change made the function almost 6 times faster. \\I am both very confused and \textcolor{red}{surprised how this one small change}\\ \textcolor{red}{made such a difference}.\end{tabular} \\
% \hline

\begin{tabular}[c]{@{}l@{}}Truth-\\Value-\\Test* \end{tabular}       & 17    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/9850245/bool-value-of-a-list-in-python}{\textbf{Question: }}bool value of a list in Python.\\
\textbf{Answer:} \textcolor{red}{99.9\%} of the time, \textcolor{red}{performance doesn't matter} as suggest-\\ed Keith. I only mention this because I once had a scenario, using \\implicit truthiness testing \textcolor{red}{shaved 30\% off the runtime}. (\textcolor{blue}{31k times})\end{tabular} \\
\hline

\begin{tabular}[c]{@{}l@{}}Loop-\\Else\end{tabular}               & 7    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/685758/pythonic-ways-to-use-else-in-a-for-loop}{\textbf{Question: }}Pythonic ways to use 'else' in a for loop.\\
\textbf{Answer:} I was introduced to a wonderful idiom in which you can \\use a for/break/else scheme with an iterator to \textcolor{red}{save both time} and\\ LOC. (\textcolor{blue}{1k times})\end{tabular}             \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Assign-\\Multi-\\Targets*\end{tabular}    & \begin{tabular}[c]{@{}l@{}}8\end{tabular}    & \begin{tabular}[c]{@{}l@{}}
\href{https://stackoverflow.com/questions/22278695/python-multiple-assignment-vs-individual-assignment-speed}{\textbf{Question: }}Python assigning two variables on one line\\
\ \ I've been looking to squeeze a little more performance out of my \\code; While browsing this \href{https://wiki.python.org/moin/PythonSpeed}{Python wiki page}, I found this claim:\\
\textcolor{red}{Multiple assignment is slower than individual assignment}.\\
I repeated several times, \textcolor{red}{but the multiple assignment snippet} \textcolor{red}{perfor-\\med at least 30\% better than the individual assignment}. (\textcolor{blue}{3k times}) 
% \href{https://stackoverflow.com/questions/44517911/swapping-variables-in-python3}{\fbox{\textbf{Question: }}}I have just started learning python3. How is this line\\ a,b = b,a working?... can I do the same for 3 or more variables in one line?\\
% Asked 4 years; Active 4 years; Viewed 8k times
\end{tabular}     \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Star-in-\\Fun-Call\end{tabular} & \begin{tabular}[c]{@{}l@{}}5\end{tabular}    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/2921847/what-does-the-star-and-doublestar-operator-mean-in-a-function-call}{\textbf{Question: }}What does the star mean in a function call?\\
\ \ Does it \textcolor{red}{affect performance} at all? Is it \textcolor{red}{fast} or \textcolor{red}{slow}? (\textcolor{blue}{245k times})
\end{tabular}          \\ 
\hline
\begin{tabular}[c]{@{}l@{}}For-Mul\\-Targets\end{tabular}       & 5    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/13024416/how-come-unpacking-is-faster-than-accessing-by-index}{\textbf{\textbf{Question: }}}How come unpacking is \textcolor{red}{faster than} accessing by \\index? (\textcolor{blue}{3k times})
\end{tabular}            \\
\hline
\end{tabular}
\vspace{-0.4cm}
\end{table}
%应该可能会加些东西，给出人们对于performance of python idioms的误区和困惑，在implications给出answer
% 1. 人们对于Python idioms的性能很感兴趣经常提出一些问题，views很多 经常询问快还是慢，进一步知道快多少， 满多少 
%2 人们到底快还是慢faster slower 3. 人们希望知道快多少，满多少
% 

% 3. 人们验证性能的时候，经常使用toy code. 人们有一种信念觉得Python idioms一定会快或者慢， 但在实际数据中发现性能的提升并不理想

% 4. 人们在实际代码中发现性能提升并不如人意。1. 不知道idioms哪些方面影响着性能，



==> motiv_old.tex <==
Python developers usually use Python idioms to write code because of the conciseness and performance~\cite{}. Although previous studies or online resources~\cite{} stated that the Python idioms may speed up the programs, we find there are many arguments about the performance of Python idioms on StackOverflow. Based on the previous studies~\cite{}, we focus on nine Python idioms: list comprehension, set comprehension, dictionary comprehension, chain comparison, truth value test, loop else, assignment multiple targets, star in function calls and for multiple targets. To understand the opinions of Python developers on the performance of Python idioms, we examine Stack Overflow questions for the nine Python idioms. We search the python-tagged questions for each python idiom by using the pythonic idiom name and performance-related keywords such as ``slow'', ``fast'' or ``performance''. We check the returned top-30 questions and summarize the interests and confusions about the performance of Python idioms. Table~\ref{tab:motivation_soposts} shows some representative examples.

\textbf{(1) Developers are interested in the performance change of Python idioms.} First, developers usually ask whether idiomatic code is faster/slower than non-idiomatic code. For example, in the 2nd-to-last row in Table~\ref{tab:motivation_soposts}, developers are interested in whether the  star-in-func-call is fast or slow. Furthermore, developers would like to know how many times idiomatic code faster/slower than the non-idiomatic code. For example, in the 3rd-to-last row in Table~\ref{tab:motivation_soposts}, the developers find that assign-multiple-targets perform at least 30\% better than the individual assignment. However, the Python official wiki states that multiple assignment is slower than of individual assignment. Finally, developers desire to know the reasons why Python idioms causes the performance change. For example, in the 5th row in Table~\ref{tab:motivation_soposts}, developers would like to know why the chain-comparison is slower than the equivalent non-idiomatic code. %there is no a large-scale code pairs of idiomatic code and non-idiomatic code and quantitative study to support  analysis  propose  are ver Python developers usually use Python idioms to write  are highly valued by Python developersPrevious researchers Python Compared with other mainstream programming languages, Python developers
%人们对性能的探索还很有限，有很多还有争议，甚至还是空白。
\textbf{(2) Developers are used to answering performance change with simple toy code for Python idioms.} For example, to explore the performance change of chain-comparison, developers write code pairs of \textsf{``a <= b <= c''} and \textsf{``a <= b and b <= c''} to compare the execution time (in the 5th row in Table~\ref{tab:motivation_soposts}).%%And 即使是toy code他们也意见不一致

\textbf{(3) Developers find that the performance change of Python idioms is not what they expect in their real code.} For example, for the list/set/dict comprehension, previous studies~\cite{} and developers generally think that it will improve the performance largely. However, for the set comprehension, developers find that the performance of set comprehension is basically same as that of the non-idiomatic code(3rd row in Table~\ref{tab:motivation_soposts}). For another example, for the truth-value-test, the developer is shock that the Python idioms could improve performance by more than 5 times (5th-to-last row in Table~\ref{tab:motivation_soposts}).
\begin{table}[tbp]
\vspace{-0.6cm}
\scriptsize\caption{Discussions about the performance change of Python idioms}
  \label{tab:motivation_soposts}
  \vspace{-0.3cm}
\centering
\begin{tabular}{|l|c|p{2.4in}|} 
\hline
Idiom          & \#C & Question \\ 
\hline
\begin{tabular}[c]{@{}l@{}}List Com-\\prehension\end{tabular}      & (3)    &\begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/59625860/python-why-is-this-list-comprehension-5000-times-slower-than-the-equivalent-for}{\fbox{\textbf{Question: }}}why is the list comprehension is slow?\\
with open("file.csv", 'r', newline = "$\backslash$n") as f:\\
    \ \ reader = csv.reader(f, delimiter = ",")\\
    \ \ data = [r for i, r in enumerate(reader) if i < 1000]\\

%\\table = ''\\for index in xrange(256):\\ \hspace{0.075cm} if index in ords\_to\_keep:\\ \hspace{0.15cm} table += chr(index)\\ \hspace{0.075cm} else:\\ \hspace{0.15cm} table += replace\_with\\
           \end{tabular}  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Set Com-\\prehension\end{tabular}       & (3)    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/38558834/use-list-set-comprehension-merely-as-a-for-loop}{\fbox{\textbf{Question: }}}Use set comprehension merely as a "for" loop?\\
record\_key\_list = \{(choice(tuple(studentID\_list)), ...,\\
                   choice(grades)[0]) 
                   for no\_use in range(NUM\_RECORDS)\}\\
I timed the two code snippets and \textbf{they are roughly the} \\\textbf{same as} fast for 20000 records.
\end{tabular}            \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Dict Com-\\prehension\end{tabular}      & \begin{tabular}[c]{@{}l@{}}(1)\\ (2)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/52542742/why-is-this-loop-faster-than-a-dictionary-comprehension-for-creating-a-dictionar/52542927#52542927}{\fbox{\textbf{Question: }}}Why is this loop faster than a dictionary\\ comprehension  for creating a dictionary?\\
a = \{'a':'hi','b':'hey','c':'yo'\}\\
b = \{v: k for k, v in a.items()\}
\end{tabular}            \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Chain-Co\\mparison\end{tabular}        & \begin{tabular}[c]{@{}l@{}}(1)\\ (2) \end{tabular}    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/48375753/why-are-chained-operator-expressions-slower-than-their-expanded-equivalent}{\fbox{\textbf{Question: }}}Why are chained operator expressions slower\\ than their expanded equivalent?\\In python, it is possible to chain operators in this manner:\\

a op b op c\\
Which is evaluated to\\

a op b and b op c \end{tabular}    \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Truth \\Value\\ Test \end{tabular}       & (3)    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/67747896/why-is-if-x-significantly-faster-than-if-x0-conways-game-of-life/67748136#67748136}{\fbox{\textbf{Question: }}}why is "if x:" significantly faster than "if x!=0"?\\
for y in range(self.cellsize):\\
      \ \       for x in range(self.cellsize):\\
      \ \ \ \           if self.neighbors[x, y] > 0:\\
      if self.neighbors[x, y] != 0 to if self.neighbors[x, y]\\ significantly speed up the function\end{tabular} \\
\hline
\begin{tabular}[c]{@{}l@{}}Loop \\Else\end{tabular}               & (1)    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/3295938/else-clause-on-python-while-statement}{\fbox{\textbf{Question: }}}Else clause on Python while statement\\
Actually a fairly useful construct for such a thing. \\Don't know how many times I've put found\_it=False\\ at the start of a loop, and then do an if check on found\_it \\at the end.\end{tabular}             \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Assign \\Multiple\\ Targets\end{tabular}    & \begin{tabular}[c]{@{}l@{}}(1)\\(2)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}
\href{https://stackoverflow.com/questions/22278695/python-multiple-assignment-vs-individual-assignment-speed}{\fbox{\textbf{Question: }}}Python assigning two variables on one line\\
I've been looking to squeeze a little more performance out of\\ my code; Recently, while browsing this Python wiki page, \\I found this claim:\\
Multiple assignment is slower than individual assignment.\\
I repeated several times, but the multiple assignment snippet\\ performed at least 30\% better than the individual assignment. 
% \href{https://stackoverflow.com/questions/44517911/swapping-variables-in-python3}{\fbox{\textbf{Question: }}}I have just started learning python3. How is this line\\ a,b = b,a working?... can I do the same for 3 or more variables in one line?\\
% Asked 4 years; Active 4 years; Viewed 8k times
\end{tabular}     \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Star in \\Func Call\end{tabular} & \begin{tabular}[c]{@{}l@{}}(1)\\(2)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/2921847/what-does-the-star-and-doublestar-operator-mean-in-a-function-call}{\fbox{\textbf{Question: }}}What does the star and double star operator\\ mean in a function call?\\
Does it affect performance at all? Is it fast or slow?
\end{tabular}          \\ 
\hline
\begin{tabular}[c]{@{}l@{}}For \\Multiple\\ Targets\end{tabular}       & (3)    & \begin{tabular}[c]{@{}l@{}}\href{https://stackoverflow.com/questions/13024416/how-come-unpacking-is-faster-than-accessing-by-index}{\fbox{\textbf{\textbf{Question: }}}}How come unpacking is faster than accessing \\by index?\\
\end{tabular}            \\
\hline
\end{tabular}
\vspace{-0.8cm}
\end{table}
%应该可能会加些东西，给出人们对于performance of python idioms的误区和困惑，在implications给出answer
% 1. 人们对于Python idioms的性能很感兴趣经常提出一些问题，views很多 经常询问快还是慢，进一步知道快多少， 满多少 
%2 人们到底快还是慢faster slower 3. 人们希望知道快多少，满多少
% 

% 3. 人们验证性能的时候，经常使用toy code. 人们有一种信念觉得Python idioms一定会快或者慢， 但在实际数据中发现性能的提升并不理想

% 4. 人们在实际代码中发现性能提升并不如人意。1. 不知道idioms哪些方面影响着性能， 

==> result.tex <==
\subsection{RQ1:What Is the Impact of Idiomatic-Refactoring on Performance?}
\subsubsection{Motivation}
Section~\ref{motivation} shows that developers are interested in whether idiomatic Python code executes faster or slower than non-idiomatic Python code. Since there is currently no systematic and complete study, developers are still unclear about the performance impact of idiomatic code refactoring. Therefore, this research question answers whether the impact of idiomatic Python code refactoring on performance is improved, reduced, or almost no effect.
\subsubsection{Approach}
\textbf{Reliable detection of performance change}. As described in Section~\ref{data}, we collect XXX non-idiomatic and the corresponding idiomatic code pairs for nine Python idioms. Each refactoring-related code has one of the following effects on the performance:
\begin{enumerate}[fullwidth,itemindent=0em,leftmargin = 0pt]
	\item[Regression:] Idiomatic code executes faster than non-idiomatic code. 
% 	\item[\textbf{RQ2:}] How much performance is improved when refactoring java-style python code into pythonic code? 
% 	\item[\textbf{RQ3:}] How much programmer effort is saved by our approach when refactoring? 
	\item[Improvement:] Idiomatic code executes slower than non-idiomatic code.
	\item[Unchanged:] The execution time of idiomatic code and non-idiomatic code is almost the same.
\end{enumerate}
To determine reliably which category the performance impact of refactoring falls into, we apply the approach of quantifying performance changes with effect size proposed by Kalibera et al.~\cite{kalibera2013rigorous,kalibera2020quantifying}. Compared to other performance evaluation approaches (e.g., hypothesis testing with Wilcoxon rank-sum combined with effect sizes~\cite{georges2007statistically,laaber2019software} and overlapping confidence intervals~\cite{georges2007statistically,laaber2019software}), the main benefit of the Kalibera et al. technique is that it provides a clear and rigorous account of the performance change magnitude and of the uncertainty involved. For example, it can indicate that an idiomatic code is slower (or faster) than a non-idiomatic code by X \% ± Y\% with 95\% confidence. Similar to previous studies~\cite{kalibera2013rigorous,kalibera2020quantifying,traini2021software}, to build the confidence interval we use bootstrapping with hierarchical random re-sampling and replacement~\cite{davison1997bootstrap,ren2010nonparametric,traini2021software} on two levels~\cite{traini2021software,kalibera2020quantifying}: VM invocations and iterations. Specifically, we run 100 bootstrap iterations. At each iteration, we compute the relative performance change as follows:
$$\rho=\frac{\sum_{i=1}^{n}\sum_{j=1}^{k}m_{i,j}^{before}}{\sum_{i=1}^{n}\sum_{j=1}^{k}m_{i,j}^{after}},$$
where $n$ is the number of VM invocations, $m$ is the number of measurements iterations, and $m_{i,j}$ is the execution time of the $k$th iteration in the $i$th invocation.

After the termination of all iterations, we collect a set of simulated realizations of the relative performance change $P = \{\rho_i \mid 1 \le i \le 100\}$ and estimated the 0.025 and 0.975 quantiles on it, for a 95\% confidence interval. The performance change is improvement if the lower limit of the confidence interval for relative performance change of total execution times is greater than 1; The performance change is regression if the upper limit of the confidence interval is less than 1. Otherwise, we consider performance as unchanged.

\textbf{Quantitative analysis of performance change}. After computing the performance changes of all refactoring-related codes, we analyze and summarize what kind of code can bring performance improvement/regression/unchanged for each Python idiom. We construct a decision tree model~\cite{} to examine the relationship between the performance change and code features from from Section~\ref{data}. The decision tree classifier is a popular popular machine learning algorithms given their intelligibility and simplicity~\cite{wu2008top}. Compared to other classifier models, e.g., logistic regression model and Naive Bayes, the unique benefit is because the decision tree classifier could visually and explicitly represent decisions based on the value of a feature at each step~\cite{shalev2014understanding}, which easily help us understand the relationship between performance change and code features. We set the max depth of decision tree is three because we find the depth is enough to help us understand relationship between performance change and code features of most of code refactorings and too much depth makes analysis too redundant and complex. To ensure reliability of decision tree classifier, we use the 10-fold cross validation to evaluate our model which is the most widely used evaluation approach~\cite{kim2008classifying,shihab2012industrial, gousiospullrequest}. Specifically, all idiomatic and corresponding non-idiomatic code pairs are divided into 10 data sets, each containing 10\% of the data. One set serves as the testing data and the remaining nine sets are used as training data. In our results, we report the average AUC-ROC across all 10 fold result as the primary accuracy indicator to indicate the effectiveness of our decision model. The AUC-ROC is widely used in many studies~\cite{fan,bao2017will,fan2018early,lamkanfi2010predicting}, which considers true positive rate and false positive rate and is not biased for different class distributions. Lessmann et al.~\cite{lessmann2008benchmarking} recommended that we use the AUC-ROC as the primary accuracy indicator to compare the performance of prediction models. Romano et al.~\cite{romano2011using} concluded that a prediction model with an AUC score above 0.7 is often considered to have adequate classification performance. 
\subsubsection{Result}%%！！！这里或许展示auc说明下分析结果的可靠性
Figure~\ref{fig:performance_rq1} reports the percentages of each kind of performance change for nine types of Python idioms.

\begin{figure}
  \centering
  \includegraphics[width=3.4in]{./data/performance_rq1.pdf}
\setlength{\abovecaptionskip}{-0.3cm}
    \caption{Types of performance change}
    
    \label{fig:performance_rq1} \vspace{-0.3cm}
    %\vspace{-0.6cm}
\end{figure}
%https://scikit-learn.org/stable/auto_examples/tree/plot_unveil_tree_structure.html#sphx-glr-auto-examples-tree-plot-unveil-tree-structure-py
\noindent\textbf{List comprehension}.
Figure~\ref{fig:performance_rq1} shows most of idiomatic refactorings of list comprehension improve or decrease performance, and the percentage of unchanged performance accounts for less than 1\%. Figure~\ref{fig:visualize_list_compre_rq1} shows how decision tree classifier make decisions based on the value of each feature. Each node consists of a threshold value of a feature, gini, samples, value and class, which means  whether splitting node or not, the impurity of the node (e.g., all samples of the node belongs to the same class if the gini is 0), the number of samples of the node, how many samples belong to the three categories of the node, the category the samples of the node belongs to, respectively. Figure~\ref{fig:visualize_list_compre_rq1} shows two interesting 
findings as follows:
\begin{enumerate}[fullwidth,itemindent=0em,leftmargin = 0pt]
	\item[a. Improvement:] When the number of elements appended to the list is larger than 1, the performance will improve (path:\textcircled{1}). Particularly, if the variables of the code is not in function (i.e., the global scope), the performance is likely to improve although the number of elements appended to the list is only 1 (path:\textcircled{2} $\rightarrow$ \textcircled{4} $\rightarrow$ \textcircled{5}). 
 
	\item[b. Regression:] If the list has no elements appended for list comprehension, the performance will decrease (path:\textcircled{2} $\rightarrow$ \textcircled{3}). Particularly, if the number of appended elements of code in the function (i.e., the local scope) is is only 1, the performance is likely to decrease(path:\textcircled{2} $\rightarrow$ \textcircled{4} $\rightarrow$ \textcircled{6}).
\end{enumerate}
\begin{figure}
  \centering
  \includegraphics[width=3in]{./data/performance_rq1_list_compre_edge.png}%performance_rq1_list_compre.pdf
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Visualization of decisions of decision tree of list comprehension}
    
    \label{fig:visualize_list_compre_rq1} \vspace{-0.3cm}
    %\vspace{-0.6cm}
\end{figure}

\noindent\textbf{Set comprehension}. Figure~\ref{fig:performance_rq1} shows most of idiomatic refactorings of set comprehension improve or decrease performance, and the percentage of unchanged performance accounts for less than 5\%. Three interesting findings as follows:
\begin{enumerate}[fullwidth,itemindent=0em,leftmargin = 0pt]
	\item[a. Improvement:] The result is the same as the result of the list comprehension. 

	\item[b. Regression:] If the list has no elements appended for list comprehension, the performance will decrease.
	\item[c. Unchanged:] If the number of appended elements of code in the local scope is only 1, the performance basically is unchanged. Although few such kind of code may decrease, the performance change is close to 1, basically above 0.95.
\end{enumerate}

%Table 2 shows that, our random forest classi￿ers achieve an average AUC of 0.86, 0.59, 0.69, 0.72, and 0.73 for elapsed time, CPU usage, memory usage, I/O read and I/O write, respectively. Similarly, for project Hadoop, our classi￿ers achieve an average AUC of 0.90, 0.68, 0.66, 0.79 for elapsed time, CPU usage, memory usage, and I/O write, respectively
\noindent\textbf{Dict comprehension}.%0.898 AUC
Figure~\ref{fig:performance_rq1} shows idiomatic refactorings of dict comprehension may improve, decrease or not change performance. Compared to idiomatic refactorings of list comprehension and set comprehension, the percentage of performance improvement of dict comprehension is lower than that of them. Three interesting findings as follows:
\begin{enumerate}[fullwidth,itemindent=0em,leftmargin = 0pt]
	\item[a. Improvement:] Compared to idiomatic refactorings of list and set comprehension, idiomatic refactorings of dict comprehension needs to append more elements than them, at least greater than 10, its performance can improve. Particularly, if the idiomatic refactorings have elements added and in global scope, the performance can improve.
 
	\item[b. Regression:] If idiomatic refactorings are in the global scope and the number of added elements is less than or equal to 1, the performance is reduced. 
	\item[c. Unchanged:] If idiomatic refactorings are in the local and the number of elements added is less than 10, the performance is basically unchanged.
\end{enumerate}

%4937 1364 5667 regre, unchange, impr
\noindent\textbf{Chain comparison}. Figure~\ref{fig:performance_rq1} shows idiomatic refactorings of chain comparison may improve, decrease or not change performance.
Three interesting findings as follows:
\begin{enumerate}[fullwidth,itemindent=0em,leftmargin = 0pt]
	\item[a. Improvement:] When the code is in the global scope, the idiomatic refactorings will improve the performance.

	\item[b. Regression/Unchanged:] When the code is in the local scope, idiomatic refactorings are more likely to  decrease or do not change the performance.
\end{enumerate}

\noindent\textbf{Truth value test}. Figure~\ref{fig:performance_rq1} shows all idiomatic refactorings of truth value test improve the performance.

%0.9375 AUC
\noindent\textbf{Loop Else}. Figure~\ref{fig:performance_rq1} shows all idiomatic refactorings of truth value test improve or do not change the performance. When the loop iterations is less than 1,000 times, the performance generally improves, otherwise the performance basically does not change.

\noindent\textbf{Assign Multiple Targets}. Figure~\ref{fig:performance_rq1} shows idiomatic refactorings may improve, decrease or not change performance.
Three interesting findings as follows:
\begin{enumerate}[fullwidth,itemindent=0em,leftmargin = 0pt]
	\item[a. Improvement:] When variable assignment code in the global scope is to swap variables, the idiomatic refactorings will improve the performance. When the assignment code is to swap two variables in the local scope, the performance will also improve. For the constant assignment code, the idiomatic refactorings can improve the performance if the number of the assignment node is larger than 8 at least.

	\item[b. Regression:] When variable assignment code is not to swap variables but to assign values, the idiomatic refactorings will decrease the performance. When the assignment code is to swap variables and the number of assign nodes is larger than 3, the performance will decrease.
	
	\item[c. Unchanged:] When the number of constant assignment node is less than 8 for the constant assignment code, the idiomatic refactorings generally does not change the performance.
\end{enumerate}

\noindent\textbf{Star in Function Calls}. Figure~\ref{fig:performance_rq1} shows most of idiomatic refactorings may improve or decrease performance. The percentage of unchanged perfofrmance accounts about 5\%. Two interesting findings as follows:

\begin{enumerate}[fullwidth,itemindent=0em,leftmargin = 0pt]
	\item[a. Improvement:] If the code fetchs all elements of the iterator, the performance generally will improve. Otherwise, when the number of subscript node is larger than 4 at least, the performance can improve.


	\item[b. Regression:]  If the code fetchs part of elements of the iterator and its number of subscript node is less than 4, the performance generally decreases.

\end{enumerate}

\noindent\textbf{For Multiple Targets}. Figure~\ref{fig:performance_rq1} shows most of idiomatic refactorings may improve or decrease performance. The percentage of unchanged performance accounts about 1\%. Two interesting findings as follows:

\begin{enumerate}[fullwidth,itemindent=0em,leftmargin = 0pt]
	\item[a. Improvement:] If the code unpack all elements of the iterator, the performance generally improves.

	\item[b. Regression:]  If the code unpack part elements of the iterator, the performance generally decreases.

\end{enumerate}
\subsection{RQ2: What is the relationship between code features and the performance change?}\label{rq2}
\subsubsection{Motivation}
Section~\ref{motivation} shows that developers are interested in how much idiomatic refactorings can improve or degrade performance. In the research question, investigating the relationship between code features and performance change could help developers make better choices about how they code and which idioms to prioritize to refactor their code.
\subsubsection{Approach}
As described in Section~\ref{measurement}, we repeatedly execute each code snippet on two levels: VM invocations and iterations. To represent the performance change before and after idiomatic refactorings, we divide the total of execution time of non-idiomatic code by that of corresponding idiomatic code which indicates how much speedup idiomatic code has compared with non-idiomatic code. The code features come from Section~\ref{data}.

% https://ecoforecast.org/workshops/statistical-methods-seminar-series/#simpson
%https://www.youtube.com/watch?v=XQ1vk7wEI7c
%
%yGAM is an extension to linear and generalized linear models, where it could  so it could find a balance between predictive power and interpretability. nonlinear and non-monotonic relationships between the response variable and explanatory variables [21]Since the performance change is a continuous value, and relationships between the performance change and code features are not assumed to be linear, we construct a Generalized additive model (GAM) to analyze their relationships
To analyze the relationship between the performance change and code features, we construct a Generalized additive model (GAM)~\cite{tan2022exploratory,hastie2017generalized}. Compared to linear models, it can analyze the nonlinear and non-monotonic relationships between the response variable and explanatory variables~\cite{hastie2017generalized}. Compared to machine learning algorithms, it is more interpretable. So, it could implement a balance between predictive power and interpretability~\cite{serven2018pygam}. Similar to previous studies~\cite{hastie2017generalized}, we first log transform highly skewed performance change and numeric code features. Then, we use the variance inflation factor (VIF) to analyze the multicollinearity of the prediction variables~\cite{mansfield1982detecting}. If the VIF of two 
features is larger than 5, there is significant multicollinearity among the features, we randomly remove a feature. Finally, we build a GAM model with the feature values and performance changes provided by the package ``mgcv'' in R language. 
\subsubsection{Result}% Figure 1 shows the distribution of the maximum spread of each benchmark for the study subjects in violin plot notation. To ease visual comprehension, we have limited the y-axis to 1.00 for Java and 0.5 for Go, even though some projects have a small number of outlier benchmarks with even higher maxSpread.展示 deviance explained 
Figure~\ref{fig:distri_rq2} shows the distribution of performance change of idiomatic code refactorings for nine types of Python idioms.

\begin{figure}[tbp]
  \centering
  \includegraphics[width=3.4in]{./data/performance_rq2.pdf}%performance_rq1_list_compre.pdf
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Distribution of performance change of experimental idiomatic refactorings of nine kind Python idioms}
    
    \label{fig:distri_rq2} %\vspace{-0.3cm}
    \vspace{-0.2cm}
\end{figure}
%https://www.statology.org/interpret-prt-regression-output-r/ p-value
\noindent\textbf{List comprehension}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.5$\sim$5.6. The deviance explained of the GAM model is about 90\%, which means our model can explain the relationship between performance change and features well. Table~\ref{tab:relation_code_performance} shows the feature importance and the positive/negative relationship between performance change and features reported by GAM model. The Pr(>|t|) column represents the p-value associated with the value in the t value column; The t column represents the feature importance, where the sign of value represent the positive/negative relationship between code features and performance change, and the larger the absolute value of t, the more important the feature is. 

There are four features in the first 4 rows of the table that have a statistically significant relationship with the performance change because the p-value is less than 0.05. The two most important features num\_ele and context are interesting. The value of performance change increases as the number of added elements increases, whereas when the number of elements appended reaches a certain degree, the value of performance change remains basically the same. For context feature, the performance change of the variables of the code in the global scope is greater than the performance in the local scope. When the number of elements added is larger than 10,000 of code not in function, the biggest performance change is about 5; When the number of elements added is larger than 10,000 of code in function, the biggest performance change is about 3.
\begin{table}[tbp]
%\vspace{-0.2cm}
\caption{The relationship between code features and performance change}
  \label{tab:relation_code_performance}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l c c c} 
\hline
Feature  & Pr(>|t|)   & t &relationship\\ \hline

num\_ele & <2e-16 & 39.013 &positive\\ %\hline

context  & <2e-16   & -27.198&negative \\%\hline
num\_if    &<2e-16  & -14.478&negative\\ 
%\hline
num\_if\_else  &<2e-16 &  -9.510&negative \\ %\hline
num\_loop &0.796 &0.259&positive\\\hline
\end{tabular}
\vspace{-0.3cm}
\end{table}

\noindent\textbf{Set comprehension}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.6$\sim$4.1. The deviance explained of the GAM model is about 88\%, which means our model can explain the relationship between performance change and features well. The relationship between code features and performance derived from the GAM is the same as the results of list comprehension. When
the number of added elements is larger than 1,000 of code in the global scope, the biggest performance change is about 4;
When the number of added elements is larger than 1,000 of
code in the local scope, the biggest performance change is about 2.6.


%When #authors is small, it is negatively related to #downstream_projects, whereas when #authors reaches a certain de- gree (> 7 developers), it shows a significantly positive relationship. This may indicate that for small teams, the collaboration among team members may reduce the efficiency of developers. The rela- tionship between #dependencies and #downstream_projects is linear, and #dependencies is negatively related with #downstream_projects. Dey et al. [15] obtain the similar finding: packages having fewer packages as dependencies are likely to see an increase in downloads. However, the number of stars, age, and many SCs related factors, e.g., SC name and No.layer do not show significant relationship.

%https://stackoverflow.com/questions/52542742/why-is-this-loop-faster-than-a-dictionary-comprehension-for-creating-a-dictionar !!! 重要的解释
\noindent\textbf{Dict comprehension}.
Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.8$\sim$2.2. The deviance explained of the GAM model is about 91\%, which means our model can explain the relationship between performance change and features well. The
relationship between code features and performance derived
from the GAM is the same as the results of set comprehension and list comprehension. Compared to list comprehension and set comprehension, the performance improvement is not big. The maximum performance change in the global scope and in the local scope can reach about 2.2 and 1.2, respectively.%The maximum of performance change of code in the global scope can reach about 2 %When the number of added elements is larger than 100 of code in the global scope, the maximum of performance change can reach about 2; When the number of added elements is larger than unsure too various of code in the local scope, the biggest performance change is about 1.2.

%%0.8256 AUC indicates the performance change
\noindent\textbf{Chain comparison}.
Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.7$\sim$1.6. The deviance explained of the GAM model is about 55\%. From the result of GAM, there are two findings about the relationship between performance change and code features. The one is that the most important feature is the context. The performance change of variables in the global scope is greater than that in the local scope. The other is that the number of chained comparison comparators has no statistically significant relationship with performance change.

\noindent\textbf{Truth value test}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 1.02$\sim$7.2. The deviance explained of the GAM model is about 99.6\%. Based on results of GAM model, there are three findings about the relationship between performance change and code features. First, the node kind of operator has no statistically significant relationship with performance change. For example, for \textsf{``if a != []''} and \textsf{``if a == []''}, their corresponding idiomatic codes are \textsf{``if a''} and \textsf{``if not a''}. Although \textsf{``if not a''} has one more \textsf{``not''} than \textsf{``if a''}, their performance changes are basically the same. Second, the parent node to which the comparison node belongs has no statistically significant relationship with performance change. For example, the performance changes of idiomatic refactorings of \textsf{``if a != []''} and \textsf{``while a != []''} basically are same. Finally, the \textsf{``Fraction(0, 1), Decimal(0), range(0), dict() and set()''} comparators have a significant positive relationship with performance change. If the comparator is \textsf{``Fraction(0, 1)''}, the performance improvement can reach about 7. If the data type of the comparator is the basic data type such as int, float and string, the performance improvement is relatively small, basically less than 1.2.

\noindent\textbf{Loop Else}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.99$\sim$1.9. The deviance explained of the GAM model is about 95.1\%. From the result of the GAM, there are three findings. First, the loop iterations have statistically negative relationship with the performance change. As the number of iterations increases, the performance change decreases. Second, whether the code goes through the break statement have statistically positive relationship with the performance change. The performance change of the code path with the break statement is greater than of the code path without the break statement. Finally, the loop node kind (i.e., for and while node) has no statistically relationship with the performance change. %which are negatively and positively related to performance change. 

\noindent\textbf{Assign Multiple Targets}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.7$\sim$1.4. The deviance explained of the GAM model is about 69\%. There are three important features. First, the most important feature is whether the assignment code is to swap variables or not. The performance change of idiomatic refactorings that swap variables is greater than of code that does not swap variables. Then the performance change of code in the global scope is greater than of code in the local scope. Finally, The performance change of idiomatic refactorings of constants assignment is greater than of code of variables assignment.

\noindent\textbf{Star in Function Calls}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.5$\sim$3.2. The deviance explained of the GAM model is about 91\%. The top three important features are the number of the subscript node, the context and whether the index of the subscript node is constant or not. First, as the number of subscript node increases, the performance change will increase. Second, the performance change of code in the global scope is greater than of code in the local scope. Finally, the performance change of the constant index of the subscript node is less than of variable index of subscript node. 

\noindent\textbf{For Multiple Targets}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.1$\sim$6.9. The deviance explained of the GAM model is about 89\%. The top three important features are whether the code unpacks all elements at each iteration, the context and the number of the subscript node. First, the performance change of code to unpack all elements is greater than of code to unpack part elements. Second, the performance change of code in the local scope is greater than of code in the global scope. Finally, as the number of subscript node increases, the performance change will increase. 

\subsection{RQ3:What are the differences of performance between experimental code and real-scenario code?}
\subsubsection{Motivation}
Although constructing experimental code could help us have a basic understanding for performance change of the idiomatic refactoring with Python idioms, real-scenario code have more complex forms such as the use of class objects and function calls. Therefore, in the research question, we would like to understand whether real-scenario code will have different impact on performance change compared to the real-scenario code.
\subsubsection{Approach}
As describe in Section~\ref{data}, we collect XXX non-idiomatic and the corresponding idiomatic code pairs for nine Python
idioms. To find the differences of performance between experimental code and real-scenario code, we first extract  the performance changes and code features for each idiomatic refactoring. Then we compare the performance change of experimental code from ~\ref{rq2} with the performance change of real-scenario code based on values of code features to get the performance change only exist in real scenarios. 

\subsubsection{Result} Figure~\ref{fig:distri_rq3} shows the distribution of performance change of idiomatic refactoring for nine types of Python idioms.
\begin{figure}
  \centering
  \includegraphics[width=3.4in]{./data/performance_rq3.pdf}%performance_rq1_list_compre.pdf
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Distribution of performance change of idiomatic refactorings in the field of nine kind Python idioms}
    
    \label{fig:distri_rq3} %\vspace{-0.3cm}
    \vspace{-0.2cm}
\end{figure}
\begin{table*}[tbp]
%\vspace{-0.2cm}
\caption{the performance change of code examples of nine Python idioms in the field code}
  \label{tab:rq3_example}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l| l| l| c| c} 
\hline
Idiom&non-idiomatic code  & idiomatic code   & code feature &X\\ \hline

\href{https://github.com/kellyjonbrazil/jc/blob/e2f1b16cb9e920968c093bd1f371b191aa7107bf/jc/parsers/csv.py#L145-L146}{list-compre} & \begin{tabular}[c]{@{}l@{}} raw\_output=[]\\for row in reader:\\    \ \  raw\_output.append(row)\end{tabular} & \begin{tabular}[c]{@{}l@{}}raw\_output = [row \\for row in reader]\end{tabular} &num\_ele:11,766& 1.03\\ \hline
\href{https://github.com/sympy/sympy/blob/82f264c62db6382fd3545bb43f57584b0f4e27c2/sympy/combinatorics/testutil.py#L195-L197}{set-compre} & \begin{tabular}[c]{@{}l@{}} conjugates = set()\\for el in group.generate\_dimino():
\\   \ \ for gen in subgr\_gens:
\\   \ \    \ \      conjugates.add(gen $\wedge$ el)\end{tabular} & \begin{tabular}[c]{@{}l@{}}conjugates = \{gen $\wedge$ el\\ for el in group.generate\_dimino() \\for gen in subgr\_gens\}\end{tabular} &num\_ele:44& 1.008\\ \hline
\href{https://github.com/networkx/networkx/blob/7b30f1a814d6b7f1b3c4311d19c251b8098d1407/networkx/algorithms/community/quality.py#L299-L302}{dict-compre} & \begin{tabular}[c]{@{}l@{}} rv = \{\}\\for (k, v) in d.items():\\
\  \    rv[k] = v.\_\_self\_\_\end{tabular} & \begin{tabular}[c]{@{}l@{}}rv = \{k: v.\_\_self\_\_ for (k, v) in d.items()\}\end{tabular} &num\_ele:1,000& 1.004\\ \hline

\href{https://github.com/brainix/pottery/blob/c7be6f1f25c5404a460b676cc60d4e6a931f8ee7/pottery/deque.py#L56}{chain-comparison} & \begin{tabular}[c]{@{}l@{}} self.maxlen is not None and \\ current\_length >= self.maxlen\end{tabular} & \begin{tabular}[c]{@{}l@{}}None is not self.maxlen <= current\_length\end{tabular} & context: in the function& 1.3\\ \hline

\href{https://github.com/nipy/nibabel/blob/225892af18d82b9a91ab63a9d072b894588b670e/nibabel/volumeutils.py#L940}{truth-value-test} & \begin{tabular}[c]{@{}l@{}} if inter != 0:\end{tabular} & \begin{tabular}[c]{@{}l@{}}if inter:\end{tabular} &comparator:0& 11.8\\ \hline

\href{https://github.com/quantumlib/OpenFermion/blob/5ef58b507270f18627ec563a43001c404cf5e6c1/src/openfermion/measurements/fermion_partitioning.py#L276-L282}{loop-else} & \begin{tabular}[c]{@{}l@{}} success\_flag = True\\
    for divisor in range(2, num\_bins - 1):\\
    \ \     if trial\_size \% divisor == 0:\\
        \ \ \ \     success\_flag = False\\
        \ \ \ \     break\\
    if success\_flag:\\
       \ \  return trial\_size\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    for divisor in range(2, num\_bins - 1):\\
    \ \     if trial\_size \% divisor == 0:\\
        \ \ \ \     break\\
    else:\\
       \ \  return trial\_size\end{tabular} &iterations:<10& 1.3\\ \hline
       
\href{https://github.com/Erotemic/ubelt/blob/cdb6aa9dea7567ce742ee6a11d8a1ca4ac89f342/ubelt/util_cache.py#L497-L501}{assign-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
cfgstr = self.\_rectify\_cfgstr(cfgstr)\\
dpath = self.dpath\\
fname = self.fname\\
verbose = self.verbose
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    cfgstr , dpath , fname , verbose  = \\ self.\_rectify\_cfgstr(cfgstr), self.dpath,\\ self.fname, self.verbose\end{tabular} &variable assignment& 0.78\\ \hline

\href{https://github.com/presslabs/gitfs/blob/12886ec5b9c7e103bfcab0cd37a8333873382fae/gitfs/repository.py#L170}{star-in-func-call} & \begin{tabular}[c]{@{}l@{}} 
Signature(commiter[0], commiter[1])
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    Signature(*commiter[:2])\end{tabular} &num\_subscript:2& 0.87\\ \hline


\href{https://github.com/alichtman/shallow-backup/blob/d71b903dacd5eeea9d0be68ef3022817f9bac601/shallow_backup/backup.py#L81-L84}{for-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
for x in dotfiles\_mp\_in:\\
\ \     x[0]\\
\ \     x[1]
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    for  (x\_0, x\_1, *x\_len)  in dotfiles\_mp\_in:\\
\ \     x\_0\\
\ \     x\_1\end{tabular} &num\_subscript:2& 0.98\\ \hline
\end{tabular}
\vspace{-0.3cm}
\end{table*}

\noindent\textbf{List comprehension}. Figure~\ref{fig:distri_rq3} shows the performance change range is about 0.4$\sim$1.5. We find the performance improvement is relatively small, not even hit 2 although the number of elements appended to the list of code in function is more than 10,000. For example, the code(the first row of Table~\ref{tab:rq3_example}), the number of added elements is 11,766, the performance improvement is only about 1.03.

\noindent\textbf{Set comprehension}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.6$\sim$1.3. Similar to list comprehension, the performance improvement
is small. For example, the code(the 2nd row of Table II),
the number of added elements is 44, the performance
change is only about 1.008 but the performance change of experimental data could reach about 1.6 although the added elements is 10. 

\noindent\textbf{Dict comprehension}.
Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.5$\sim$1.1. Similar to list comprehension, the performance improvement
is small. For example, the code(the 3rd row of Table~\ref{tab:rq3_example}),
the number of added elements is 1,000, the performance
change is only about 1.004. 


\noindent\textbf{Chain comparison}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.5$\sim$1.3. The one difference is that the idiomatic refactorings can improve performance in the field code instead of decreasing performance in the experimental code when the variables of code are in the local scope. For example, the performance improvement is about 1.3 for the \textsf{``self.maxlen is not None and current\_length >= self.maxlen''} code in the local scope (the 4th row of Table~\ref{tab:rq3_example}). 

\noindent\textbf{Truth value test}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.1$\sim$12. There are two main differences between the performance changes of idiomatic refactorings of experimental data and real scene data. The one is that the performance improvement may bigger than 7 when the data type of the comparator is not Python built-in data types. For example, the \textsf{``inter $!=$ 0''} code (the 5th row of Table~\ref{tab:rq3_example}), the data type of \textsf{``inter''} is \textsf{``numpy.array''}, the performance change is even more than ten times. The other is that the performance may even decrease, less than 1, when the data type of the comparator is not Python built-in data types. For example, for the \href{https://github.com/searx/searx/blob/5b50d7455a719b145be5f90069026a60b480673d/searx/utils.py#L259}{\textsf{``xpath\_results $==$ []''} code}, the data type of \textsf{``xpath\_results''} is \textsf{``lxml.html.HtmlElement''}, the performance change is less than 0.2.

% remove one sample!!! 0.2
\noindent\textbf{Loop Else}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.9$\sim$1.3. There is no difference in performance change of idiomatic refactorings between the field code and the experimental code.

\noindent\textbf{Assign Multiple Targets}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.7$\sim$1.2. There is no difference in performance change of idiomatic refactorings between the field code and the experimental code.

\noindent\textbf{Star in Function Calls}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.6$\sim$1.03. There is no difference in performance change of idiomatic refactorings between the field code and the experimental code. %The maximum of performance change in the field code is relatively smaller than of performance change in the experimental code because 

\noindent\textbf{For Multiple Targets}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.18$\sim$1.0. There is no difference in performance change of idiomatic refactorings between the field code and the experimental code. The maximum of performance change is almost 1 because we set the code unpacks the part of elements to ensure the correctness of the code refactoring. For example, the \textsf{``*x\_len''} code represents there may be some unused elements in the the last row of the Table~\ref{tab:rq3_example}. Therefore, there is no idiomatic refactorings improve the performance.

\subsection{RQ4:What are the reasons of performance change caused by idiomatic refactorings?}
\subsubsection{Motivation}
 In the 3 previous research questions, we find that code refactoring with the same Python idiom could improve or decrease performance if the code is different. And the relationship between code features and performance change is various. Therefore, in this research question, we would like to understand the reason that different code have different effects on performance change of 
idiomatic refactoring for each Python idiom.% The findings can assist help developers practition- ers in avoiding the use of certain tests in performance assurance activities and in improving tests to serve as performance tests.
\subsubsection{Approach}
To explore the reason of performance change caused by idiomatic refactorings for each Python idiom, it is not reliable to compare the difference of source code between idiomatic code and the corresponding non-idiomatic code because Python interpreter does not directly execute the source code. When the Python code runs, source code first gets compiled into a set of instructions called bytecode. Then the bytecode is executed by the Python interpreter. Therefore, we first get the bytecode instructions of idiomatic code and the corresponding non-idiomatic code for each Python idiom with dis module~\cite{dis_python}. The dis module supports the analysis of CPython bytecode by disassembling it. Then we compare their difference of instructions to understand the impact of code features on performance.%说明为什么用字节码解释 source code 执行的过程https://legacy.python.org/workshops/1998-11/proceedings/papers/montanaro/montanaro.html，用字节码解释的方法过程 字节码每个meta的概念https://github.com/python/cpython/blob/main/Doc/library/dis.rst


% https://towardsdatascience.com/list-comprehensions-vs-for-loops-it-is-not-what-you-think-34071d4d8207
%https://stackoverflow.com/questions/58844643/why-is-my-list-comprehension-function-slower-than-my-list-appending-function-for
\subsubsection{Result}
\noindent\textbf{List comprehension}.
The reason of performance improvement is that the list comprehension replaces the instructions of function calls with an instruction \textsf{``LIST\_APPEND''} (green dotted box in Figure~\ref{fig:bytecode_list_compre}). Each iteration, the non-idiomatic code executes instructions of function call, but the corresponding idiomatic code only needs to execute the \textsf{``LIST\_APPEND''} instruction for appending elements, so as more elements are appended, the greater the performance change. When the added element exceeds a certain value, the performance change basically no longer increases, which is approximately the cost of instructions of function call divided by the cost of the \textsf{``LIST\_APPEND''} instruction.

The reason of performance regression is the extra cost of instructions of listcomp function call (red dotted box in Figure~\ref{fig:bytecode_list_compre}). Before iteration, idiomatic code needs to load and call listcomp function.

% https://blog.csdn.net/xfxf996/article/details/105391374
The reason of performance change in global scope is larger than the performance change in local scope is that the cost of \textsf{    ``LOAD\_FAST''} instruction of loading local variables is less than the cost of \textsf{``LOAD\_NAME''} instruction of loading global variables. For example, each iteration, non-idiomatic code needs to execute instructions of loading variables \textsf{``raw\_output''} and  \textsf{``row''}. When the code are in function, the variables are local variables. The instruction of loading local variables is \textsf{``LOAD\_FAST''} while the instruction of global variables is \textsf{``LOAD\_NAME''}. Since the cost of \textsf{``LOAD\_FAST''} is 
less than the cost of \textsf{``LOAD\_NAME''}, the cost of instructions of executing  \textsf{``raw\_output.append(row)''} in the local scope is less than the corresponding cost in the global scope, so the performance change of idiomatic code in the local scope is less than that of idiomatic code in the global scope.

%why generator或者非内置的object slower 有https://www.programiz.com/python-programming/generator
%https://www.programiz.com/python-programming/iterator
The reason of performance change is relatively small although the real-scenario code adds lots of elements is the cost of method calls of non-built-in types. For example, for the code of the 1st row of Table~\ref{tab:rq3_example}, the \textsf{``reader''} is a reader object from csv library. Each time self-implemented \textsf{``\_\_next\_\_()''} method is called, the cost is larger than the cost of \textsf{``append''} method of list.
\begin{figure}
  \centering
  \includegraphics[width=3.5in]{./data/rq4_bytecode.png}%performance_rq1_list_compre.pdf
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Bytecode instructions of idiomatic refactorings of list comprehension}
    
    \label{fig:bytecode_list_compre} \vspace{-0.3cm}
    %\vspace{-0.6cm}
\end{figure}

\noindent\textbf{Set comprehension}.
The reason of performance improvement is that the set comprehension replaces the instructions of function calls with an instruction \textsf{``SET\_ADD''}. Similar to list comprehension, \textsf{``SET\_ADD''} instruction of idiomatic code reduces the cost of \textsf{``add''} function call of non-idiomatic code.

The reason of performance regression is the extra cost of instructions of setcomp function call. Before iteration, idiomatic code needs to load and call setcomp function.



Similar to list comprehension, the reason of performance change in global scope is larger than the performance change in local scope is that the cost of instructions of the function call is reduced in the local scope compared to that of cost in the local scope. Therefore, the difference between \textsf{``SET\_ADD''} instruction and instructions of \textsf{``obj.add(e)''} function call.

The reason of performance change is relatively small although the real-scenario code adds many elements is that the cost of method calls of non-built-in types and the use of Python generators. For example,
for the code of the 2nd row of Table~\ref{tab:rq3_example}, the \textsf{``group.generate\_dimino()''} returns a generator object, each time it will pause the funtion and later continue from the successive calls. Besides, the  
\textsf{``gen''} and \textsf{``el''} are Permutation classes from sympy libary, the \textsf{``$\wedge$''} is self-implemented. Their costs are larger than the cost
of \textsf{``add''} method of list.

%https://stackoverflow.com/questions/52542742/why-is-this-loop-faster-than-a-dictionary-comprehension-for-creating-a-dictionar
%%在新的版本中更新成了predict所以dict comprehension的performance improvement 可能更大一些
\noindent\textbf{Dict comprehension}.
The reason that the performance improvement of dict comprehension (maximum is 1.2 when code is in the local cope) is significantly smaller than that of list comprehension and set comprehension is that the non-idiomatic code of dict comprehension does not need to execute the instructions of function calls. The instruction of storing key-value pairs is \textsf{``STORE\_SUBSCR''} achieve the same thing as \textsf{``MAP\_ADD''} but doesn't have to load that the dictionary variable each time.

The reason of performance regression is the extra cost of instructions of dictcomp function call of idiomatic code. Since the difference of storing key-value pairs between idiomatic code and non-idiomatic code is small, the code of dict comprehension needs to add few elements to make up for the cost of dictcomp function call. The reason also is that the percentage of unchanged performance of dict comprehension is larger than of list comprehension and set comprehension.

%https://docs.python.org/3/reference/datamodel.html
The reason of performance change is relatively small although the real-scenario code adds many elements is the extra cost 
except for storing key-value pairs each iteration such as attribute accesses and function calls. For example, for the code in the 3rd row of Table~\ref{tab:rq3_example}, the \textsf{``v.\_\_self\_\_''} is a attribute access, \textsf{``v''} is the built-in method append of list object, the attribute access returns the list object. Generally, the cost of built-in methods is smaller than the non-built-in methods. Therefore, for the dict comprehension, if there is extra cost 
except for storing key-value pairs each iteration, the idiomatic refactorings may have little effect on the performance change. 




\noindent\textbf{Chain comparison}. The reason of performance improvement of idiomatic refactorings of the global scope is that the cost of loading global variables (\textsf{``LOAD\_NAME''}) of non-idiomatic code is larger than the cost of creating a reference to a comparator (\textsf{``DUP\_TOP''}) and reference shuffling (\textsf{``ROT\_THREE''}) of idiomatic code. For example, the \textsf{``a<b and b<c''} code has four variables:  \textsf{``a, b, b, c''}, so it needs to execute \textsf{``LOAD\_NAME''} instructions four times. Its corresponding idiomatic code is \textsf{``a<b<c''}. Although the idiomatic code only need to execute the \textsf{``LOAD\_NAME''} instruction three times, it needs to creating a reference to the \textsf{``b''} (\textsf{``DUP\_TOP''}) and then shove it two places down in the stack (\textsf{``ROT\_THREE''}) to get it out of the way.%https://stackoverflow.com/questions/48375753/why-are-chained-operator-expressions-slower-than-their-expanded-equivalent

The reason of performance improvement of idiomatic refactorings of the local scope in the experimental code is that the cost of loading local variables (\textsf{``LOAD\_FAST''}) is less than the cost of \textsf{``DUP\_TOP''} and \textsf{``ROT\_THREE''} instructions of idiomatic code. 

The reason of performance improvement of idiomatic refactorings of the local scope in the field code is that the chained comparators are generally attribute accesses or function calls. The cost of their instructions is larger than the cost of \textsf{``DUP\_TOP''} and \textsf{``ROT\_THREE''} instructions.  

\noindent\textbf{Truth value test}. The reason of performance improvement of idiomatic refactorings is the idiomatic code reduces the instruction cost of a comparator loading and comparison operations. If the comparator is a function call (e.g., \textsf{``Fraction(0,1)''} and \textsf{``dict()''}) instead of basic data types, the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants, so the performance improvement is greater. %the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants.The greater performance improvement of idiomatic refactorings with function call comparator (e.g., \textsf{``Fraction(0,1)''} and \textsf{``dict()''}) instead of basic data types because the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants.%  instruction rather than instructions of loading variables or constants, the differences in performance change of idiomatic refactorings will be greater, so the performance improvement will be greater. 

The reason of performance change of \textsf{``not object''} and \textsf{`object''} idiomatic codes have no difference is that their instructions are to test the top item of the stack is true or not. Specifically, the instruction \textsf{`object''} of test node is  \textsf{``POP\_JUMP\_IF\_FALSE''}, and for the \textsf{``not object''}, Python interpreter will automatically compiles it \textsf{``POP\_JUMP\_IF\_TRUE''} and does not need to execute extra instructions. Therefore, although the comparison operators \textsf{``==''} and \textsf{``!=''} have different number of tokens, their performance changes are basically the same.

%https://github.com/hemildesai/numpy/blob/6fbbadb676dfa7cee56be3bd17b92bde661f8869/numpy/core/numeric.py#L363-L372 built-in method ``__nonzero__()`` (renamed ``__bool__()`` in python3.x
%https://github.com/lxml/lxml/blob/c742576c105f40fc8b754fcae56fee4aa35840a3/src/lxml/etree.pyx#L2500-L2507
The reason of performance change of idiomatic refactorings in the field code is larger than 10 or less than 1 is whether the \textsf{``\_\_bool\_\_''} method of the class of the comparator is implemented effectively. When testing an object for truth value, it will execute \textsf{``POP\_JUMP\_IF\_TRUE''} or \textsf{``POP\_JUMP\_IF\_FALSE''} instructions. Then the idiomatic code will automatically call \textsf{``\_\_bool\_\_''} method in the process. Therefore, the truth value test for the classes of numpy library is generally greater than that of idiomatic refactorings in experimental code. However, the truth value test for the the classes of lxml library generally leads to the performance regression. And we find that the developers may improve the \textsf{``\_\_bool\_\_''} method because a warning is output when the code is executed: the behavior of \textsf{``\_\_bool\_\_''} method will change in future versions.


\noindent\textbf{Loop Else}. The reason of performance improvement of idiomatic refactorings is that the idiomatic code reduces the instruction cost of loading and storing variables and testing for true value. For example, for the code in 7th row of Table~\ref{tab:rq3_example}, the idiomatic code reduces the cost of loading and storing the \textsf{``success\_flag''}  variable by removing the \textsf{``success\_flag = True''},  \textsf{``success\_flag = False''}, and \textsf{``if success\_flag''} statements.

The reason of unchanged performance of idiomatic refactorings is that the cost of executing instructions of body of loop node is much bigger than the cost of loading and storing a flag variable. If the body of for node takes much time than flag variable statements, the performance change is almost approximately 1. Meanwhile, regardless of whether the code body takes a little or lots of time to execute once, as the loop iterations increase, the more times statements in the loop body is executed, the more time they take up than the time of flag variable statements. Therefore, when loop iterations increases to a certain 
degree, the performance remains basically unchanged.

\noindent\textbf{Assign Multiple Targets}. The reason of performance regression of variable assignment code refactorings is that the extra cost of instructions of building a tuple for multiple values (\textsf{``BUILD\_TUPLE''}) and unpack the tuple (\textsf{``UNPACK\_SEQUENCE''} ). For example, for the code in the 8th row of Table~\ref{tab:rq3_example}, the non-idiomatic code has four assignment node but the idiomatic code only has one assignment node, so it seems that the idiomatic code may improve performance. However, the (\textsf{``=''}) has no real byte code instructions and one assignment statement consists of instructions of loading objects and storing objects. The non-idiomatic code loads one object and then stores one object each time. While the idiomatic code first loads four objects four times. For assigning values into targets correctly, idiomatic code then executes two extra instructions \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''} to put values onto the stack right-to-left. Finally, the idiomatic code stores four objects four times. Therefore, the idiomatic refactorings of assign-multiple-targets actually decrease the performance.

The reason of performance improvement of code of swapping variables in the global scope is that the cost of instructions of loading and storing global temporary variables is larger than instructions of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. However, when variables are in the local scope, the cost of instructions of loading and storing local temporary variables is generally less than of instructions of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. Particularly, when the idiomatic code is to swap two variables in the local scope, the performance improves because Python developers design an instruction \textsf{``ROT\_TWO''} to quickly swap two variables on the stack.

The reason of performance improvement of code of constant assignment code with more than about 8 constants is that the idiomatic code directly loads all constants once as a tuple (\textsf{``LOAD\_CONST''}) and then unpacks the tuple (\textsf{``UNPACK\_SEQUENCE''}) rather than loading a constant at a time like the non-idiomatic code. When the number of constants is larger than 8, the cost of \textsf{``UNPACK\_SEQUENCE''} is generally larger than of  8 \textsf{``LOAD\_CONST''} instructions.

\noindent\textbf{Star in Function Calls}. The difference in instructions of non-idiomatic code and idiomatic code is that the non-idiomatic code needs to access elements with specified continuous indices several times (\textsf{``LOAD\_FAST/LOAD\_NAME''} and \textsf{``BINARY\_SUBSCR''}) but the idiomatic code needs to access elements once and additionally build a slice ( \textsf{``BUILD\_SLICE''} ). Therefore, when the  the number of subscript node increases to a degree, the cost of \textsf{``BUILD\_SLICE''} is less than that of instructions of accessing elements multiple times. For example, for the \textsf{``commiter[0], commiter[1]''} code in the 9th row of Table~\ref{tab:rq3_example}, there are only two subscript nodes, 
the cost is still less than of \textsf{``BUILD\_SLICE''}, so the performance decreases. 

The reason of performance change of code in the global scope is greater than of code in the local scope is that the cost of loading global variables is greater than of loading local variables. And the reason of performance change of the variable index is greater than of the constant index is that the cost of loading variables is greater than of loading constants. 

\noindent\textbf{For Multiple Targets}. The difference in bytecode instructions of idiomatic code and idiomatic code is that the body of non-idiomatic code needs to accessing elements at specified indices (\textsf{``LOAD\_CONST''} and \textsf{``BINARY\_SUBSCR''}) but the idiomatic code does not do it. Therefore, when the code unpacks all elements, the performance will improve the performance. However, if the code unpacks part of elements, each iteration the idiomatic code needs to store an extra variable, e.g., the \textsf{``*x\_len''} variable in the the last row of the Table~\ref{tab:rq3_example}, the performance will decrease.

==> result_2.tex <==
\subsection{RQ1:What Is the Peformance Impact of Idiomatic Refactoring on the laboratory dataset and field dataset?}
\subsubsection{Motivation}
Section~\ref{motivation} shows that developers are interested in whether idiomatic Python code executes faster or slower than non-idiomatic Python code. More importantly, Since there is currently no systematic and complete study, developers are still unclear about the performance impact of idiomatic code refactoring. Therefore, this research question answers whether the impact of idiomatic Python code refactoring on performance is improved, reduced, or almost no effect.
\subsubsection{Approach}
XXXXXX
\subsubsection{Result}%%！！！这里或许展示auc说明下分析结果的可靠性
Figure~\ref{fig:performance_rq1} shows the distribution of performance change of nine Python idioms on the laboratory dataset and on the real-world dataset.

\begin{figure}
  \centering
  \includegraphics[width=3.4in]{./data/performance_rq1_compare_boxplot.pdf}
% \setlength{\abovecaptionskip}{-0.1cm}
    \caption{Performance change of the idiomatic refactoring on the laboratory data and the real-world data}
    
    \label{fig:performance_rq1} 
    \vspace{-0.3cm}
    %\vspace{-0.6cm}
\end{figure}
\noindent\textbf{List comprehension}. Figure~\ref{fig:performance_rq1} shows the performance change range on the laboratory data and real-word data is about 0.5$\sim$5.6 and 0.4$\sim$1.5, respectively. It indicates the significant difference between the laboratory data and real-word data. First, the performance improvement of the laboratory data (5.6) is obviously larger than of real-world dataset (1.5) although most of performance improvement of laboratory data is less than 2.8. Besides, the performance change of most of real-world dataset is above about 0.9, which indicates the idiomatic refactoring of list comprehension does not leads to significant performance regression like the lab dataset. %no major performance degradation of is larger than of m
%the performance change of most of real-word dataset is above about 0.9.  is   shows the distribution of performance change of the idiomatic refactoring on the laboratory dataset and real-word dataset for nine types of Python idioms.
%https://scikit-learn.org/stable/auto_examples/tree/plot_unveil_tree_structure.html#sphx-glr-auto-examples-tree-plot-unveil-tree-structure-py

\noindent\textbf{Set comprehension}.
Figure~\ref{fig:performance_rq1} shows the performance change range on the laboratory data and real-word data is about 0.6$\sim$4.1 and 0.6$\sim$1.3, respectively. The difference of performance change on two datasets of the set comprehension is the same as of the list comprehension. Besides, we find the maximum of performance improvement of the list comprehension is less than of the set comprehension regardless of laboratory dataset or real-world dataset. 

\noindent\textbf{Dict comprehension}.
Figure~\ref{fig:performance_rq1} shows the performance change range on the laboratory data and real-word data is about 0.8$\sim$2.2 and 0.5$\sim$1.06, respectively. The difference of performance change on two datasets of the list comprehension is the same as of the list comprehension and the set comprehension. Different from the list comprehension and the dict comprehension, the performance improvement of the dict comprehension of most of laboratory dataset or real-world dataset is significantly less than of the set comprehension and the list comprehension, which is basically less than 1.4.

\noindent\textbf{Chained comprehension}.
Figure~\ref{fig:performance_rq1} shows the performance change range on the laboratory data and real-word data is about 0.7$\sim$1.6 and 0.5$\sim$1.3, respectively. %Different from the list comprehension and the dict comprehension, the performance improvement of the dict comprehension of most of laboratory dataset or real-world dataset is significantly less than of the set comprehension and the list comprehension, which is basically less than 1.4.

\noindent\textbf{Truth value test}.
Figure~\ref{fig:performance_rq1} shows the performance change range on the laboratory data and real-word data is about 1.02$\sim$7.2 and 0.05$\sim$11.9, respectively. First, the performance change of all idiomatic refactorings on the laboratory dataset is greater than 1 but some idiomatic refactorings cause the performance improvement and some cause the performance regression on the real-world dataset. Besides, the performance change range of most of idiomatic refactorings of laboratory dataset is significantly larger than of real-world dataset. For example, the maximum of performance improvement of laboratory dataset is more than 10 and the minimum of performance regression is less than 1.   

\noindent\textbf{Loop else}.
Figure~\ref{fig:performance_rq1} shows the performance change range on the laboratory data and real-word data is about 0.98$\sim$1.9 and 0.2$\sim$1.3, respectively. It shows the idiomatic refactoring of the loop else generally does not cause the big performance change.

\noindent\textbf{Assign Multiple Targets}.
Figure~\ref{fig:performance_rq1} shows the performance change range on the laboratory data and real-word data is about 0.7$\sim$1.4 and 0.7$\sim$1.2, respectively. It shows the idiomatic refactoring of the assign multiple targets generally does not cause the big performance change.

\noindent\textbf{Star in Function Calls}.
Figure~\ref{fig:performance_rq1} shows the performance change range on the laboratory data and real-word data is about 0.5$\sim$3.2 and 0.06$\sim$1.3, respectively. The performance change range of idiomatic refactoring of laboratory data is bigger than of real-world data.

\noindent\textbf{For Multiple Targets}.
Figure~\ref{fig:performance_rq1} shows the performance change range on the laboratory data and real-word data is about 0.1$\sim$1.5 and 0.2$\sim$1.04, respectively. The performance change range of idiomatic refactoring of laboratory data is bigger than of real-world data.

\subsection{RQ2: What is the relationship between code features and the performance change?}\label{rq2}
\subsubsection{Motivation}
Section~\ref{motivation} shows that developers are interested in how much idiomatic refactorings can improve or degrade performance. In the research question, investigating the relationship between code features and performance change could help developers make better choices about how they code and which idioms to prioritize to refactor their code.
\subsubsection{Approach}
As described in Section~\ref{measurement}, we repeatedly execute each code snippet on two levels: VM invocations and iterations. To represent the performance change before and after idiomatic refactorings, we divide the total of execution time of non-idiomatic code by that of corresponding idiomatic code which indicates how much speedup idiomatic code has compared with non-idiomatic code. The code features come from Section~\ref{data}.

% https://ecoforecast.org/workshops/statistical-methods-seminar-series/#simpson
%https://www.youtube.com/watch?v=XQ1vk7wEI7c
%
%yGAM is an extension to linear and generalized linear models, where it could  so it could find a balance between predictive power and interpretability. nonlinear and non-monotonic relationships between the response variable and explanatory variables [21]Since the performance change is a continuous value, and relationships between the performance change and code features are not assumed to be linear, we construct a Generalized additive model (GAM) to analyze their relationships
To analyze the relationship between the performance change and code features, we construct a Generalized additive model (GAM)~\cite{tan2022exploratory,hastie2017generalized}. Compared to linear models, it can analyze the nonlinear and non-monotonic relationships between the response variable and explanatory variables~\cite{hastie2017generalized}. Compared to machine learning algorithms, it is more interpretable. So, it could implement a balance between predictive power and interpretability~\cite{serven2018pygam}. Similar to previous studies~\cite{hastie2017generalized}, we first log transform highly skewed performance change and numeric code features. Then, we use the variance inflation factor (VIF) to analyze the multicollinearity of the prediction variables~\cite{mansfield1982detecting}. If the VIF of two 
features is larger than 5, there is significant multicollinearity among the features, we randomly remove a feature. Finally, we build a GAM model with the feature values and performance changes provided by the package ``mgcv'' in R language. 
\subsubsection{Result}% Figure 1 shows the distribution of the maximum spread of each benchmark for the study subjects in violin plot notation. To ease visual comprehension, we have limited the y-axis to 1.00 for Java and 0.5 for Go, even though some projects have a small number of outlier benchmarks with even higher maxSpread.展示 deviance explained 
Figure~\ref{fig:distri_rq2} shows the distribution of performance change of idiomatic code refactorings for nine types of Python idioms.

\begin{figure}[tbp]
  \centering
  \includegraphics[width=3.4in]{./data/performance_rq2.pdf}%performance_rq1_list_compre.pdf
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Distribution of performance change of experimental idiomatic refactorings of nine kind Python idioms}
    
    \label{fig:distri_rq2} %\vspace{-0.3cm}
    \vspace{-0.2cm}
\end{figure}
%https://www.statology.org/interpret-prt-regression-output-r/ p-value
\noindent\textbf{List comprehension}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.5$\sim$5.6. The deviance explained of the GAM model is about 90\%, which means our model can explain the relationship between performance change and features well. Table~\ref{tab:relation_code_performance} shows the feature importance and the positive/negative relationship between performance change and features reported by GAM model. The Pr(>|t|) column represents the p-value associated with the value in the t value column; The t column represents the feature importance, where the sign of value represent the positive/negative relationship between code features and performance change, and the larger the absolute value of t, the more important the feature is. 

There are four features in the first 4 rows of the table that have a statistically significant relationship with the performance change because the p-value is less than 0.05. The two most important features num\_ele and context are interesting. The value of performance change increases as the number of added elements increases, whereas when the number of elements appended reaches a certain degree, the value of performance change remains basically the same. For context feature, the performance change of the variables of the code in the global scope is greater than the performance in the local scope. When the number of elements added is larger than 10,000 of code not in function, the biggest performance change is about 5; When the number of elements added is larger than 10,000 of code in function, the biggest performance change is about 3.
\begin{table}[tbp]
%\vspace{-0.2cm}
\caption{The relationship between code features and performance change}
  \label{tab:relation_code_performance}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l c c c} 
\hline
Feature  & Pr(>|t|)   & t &relationship\\ \hline

num\_ele & <2e-16 & 39.013 &positive\\ %\hline

context  & <2e-16   & -27.198&negative \\%\hline
num\_if    &<2e-16  & -14.478&negative\\ 
%\hline
num\_if\_else  &<2e-16 &  -9.510&negative \\ %\hline
num\_loop &0.796 &0.259&positive\\\hline
\end{tabular}
\vspace{-0.3cm}
\end{table}

\noindent\textbf{Set comprehension}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.6$\sim$4.1. The deviance explained of the GAM model is about 88\%, which means our model can explain the relationship between performance change and features well. The relationship between code features and performance derived from the GAM is the same as the results of list comprehension. When
the number of added elements is larger than 1,000 of code in the global scope, the biggest performance change is about 4;
When the number of added elements is larger than 1,000 of
code in the local scope, the biggest performance change is about 2.6.


%When #authors is small, it is negatively related to #downstream_projects, whereas when #authors reaches a certain de- gree (> 7 developers), it shows a significantly positive relationship. This may indicate that for small teams, the collaboration among team members may reduce the efficiency of developers. The rela- tionship between #dependencies and #downstream_projects is linear, and #dependencies is negatively related with #downstream_projects. Dey et al. [15] obtain the similar finding: packages having fewer packages as dependencies are likely to see an increase in downloads. However, the number of stars, age, and many SCs related factors, e.g., SC name and No.layer do not show significant relationship.

%https://stackoverflow.com/questions/52542742/why-is-this-loop-faster-than-a-dictionary-comprehension-for-creating-a-dictionar !!! 重要的解释
\noindent\textbf{Dict comprehension}.
Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.8$\sim$2.2. The deviance explained of the GAM model is about 91\%, which means our model can explain the relationship between performance change and features well. The
relationship between code features and performance derived
from the GAM is the same as the results of set comprehension and list comprehension. Compared to list comprehension and set comprehension, the performance improvement is not big. The maximum performance change in the global scope and in the local scope can reach about 2.2 and 1.2, respectively.%The maximum of performance change of code in the global scope can reach about 2 %When the number of added elements is larger than 100 of code in the global scope, the maximum of performance change can reach about 2; When the number of added elements is larger than unsure too various of code in the local scope, the biggest performance change is about 1.2.

%%0.8256 AUC indicates the performance change
\noindent\textbf{Chain comparison}.
Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.7$\sim$1.6. The deviance explained of the GAM model is about 55\%. From the result of GAM, there are two findings about the relationship between performance change and code features. The one is that the most important feature is the context. The performance change of variables in the global scope is greater than that in the local scope. The other is that the number of chained comparison comparators has no statistically significant relationship with performance change.

\noindent\textbf{Truth value test}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 1.02$\sim$7.2. The deviance explained of the GAM model is about 99.6\%. Based on results of GAM model, there are three findings about the relationship between performance change and code features. First, the node kind of operator has no statistically significant relationship with performance change. For example, for \textsf{``if a != []''} and \textsf{``if a == []''}, their corresponding idiomatic codes are \textsf{``if a''} and \textsf{``if not a''}. Although \textsf{``if not a''} has one more \textsf{``not''} than \textsf{``if a''}, their performance changes are basically the same. Second, the parent node to which the comparison node belongs has no statistically significant relationship with performance change. For example, the performance changes of idiomatic refactorings of \textsf{``if a != []''} and \textsf{``while a != []''} basically are same. Finally, the \textsf{``Fraction(0, 1), Decimal(0), range(0), dict() and set()''} comparators have a significant positive relationship with performance change. If the comparator is \textsf{``Fraction(0, 1)''}, the performance improvement can reach about 7. If the data type of the comparator is the basic data type such as int, float and string, the performance improvement is relatively small, basically less than 1.2.

\noindent\textbf{Loop Else}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.99$\sim$1.9. The deviance explained of the GAM model is about 95.1\%. From the result of the GAM, there are three findings. First, the loop iterations have statistically negative relationship with the performance change. As the number of iterations increases, the performance change decreases. Second, whether the code goes through the break statement have statistically positive relationship with the performance change. The performance change of the code path with the break statement is greater than of the code path without the break statement. Finally, the loop node kind (i.e., for and while node) has no statistically relationship with the performance change. %which are negatively and positively related to performance change. 

\noindent\textbf{Assign Multiple Targets}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.7$\sim$1.4. The deviance explained of the GAM model is about 69\%. There are three important features. First, the most important feature is whether the assignment code is to swap variables or not. The performance change of idiomatic refactorings that swap variables is greater than of code that does not swap variables. Then the performance change of code in the global scope is greater than of code in the local scope. Finally, The performance change of idiomatic refactorings of constants assignment is greater than of code of variables assignment.

\noindent\textbf{Star in Function Calls}. Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.5$\sim$3.2. The deviance explained of the GAM model is about 91\%. The top three important features are the number of the subscript node, the context and whether the index of the subscript node is constant or not. First, as the number of subscript node increases, the performance change will increase. Second, the performance change of code in the global scope is greater than of code in the local scope. Finally, the performance change of the constant index of the subscript node is less than of variable index of subscript node. 

\noindent\textbf{For Multiple Targets}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.1$\sim$6.9. The deviance explained of the GAM model is about 89\%. The top three important features are whether the code unpacks all elements at each iteration, the context and the number of the subscript node. First, the performance change of code to unpack all elements is greater than of code to unpack part elements. Second, the performance change of code in the local scope is greater than of code in the global scope. Finally, as the number of subscript node increases, the performance change will increase. 

\subsection{RQ3:What are the differences of performance between experimental code and real-scenario code?}
\subsubsection{Motivation}
Although constructing experimental code could help us have a basic understanding for performance change of the idiomatic refactoring with Python idioms, real-scenario code have more complex forms such as the use of class objects and function calls. Therefore, in the research question, we would like to understand whether real-scenario code will have different impact on performance change compared to the real-scenario code.
\subsubsection{Approach}
As describe in Section~\ref{data}, we collect XXX non-idiomatic and the corresponding idiomatic code pairs for nine Python
idioms. To find the differences of performance between experimental code and real-scenario code, we first extract  the performance changes and code features for each idiomatic refactoring. Then we compare the performance change of experimental code from ~\ref{rq2} with the performance change of real-scenario code based on values of code features to get the performance change only exist in real scenarios. 

\subsubsection{Result} Figure~\ref{fig:distri_rq3} shows the distribution of performance change of idiomatic refactoring for nine types of Python idioms.
\begin{figure}
  \centering
  \includegraphics[width=3.4in]{./data/performance_rq3.pdf}%performance_rq1_list_compre.pdf
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Distribution of performance change of idiomatic refactorings in the field of nine kind Python idioms}
    
    \label{fig:distri_rq3} %\vspace{-0.3cm}
    \vspace{-0.2cm}
\end{figure}
\begin{table*}[tbp]
%\vspace{-0.2cm}
\caption{the performance change of code examples of nine Python idioms in the field code}
  \label{tab:rq3_example}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l| l| l| c| c} 
\hline
Idiom&non-idiomatic code  & idiomatic code   & code feature &X\\ \hline

\href{https://github.com/kellyjonbrazil/jc/blob/e2f1b16cb9e920968c093bd1f371b191aa7107bf/jc/parsers/csv.py#L145-L146}{list-compre} & \begin{tabular}[c]{@{}l@{}} raw\_output=[]\\for row in reader:\\    \ \  raw\_output.append(row)\end{tabular} & \begin{tabular}[c]{@{}l@{}}raw\_output = [row \\for row in reader]\end{tabular} &num\_ele:11,766& 1.03\\ \hline
\href{https://github.com/sympy/sympy/blob/82f264c62db6382fd3545bb43f57584b0f4e27c2/sympy/combinatorics/testutil.py#L195-L197}{set-compre} & \begin{tabular}[c]{@{}l@{}} conjugates = set()\\for el in group.generate\_dimino():
\\   \ \ for gen in subgr\_gens:
\\   \ \    \ \      conjugates.add(gen $\wedge$ el)\end{tabular} & \begin{tabular}[c]{@{}l@{}}conjugates = \{gen $\wedge$ el\\ for el in group.generate\_dimino() \\for gen in subgr\_gens\}\end{tabular} &num\_ele:44& 1.008\\ \hline
\href{https://github.com/networkx/networkx/blob/7b30f1a814d6b7f1b3c4311d19c251b8098d1407/networkx/algorithms/community/quality.py#L299-L302}{dict-compre} & \begin{tabular}[c]{@{}l@{}} rv = \{\}\\for (k, v) in d.items():\\
\  \    rv[k] = v.\_\_self\_\_\end{tabular} & \begin{tabular}[c]{@{}l@{}}rv = \{k: v.\_\_self\_\_ for (k, v) in d.items()\}\end{tabular} &num\_ele:1,000& 1.004\\ \hline

\href{https://github.com/brainix/pottery/blob/c7be6f1f25c5404a460b676cc60d4e6a931f8ee7/pottery/deque.py#L56}{chain-comparison} & \begin{tabular}[c]{@{}l@{}} self.maxlen is not None and \\ current\_length >= self.maxlen\end{tabular} & \begin{tabular}[c]{@{}l@{}}None is not self.maxlen <= current\_length\end{tabular} & context: in the function& 1.3\\ \hline

\href{https://github.com/nipy/nibabel/blob/225892af18d82b9a91ab63a9d072b894588b670e/nibabel/volumeutils.py#L940}{truth-value-test} & \begin{tabular}[c]{@{}l@{}} if inter != 0:\end{tabular} & \begin{tabular}[c]{@{}l@{}}if inter:\end{tabular} &comparator:0& 11.8\\ \hline

\href{https://github.com/quantumlib/OpenFermion/blob/5ef58b507270f18627ec563a43001c404cf5e6c1/src/openfermion/measurements/fermion_partitioning.py#L276-L282}{loop-else} & \begin{tabular}[c]{@{}l@{}} success\_flag = True\\
    for divisor in range(2, num\_bins - 1):\\
    \ \     if trial\_size \% divisor == 0:\\
        \ \ \ \     success\_flag = False\\
        \ \ \ \     break\\
    if success\_flag:\\
       \ \  return trial\_size\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    for divisor in range(2, num\_bins - 1):\\
    \ \     if trial\_size \% divisor == 0:\\
        \ \ \ \     break\\
    else:\\
       \ \  return trial\_size\end{tabular} &iterations:<10& 1.3\\ \hline
       
\href{https://github.com/Erotemic/ubelt/blob/cdb6aa9dea7567ce742ee6a11d8a1ca4ac89f342/ubelt/util_cache.py#L497-L501}{assign-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
cfgstr = self.\_rectify\_cfgstr(cfgstr)\\
dpath = self.dpath\\
fname = self.fname\\
verbose = self.verbose
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    cfgstr , dpath , fname , verbose  = \\ self.\_rectify\_cfgstr(cfgstr), self.dpath,\\ self.fname, self.verbose\end{tabular} &variable assignment& 0.78\\ \hline

\href{https://github.com/presslabs/gitfs/blob/12886ec5b9c7e103bfcab0cd37a8333873382fae/gitfs/repository.py#L170}{star-in-func-call} & \begin{tabular}[c]{@{}l@{}} 
Signature(commiter[0], commiter[1])
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    Signature(*commiter[:2])\end{tabular} &num\_subscript:2& 0.87\\ \hline


\href{https://github.com/alichtman/shallow-backup/blob/d71b903dacd5eeea9d0be68ef3022817f9bac601/shallow_backup/backup.py#L81-L84}{for-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
for x in dotfiles\_mp\_in:\\
\ \     x[0]\\
\ \     x[1]
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    for  (x\_0, x\_1, *x\_len)  in dotfiles\_mp\_in:\\
\ \     x\_0\\
\ \     x\_1\end{tabular} &num\_subscript:2& 0.98\\ \hline
\end{tabular}
\vspace{-0.3cm}
\end{table*}

\noindent\textbf{List comprehension}. Figure~\ref{fig:distri_rq3} shows the performance change range is about 0.4$\sim$1.5. We find the performance improvement is relatively small, not even hit 2 although the number of elements appended to the list of code in function is more than 10,000. For example, the code(the first row of Table~\ref{tab:rq3_example}), the number of added elements is 11,766, the performance improvement is only about 1.03.

\noindent\textbf{Set comprehension}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.6$\sim$1.3. Similar to list comprehension, the performance improvement
is small. For example, the code(the 2nd row of Table II),
the number of added elements is 44, the performance
change is only about 1.008 but the performance change of experimental data could reach about 1.6 although the added elements is 10. 

\noindent\textbf{Dict comprehension}.
Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.5$\sim$1.1. Similar to list comprehension, the performance improvement
is small. For example, the code(the 3rd row of Table~\ref{tab:rq3_example}),
the number of added elements is 1,000, the performance
change is only about 1.004. 


\noindent\textbf{Chain comparison}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.5$\sim$1.3. The one difference is that the idiomatic refactorings can improve performance in the field code instead of decreasing performance in the experimental code when the variables of code are in the local scope. For example, the performance improvement is about 1.3 for the \textsf{``self.maxlen is not None and current\_length >= self.maxlen''} code in the local scope (the 4th row of Table~\ref{tab:rq3_example}). 

\noindent\textbf{Truth value test}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.1$\sim$12. There are two main differences between the performance changes of idiomatic refactorings of experimental data and real scene data. The one is that the performance improvement may bigger than 7 when the data type of the comparator is not Python built-in data types. For example, the \textsf{``inter $!=$ 0''} code (the 5th row of Table~\ref{tab:rq3_example}), the data type of \textsf{``inter''} is \textsf{``numpy.array''}, the performance change is even more than ten times. The other is that the performance may even decrease, less than 1, when the data type of the comparator is not Python built-in data types. For example, for the \href{https://github.com/searx/searx/blob/5b50d7455a719b145be5f90069026a60b480673d/searx/utils.py#L259}{\textsf{``xpath\_results $==$ []''} code}, the data type of \textsf{``xpath\_results''} is \textsf{``lxml.html.HtmlElement''}, the performance change is less than 0.2.

% remove one sample!!! 0.2
\noindent\textbf{Loop Else}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.9$\sim$1.3. There is no difference in performance change of idiomatic refactorings between the field code and the experimental code.

\noindent\textbf{Assign Multiple Targets}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.7$\sim$1.2. There is no difference in performance change of idiomatic refactorings between the field code and the experimental code.

\noindent\textbf{Star in Function Calls}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.6$\sim$1.03. There is no difference in performance change of idiomatic refactorings between the field code and the experimental code. %The maximum of performance change in the field code is relatively smaller than of performance change in the experimental code because 

\noindent\textbf{For Multiple Targets}. Figure~\ref{fig:distri_rq3} shows the performance change
range is about 0.18$\sim$1.0. There is no difference in performance change of idiomatic refactorings between the field code and the experimental code. The maximum of performance change is almost 1 because we set the code unpacks the part of elements to ensure the correctness of the code refactoring. For example, the \textsf{``*x\_len''} code represents there may be some unused elements in the the last row of the Table~\ref{tab:rq3_example}. Therefore, there is no idiomatic refactorings improve the performance.

\subsection{RQ4:What are the reasons of performance change caused by idiomatic refactorings?}
\subsubsection{Motivation}
 In the 3 previous research questions, we find that code refactoring with the same Python idiom could improve or decrease performance if the code is different. And the relationship between code features and performance change is various. Therefore, in this research question, we would like to understand the reason that different code have different effects on performance change of 
idiomatic refactoring for each Python idiom.% The findings can assist help developers practition- ers in avoiding the use of certain tests in performance assurance activities and in improving tests to serve as performance tests.
\subsubsection{Approach}
To explore the reason of performance change caused by idiomatic refactorings for each Python idiom, it is not reliable to compare the difference of source code between idiomatic code and the corresponding non-idiomatic code because Python interpreter does not directly execute the source code. When the Python code runs, source code first gets compiled into a set of instructions called bytecode. Then the bytecode is executed by the Python interpreter. Therefore, we first get the bytecode instructions of idiomatic code and the corresponding non-idiomatic code for each Python idiom with dis module~\cite{dis_python}. The dis module supports the analysis of CPython bytecode by disassembling it. Then we compare their difference of instructions to understand the impact of code features on performance.%说明为什么用字节码解释 source code 执行的过程https://legacy.python.org/workshops/1998-11/proceedings/papers/montanaro/montanaro.html，用字节码解释的方法过程 字节码每个meta的概念https://github.com/python/cpython/blob/main/Doc/library/dis.rst


% https://towardsdatascience.com/list-comprehensions-vs-for-loops-it-is-not-what-you-think-34071d4d8207
%https://stackoverflow.com/questions/58844643/why-is-my-list-comprehension-function-slower-than-my-list-appending-function-for
\subsubsection{Result}
\noindent\textbf{List comprehension}.
The reason of performance improvement is that the list comprehension replaces the instructions of function calls with an instruction \textsf{``LIST\_APPEND''} (green dotted box in Figure~\ref{fig:bytecode_list_compre}). Each iteration, the non-idiomatic code executes instructions of function call, but the corresponding idiomatic code only needs to execute the \textsf{``LIST\_APPEND''} instruction for appending elements, so as more elements are appended, the greater the performance change. When the added element exceeds a certain value, the performance change basically no longer increases, which is approximately the cost of instructions of function call divided by the cost of the \textsf{``LIST\_APPEND''} instruction.

The reason of performance regression is the extra cost of instructions of listcomp function call (red dotted box in Figure~\ref{fig:bytecode_list_compre}). Before iteration, idiomatic code needs to load and call listcomp function.

% https://blog.csdn.net/xfxf996/article/details/105391374
The reason of performance change in global scope is larger than the performance change in local scope is that the cost of \textsf{    ``LOAD\_FAST''} instruction of loading local variables is less than the cost of \textsf{``LOAD\_NAME''} instruction of loading global variables. For example, each iteration, non-idiomatic code needs to execute instructions of loading variables \textsf{``raw\_output''} and  \textsf{``row''}. When the code are in function, the variables are local variables. The instruction of loading local variables is \textsf{``LOAD\_FAST''} while the instruction of global variables is \textsf{``LOAD\_NAME''}. Since the cost of \textsf{``LOAD\_FAST''} is 
less than the cost of \textsf{``LOAD\_NAME''}, the cost of instructions of executing  \textsf{``raw\_output.append(row)''} in the local scope is less than the corresponding cost in the global scope, so the performance change of idiomatic code in the local scope is less than that of idiomatic code in the global scope.

%why generator或者非内置的object slower 有https://www.programiz.com/python-programming/generator
%https://www.programiz.com/python-programming/iterator
The reason of performance change is relatively small although the real-scenario code adds lots of elements is the cost of method calls of non-built-in types. For example, for the code of the 1st row of Table~\ref{tab:rq3_example}, the \textsf{``reader''} is a reader object from csv library. Each time self-implemented \textsf{``\_\_next\_\_()''} method is called, the cost is larger than the cost of \textsf{``append''} method of list.
\begin{figure}
  \centering
  \includegraphics[width=3.5in]{./data/rq4_bytecode.png}%performance_rq1_list_compre.pdf
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Bytecode instructions of idiomatic refactorings of list comprehension}
    
    \label{fig:bytecode_list_compre} \vspace{-0.3cm}
    %\vspace{-0.6cm}
\end{figure}

\noindent\textbf{Set comprehension}.
The reason of performance improvement is that the set comprehension replaces the instructions of function calls with an instruction \textsf{``SET\_ADD''}. Similar to list comprehension, \textsf{``SET\_ADD''} instruction of idiomatic code reduces the cost of \textsf{``add''} function call of non-idiomatic code.

The reason of performance regression is the extra cost of instructions of setcomp function call. Before iteration, idiomatic code needs to load and call setcomp function.



Similar to list comprehension, the reason of performance change in global scope is larger than the performance change in local scope is that the cost of instructions of the function call is reduced in the local scope compared to that of cost in the local scope. Therefore, the difference between \textsf{``SET\_ADD''} instruction and instructions of \textsf{``obj.add(e)''} function call.

The reason of performance change is relatively small although the real-scenario code adds many elements is that the cost of method calls of non-built-in types and the use of Python generators. For example,
for the code of the 2nd row of Table~\ref{tab:rq3_example}, the \textsf{``group.generate\_dimino()''} returns a generator object, each time it will pause the funtion and later continue from the successive calls. Besides, the  
\textsf{``gen''} and \textsf{``el''} are Permutation classes from sympy libary, the \textsf{``$\wedge$''} is self-implemented. Their costs are larger than the cost
of \textsf{``add''} method of list.

%https://stackoverflow.com/questions/52542742/why-is-this-loop-faster-than-a-dictionary-comprehension-for-creating-a-dictionar
%%在新的版本中更新成了predict所以dict comprehension的performance improvement 可能更大一些
\noindent\textbf{Dict comprehension}.
The reason that the performance improvement of dict comprehension (maximum is 1.2 when code is in the local cope) is significantly smaller than that of list comprehension and set comprehension is that the non-idiomatic code of dict comprehension does not need to execute the instructions of function calls. The instruction of storing key-value pairs is \textsf{``STORE\_SUBSCR''} achieve the same thing as \textsf{``MAP\_ADD''} but doesn't have to load that the dictionary variable each time.

The reason of performance regression is the extra cost of instructions of dictcomp function call of idiomatic code. Since the difference of storing key-value pairs between idiomatic code and non-idiomatic code is small, the code of dict comprehension needs to add few elements to make up for the cost of dictcomp function call. The reason also is that the percentage of unchanged performance of dict comprehension is larger than of list comprehension and set comprehension.

%https://docs.python.org/3/reference/datamodel.html
The reason of performance change is relatively small although the real-scenario code adds many elements is the extra cost 
except for storing key-value pairs each iteration such as attribute accesses and function calls. For example, for the code in the 3rd row of Table~\ref{tab:rq3_example}, the \textsf{``v.\_\_self\_\_''} is a attribute access, \textsf{``v''} is the built-in method append of list object, the attribute access returns the list object. Generally, the cost of built-in methods is smaller than the non-built-in methods. Therefore, for the dict comprehension, if there is extra cost 
except for storing key-value pairs each iteration, the idiomatic refactorings may have little effect on the performance change. 




\noindent\textbf{Chain comparison}. The reason of performance improvement of idiomatic refactorings of the global scope is that the cost of loading global variables (\textsf{``LOAD\_NAME''}) of non-idiomatic code is larger than the cost of creating a reference to a comparator (\textsf{``DUP\_TOP''}) and reference shuffling (\textsf{``ROT\_THREE''}) of idiomatic code. For example, the \textsf{``a<b and b<c''} code has four variables:  \textsf{``a, b, b, c''}, so it needs to execute \textsf{``LOAD\_NAME''} instructions four times. Its corresponding idiomatic code is \textsf{``a<b<c''}. Although the idiomatic code only need to execute the \textsf{``LOAD\_NAME''} instruction three times, it needs to creating a reference to the \textsf{``b''} (\textsf{``DUP\_TOP''}) and then shove it two places down in the stack (\textsf{``ROT\_THREE''}) to get it out of the way.%https://stackoverflow.com/questions/48375753/why-are-chained-operator-expressions-slower-than-their-expanded-equivalent

The reason of performance improvement of idiomatic refactorings of the local scope in the experimental code is that the cost of loading local variables (\textsf{``LOAD\_FAST''}) is less than the cost of \textsf{``DUP\_TOP''} and \textsf{``ROT\_THREE''} instructions of idiomatic code. 

The reason of performance improvement of idiomatic refactorings of the local scope in the field code is that the chained comparators are generally attribute accesses or function calls. The cost of their instructions is larger than the cost of \textsf{``DUP\_TOP''} and \textsf{``ROT\_THREE''} instructions.  

\noindent\textbf{Truth value test}. The reason of performance improvement of idiomatic refactorings is the idiomatic code reduces the instruction cost of a comparator loading and comparison operations. If the comparator is a function call (e.g., \textsf{``Fraction(0,1)''} and \textsf{``dict()''}) instead of basic data types, the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants, so the performance improvement is greater. %the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants.The greater performance improvement of idiomatic refactorings with function call comparator (e.g., \textsf{``Fraction(0,1)''} and \textsf{``dict()''}) instead of basic data types because the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants.%  instruction rather than instructions of loading variables or constants, the differences in performance change of idiomatic refactorings will be greater, so the performance improvement will be greater. 

The reason of performance change of \textsf{``not object''} and \textsf{`object''} idiomatic codes have no difference is that their instructions are to test the top item of the stack is true or not. Specifically, the instruction \textsf{`object''} of test node is  \textsf{``POP\_JUMP\_IF\_FALSE''}, and for the \textsf{``not object''}, Python interpreter will automatically compiles it \textsf{``POP\_JUMP\_IF\_TRUE''} and does not need to execute extra instructions. Therefore, although the comparison operators \textsf{``==''} and \textsf{``!=''} have different number of tokens, their performance changes are basically the same.

%https://github.com/hemildesai/numpy/blob/6fbbadb676dfa7cee56be3bd17b92bde661f8869/numpy/core/numeric.py#L363-L372 built-in method ``__nonzero__()`` (renamed ``__bool__()`` in python3.x
%https://github.com/lxml/lxml/blob/c742576c105f40fc8b754fcae56fee4aa35840a3/src/lxml/etree.pyx#L2500-L2507
The reason of performance change of idiomatic refactorings in the field code is larger than 10 or less than 1 is whether the \textsf{``\_\_bool\_\_''} method of the class of the comparator is implemented effectively. When testing an object for truth value, it will execute \textsf{``POP\_JUMP\_IF\_TRUE''} or \textsf{``POP\_JUMP\_IF\_FALSE''} instructions. Then the idiomatic code will automatically call \textsf{``\_\_bool\_\_''} method in the process. Therefore, the truth value test for the classes of numpy library is generally greater than that of idiomatic refactorings in experimental code. However, the truth value test for the the classes of lxml library generally leads to the performance regression. And we find that the developers may improve the \textsf{``\_\_bool\_\_''} method because a warning is output when the code is executed: the behavior of \textsf{``\_\_bool\_\_''} method will change in future versions.


\noindent\textbf{Loop Else}. The reason of performance improvement of idiomatic refactorings is that the idiomatic code reduces the instruction cost of loading and storing variables and testing for true value. For example, for the code in 7th row of Table~\ref{tab:rq3_example}, the idiomatic code reduces the cost of loading and storing the \textsf{``success\_flag''}  variable by removing the \textsf{``success\_flag = True''},  \textsf{``success\_flag = False''}, and \textsf{``if success\_flag''} statements.

The reason of unchanged performance of idiomatic refactorings is that the cost of executing instructions of body of loop node is much bigger than the cost of loading and storing a flag variable. If the body of for node takes much time than flag variable statements, the performance change is almost approximately 1. Meanwhile, regardless of whether the code body takes a little or lots of time to execute once, as the loop iterations increase, the more times statements in the loop body is executed, the more time they take up than the time of flag variable statements. Therefore, when loop iterations increases to a certain 
degree, the performance remains basically unchanged.

\noindent\textbf{Assign Multiple Targets}. The reason of performance regression of variable assignment code refactorings is that the extra cost of instructions of building a tuple for multiple values (\textsf{``BUILD\_TUPLE''}) and unpack the tuple (\textsf{``UNPACK\_SEQUENCE''} ). For example, for the code in the 8th row of Table~\ref{tab:rq3_example}, the non-idiomatic code has four assignment node but the idiomatic code only has one assignment node, so it seems that the idiomatic code may improve performance. However, the (\textsf{``=''}) has no real byte code instructions and one assignment statement consists of instructions of loading objects and storing objects. The non-idiomatic code loads one object and then stores one object each time. While the idiomatic code first loads four objects four times. For assigning values into targets correctly, idiomatic code then executes two extra instructions \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''} to put values onto the stack right-to-left. Finally, the idiomatic code stores four objects four times. Therefore, the idiomatic refactorings of assign-multiple-targets actually decrease the performance.

The reason of performance improvement of code of swapping variables in the global scope is that the cost of instructions of loading and storing global temporary variables is larger than instructions of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. However, when variables are in the local scope, the cost of instructions of loading and storing local temporary variables is generally less than of instructions of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. Particularly, when the idiomatic code is to swap two variables in the local scope, the performance improves because Python developers design an instruction \textsf{``ROT\_TWO''} to quickly swap two variables on the stack.

The reason of performance improvement of code of constant assignment code with more than about 8 constants is that the idiomatic code directly loads all constants once as a tuple (\textsf{``LOAD\_CONST''}) and then unpacks the tuple (\textsf{``UNPACK\_SEQUENCE''}) rather than loading a constant at a time like the non-idiomatic code. When the number of constants is larger than 8, the cost of \textsf{``UNPACK\_SEQUENCE''} is generally larger than of  8 \textsf{``LOAD\_CONST''} instructions.

\noindent\textbf{Star in Function Calls}. The difference in instructions of non-idiomatic code and idiomatic code is that the non-idiomatic code needs to access elements with specified continuous indices several times (\textsf{``LOAD\_FAST/LOAD\_NAME''} and \textsf{``BINARY\_SUBSCR''}) but the idiomatic code needs to access elements once and additionally build a slice ( \textsf{``BUILD\_SLICE''} ). Therefore, when the  the number of subscript node increases to a degree, the cost of \textsf{``BUILD\_SLICE''} is less than that of instructions of accessing elements multiple times. For example, for the \textsf{``commiter[0], commiter[1]''} code in the 9th row of Table~\ref{tab:rq3_example}, there are only two subscript nodes, 
the cost is still less than of \textsf{``BUILD\_SLICE''}, so the performance decreases. 

The reason of performance change of code in the global scope is greater than of code in the local scope is that the cost of loading global variables is greater than of loading local variables. And the reason of performance change of the variable index is greater than of the constant index is that the cost of loading variables is greater than of loading constants. 

\noindent\textbf{For Multiple Targets}. The difference in bytecode instructions of idiomatic code and idiomatic code is that the body of non-idiomatic code needs to accessing elements at specified indices (\textsf{``LOAD\_CONST''} and \textsf{``BINARY\_SUBSCR''}) but the idiomatic code does not do it. Therefore, when the code unpacks all elements, the performance will improve the performance. However, if the code unpacks part of elements, each iteration the idiomatic code needs to store an extra variable, e.g., the \textsf{``*x\_len''} variable in the the last row of the Table~\ref{tab:rq3_example}, the performance will decrease.

==> result_3.tex <==
\subsection{RQ1:What Is the Peformance Impact of Idiomatic Refactoring on the laboratory dataset and field dataset?}
\subsubsection{Motivation}
Section~\ref{motivation} shows that developers are interested in whether idiomatic Python code executes faster or slower than non-idiomatic Python code. Furthermore, we find there are some arguments on different code. Therefore, this research question answers the performance impact of the idiomatic refactoring on the laboratory dataset and field dataset.% 
%之后再改
\subsubsection{Approach}
As described in Section~\ref{data}, we collect XXX non-idiomatic and the corresponding idiomatic code pairs for nine Python idioms, and then we compute the performance change on the two datasets based on the approach of Section~\ref{measurement}. For each Python idiom, we analyze what kind of performance impact on the two datasets, and compare how well the performance change of the laboratory dataset align with the performance change of real-world dataset from the upper bond, lower bond and the range of performance change. %the differenceschange () % 先计算两组数据的数值，然后XXX If the performance change is larger than 1, the performance improves (i.e., performance improvement). If the performance change is less than 1, the performance decreases (i.e., performance regression). Otherwise, the performance basically is unchanged (i.e., performance unchanged). 

\subsubsection{Result}
Figure~\ref{fig:performance_rq1} shows the distribution of performance change of nine Python idioms on the laboratory dataset and on the real-world dataset. The gray circle represents the outliers of dataset. The upper and lower whiskers represent the maximum and the minimum of performance change of dataset excluding the outliers. The range of the box represents 25th to the 75th percentile of dataset.

\begin{figure}
  \centering
  \includegraphics[width=3.4in]{./data/performance_rq1_compare_boxplot.pdf}
% \setlength{\abovecaptionskip}{-0.1cm}
    \caption{Performance change of the idiomatic refactoring on the laboratory data and the real-world data}
    
    \label{fig:performance_rq1} 
    \vspace{-0.3cm}
    %\vspace{-0.6cm}
\end{figure}
All idiomatic refactorings of nine Python idioms can improve or decrease the performance among the two datasets. First, for the performance improvement, among the two datasets, there are six Python idioms (list/set/dict comprehension, star-in-function-call, for-multiple-targets and truth value test) where idiomatic refactoring can make performance changes greater than 2. However, for the remaining three Python idioms, chain-comparison, loop-else and assign-multiple-targets,  their maximums of performance improvement of all idiomatic refactorings on the two datasets are less than 2. Besides, for the performance regression, among the two datasets, there are two Python idioms (for-multiple-targets and truth-value-test) where some idiomatic refactorings make the performance change less than 0.5. For the six Python idioms (list/set/dict-comprehension, chain-comparison, assign-multiple-targets and star-in-func-call), their performance changes of idiomatic refactoring basically are above 0.5. The performance change of idiomatic refactorings of loop-else basically is greater than 0.9.

There are three differences in the maximum performance change, minimum performance change and the range of performance change on the two datasets.

First, the maximum performance change (11.9) of the truth-value-test of the real-world dataset is larger than of laboratory dataset (7.2). While the maximum of performance improvement of remaining eight Python idioms are less than of real-world dataset.%have the opposite results from the truth-value-test. 

Second, for the difference in minimum performance change on the two datasets, the two Python idioms (star-in-fun-call and for-multiple-targets) of the real-world dataset is greater than of laboratory dataset. The remaining six Python idioms have the opposite results to the results of star-in-fun-call and for-multiple-targets. Particularly, the minimum performance change of the truth-value-test is larger than 1 on the laboratory dataset but the minimum of performance change on the real-world dataset only is 0.05.

Finally, for the difference of the performance change variation of most of idiomatic refactorings for each Python idiom on the two datasets, we could observe the upper and lower whiskers of the Figure~\ref{fig:performance_rq1}. The variation of performance change of laboratory dataset is smaller than that of real-world dataset for the truth-value test idiom. For example, the range of performance change of list comprehension is about 1.02$\sim$2.3, but the performance change of real-world dataset is about 0.05$\sim$11.9. The variation of performance change of laboratory dataset intersects with that of real-world dataset for the dict comprehension, but the performance change of most of idiomatic refactorings of the real-world dataset is less than of laboratory dataset. The variation of performance change of laboratory dataset is relatively greater than that of real-world dataset for the remaining seven Python idioms. For example, for the list comprehension, the ranges of performance change on the laboratory dataset and the real-world dataset are about 0.5$\sim$2.8 and 0.7$\sim$1.2 respectively. 

\subsection{RQ2: How well the symptom features can explain the performance change of idiomatic refactorings on the laboratory dataset and the real-world dataset?}\label{rq2}
\subsubsection{Motivation}
Section~\ref{motivation} shows that developers are interested in how much idiomatic refactorings can improve or degrade performance. In the research question, investigating the relationship between code features and performance change could help developers make better choices about how they code, which idioms to prioritize to refactor their code, and how they optimize their code to make Python idioms faster.
\subsubsection{Approach}

% https://ecoforecast.org/workshops/statistical-methods-seminar-series/#simpson
%https://www.youtube.com/watch?v=XQ1vk7wEI7c
%
%yGAM is an extension to linear and generalized linear models, where it could  so it could find a balance between predictive power and interpretability. nonlinear and non-monotonic relationships between the response variable and explanatory variables [21]Since the performance change is a continuous value, and relationships between the performance change and code features are not assumed to be linear, we construct a Generalized additive model (GAM) to analyze their relationships
To analyze the relationship between the performance change and code features, we construct a Generalized additive model (GAM)~\cite{tan2022exploratory,hastie2017generalized}. The code features come from Section~\ref{data} and the performance changes come from Section~\ref{measurement}. Compared to linear models, it can analyze the nonlinear and non-monotonic relationships between the response variable and explanatory variables~\cite{hastie2017generalized}. Compared to machine learning algorithms, it is more interpretable. So, it could implement a balance between predictive power and interpretability~\cite{serven2018pygam}. Similar to previous studies~\cite{hastie2017generalized}, we first log transform highly skewed performance change and numeric code features. Then, we use the variance inflation factor (VIF) to analyze the multicollinearity of the prediction variables~\cite{mansfield1982detecting}. If the VIF of two 
features is larger than 5, there is significant multicollinearity among the features, we randomly remove a feature. Finally, we build a GAM model with the feature values and performance changes provided by the package ``mgcv'' in R language. 
\subsubsection{Result}% Figure 1 shows the distribution of the maximum spread of each benchmark for the study subjects in violin plot notation. To ease visual comprehension, we have limited the y-axis to 1.00 for Java and 0.5 for Go, even though some projects have a small number of outlier benchmarks with even higher maxSpread.展示 deviance explained 
\begin{table}[tbp]
%\vspace{-0.2cm}
\caption{The interpretability of symptom features to performance change on the laboratory dataset and on the real-world dataset}
  \label{tab:relation_code_performance}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l |c | c｜c } 
\hline
\multirow{2}{*}{Idiom}                                    & \multicolumn{2}{c|}{Deviance Explained(\%)} & \multirow{2}{*}{Important features}\\
\cline{2-3} &lab-data & \multicolumn{1}{c|}{field-data}\\\hline

List-Comprehension  & 90.3 & \multicolumn{1}{c|}{28.3} & \begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}*\\
\texttt{scope}
\end{tabular}
\\ 
\hline
Set-Comprehension  & 88.1 &  \multicolumn{1}{c|}{8.8} &\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}*\\
\texttt{scope}
\end{tabular}\\
\hline%1292
Dict-Comprehension  & 91.2   & \multicolumn{1}{c|}{29.3}&\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}*\\
\texttt{scope}
\end{tabular}\\ 
\hline

Chain-Comparison   & 55.4  & \multicolumn{1}{c|}{19.8} &\texttt{scope}*\\ 
\hline
Truth-Value-Test   & 99.6   & \multicolumn{1}{c|}{32}&\begin{tabular}[c]{@{}l@{}}\texttt{empty\_set}*\\
\texttt{scope}
\end{tabular}
\\ 
\hline
Loop-Else    & 95.1 & \multicolumn{1}{c|}{53.4} &\texttt{size\_ele}*\\ 
\hline
Assign-Multi-Targets  & 68.6  & \multicolumn{1}{c|}{55.1}& \begin{tabular}[c]{@{}l@{}}\texttt{is\_swap}\\
\texttt{scope}\\
\texttt{is\_const}
\end{tabular}\\ 
\hline
Star-in-Func-Call  & 90.9   & \multicolumn{1}{c|}{31.9} &\begin{tabular}[c]{@{}l@{}}num\_Subscript*\\
\texttt{scope}\\
\texttt{is\_const}\end{tabular}\\ 
\hline
For-Multi-Targets & 88.3 & \multicolumn{1}{c|}{67.8}&\begin{tabular}[c]{@{}l@{}} 
\texttt{is\_total\_data}\\
\texttt{scope}\\
num\_Subscript*\\
\end{tabular}\\
\hline
\end{tabular}

{\raggedright    $*$ represents that the relationship of features with performance change of the laboratory dataset maybe inapplicable to the real-world dataset.\par}
\vspace{-0.3cm}
\end{table}

\begin{table*}[tbp]
%\vspace{-0.2cm}
\caption{the performance change of code examples of nine Python idioms in the field code}
  \label{tab:rq3_example}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l| l| l| c| c} 
\hline
Idiom&non-idiomatic code  & idiomatic code   & code feature &X\\ \hline

\href{https://github.com/kellyjonbrazil/jc/blob/e2f1b16cb9e920968c093bd1f371b191aa7107bf/jc/parsers/csv.py#L145-L146}{list-compre} & \begin{tabular}[c]{@{}l@{}} raw\_output=[]\\for row in reader:\\    \ \  raw\_output.append(row)\end{tabular} & \begin{tabular}[c]{@{}l@{}}raw\_output = [row \\for row in reader]\end{tabular} &\texttt{size\_ele}:11,766& 1.03\\ \hline
\href{https://github.com/sympy/sympy/blob/82f264c62db6382fd3545bb43f57584b0f4e27c2/sympy/combinatorics/testutil.py#L195-L197}{set-compre} & \begin{tabular}[c]{@{}l@{}} conjugates = set()\\for el in group.generate\_dimino():
\\   \ \ for gen in subgr\_gens:
\\   \ \    \ \      conjugates.add(gen $\wedge$ el)\end{tabular} & \begin{tabular}[c]{@{}l@{}}conjugates = \{gen $\wedge$ el\\ for el in group.generate\_dimino() \\for gen in subgr\_gens\}\end{tabular} &\texttt{size\_ele}:44& 1.008\\ \hline
\href{https://github.com/networkx/networkx/blob/7b30f1a814d6b7f1b3c4311d19c251b8098d1407/networkx/algorithms/community/quality.py#L299-L302}{dict-compre} & \begin{tabular}[c]{@{}l@{}} rv = \{\}\\for (k, v) in d.items():\\
\  \    rv[k] = v.\_\_self\_\_\end{tabular} & \begin{tabular}[c]{@{}l@{}}rv = \{k: v.\_\_self\_\_ for (k, v) in d.items()\}\end{tabular} &\texttt{size\_ele}:1,000& 1.004\\ \hline

\href{https://github.com/brainix/pottery/blob/c7be6f1f25c5404a460b676cc60d4e6a931f8ee7/pottery/deque.py#L56}{chain-comparison} & \begin{tabular}[c]{@{}l@{}} self.maxlen is not None and \\ current\_length >= self.maxlen\end{tabular} & \begin{tabular}[c]{@{}l@{}}None is not self.maxlen <= current\_length\end{tabular} & \texttt{scope}: in the function& 1.3\\ \hline

\href{https://github.com/nipy/nibabel/blob/225892af18d82b9a91ab63a9d072b894588b670e/nibabel/volumeutils.py#L940}{truth-value-test} & \begin{tabular}[c]{@{}l@{}} if inter != 0:\end{tabular} & \begin{tabular}[c]{@{}l@{}}if inter:\end{tabular} &comparator:0& 11.8\\ \hline

\href{https://github.com/quantumlib/OpenFermion/blob/5ef58b507270f18627ec563a43001c404cf5e6c1/src/openfermion/measurements/fermion_partitioning.py#L276-L282}{loop-else} & \begin{tabular}[c]{@{}l@{}} success\_flag = True\\
    for divisor in range(2, num\_bins - 1):\\
    \ \     if trial\_size \% divisor == 0:\\
        \ \ \ \     success\_flag = False\\
        \ \ \ \     break\\
    if success\_flag:\\
       \ \  return trial\_size\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    for divisor in range(2, num\_bins - 1):\\
    \ \     if trial\_size \% divisor == 0:\\
        \ \ \ \     break\\
    else:\\
       \ \  return trial\_size\end{tabular} &iterations:<10& 1.3\\ \hline
       
\href{https://github.com/Erotemic/ubelt/blob/cdb6aa9dea7567ce742ee6a11d8a1ca4ac89f342/ubelt/util_cache.py#L497-L501}{assign-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
cfgstr = self.\_rectify\_cfgstr(cfgstr)\\
dpath = self.dpath\\
fname = self.fname\\
verbose = self.verbose
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    cfgstr , dpath , fname , verbose  = \\ self.\_rectify\_cfgstr(cfgstr), self.dpath,\\ self.fname, self.verbose\end{tabular} &num\_assign:4& 0.78\\ \hline

\href{https://github.com/maxpumperla/elephas/blob/c474bb4f2565185dfd89fd06a8fe467fa9c64b2b/elephas/mllib/adapter.py#L13-L14}{star-in-func-call} & \begin{tabular}[c]{@{}l@{}} 
func(np\_array.shape[0], np\_array.shape[1])
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    func(*np\_array.shape[:2])\end{tabular} &num\_subscript:2& 1.004\\ \hline
\href{https://github.com/gugarosa/opytimizer/blob/f3e110cdc7fb8557d7e041737d3c9fd63f375c1e/opytimizer/visualization/surface.py#L39}{star-in-func-call} & \begin{tabular}[c]{@{}l@{}} 
func(points[0], points[1], points[2])
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
 func(*points[:3])\end{tabular} &num\_subscript:3& 0.58\\ \hline

\href{https://github.com/networkx/networkx/blob/e0c055a3524f583b60c89ea5d72a3b624212f357/networkx/algorithms/community/quality.py#L327}{for-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
for e in G.edges():\\
\ \     e[0]\\
\ \     e[1]
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    for  (e\_0, e\_1, *e\_len) in G.edges():\\
\ \     e\_0\\
\ \     e\_1\end{tabular} &num\_subscript:2& 0.9\\ \hline

\href{https://github.com/alichtman/shallow-backup/blob/d71b903dacd5eeea9d0be68ef3022817f9bac601/shallow_backup/backup.py#L81-L84}{for-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
for pacman\_option in \\pacman\_options.values():\\
\ \     pacman\_option[0]\\
\ \     pacman\_option[1]
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    for  (pacman\_option\_0, pacman\_option\_1, *pac-\\man\_option\_len)  in pacman\_options.values():\\
\ \     pacman\_option\_0\\
\ \     pacman\_option\_1\end{tabular} &num\_subscript:2& 0.33\\ \hline
\end{tabular}
\vspace{-0.3cm}
\end{table*}
%https://www.statology.org/interpret-prt-regression-output-r/ p-value
Table~\ref{tab:relation_code_performance} shows the interpretability of symptom features to performance change of idiomatic refactoring on the laboratory dataset and the real-world dataset for each Python idiom, the Deviance Explained shows how well the model could explain the relationship between the performance change and symptom features. On the laboratory dataset,  the symptom features are enough to reflect performance change on the laboratory dataset (the deviance explained is above 50\%). However, On the real-world dataset, for the six Python idioms (list/set/dict-comprehension, chain-comparison, truth-value-test and star-in-func-call), the symptom features alone cannot reflect the performance change on the real-world dataset, 
which indicates many other complex factors that affect the performance change. For the loop-else, assign-multiple-targets and for-multiple-targets, the symptom features can reflect the performance change well.
However, for the loop-else and for-multiple-targets, their differences in deviance explained are larger than 20\% on the two datasets, which reflect some idiomatic refactorings maybe influenced by other symptom features. 

%28.3 90.3
\noindent\textbf{List/Set/Dict comprehension}. For the three Python idioms on the laboratory dataset, the \texttt{size\_ele} and \texttt{scope} are the most important features. The relationship between the features and the performance change is expressed as follows:

\textsf{REL1}: The value of performance change increases as the number of added elements increases, whereas when the number of elements appended reaches a certain degree, the value of performance change remains stable. Particularly, the performance will decrease if there is no element appended to the list. 

\textsf{REL2}: For context feature, the performance change of the variables of the code in the global scope is greater than the performance in the local scope. 

% \noindent\textbf{Commonality}: The performance will decrease if there is no element appended to the list on the two datasets for the three Python idioms.

\noindent\textbf{Difference}: However, on the real-world dataset, we find the performance improvement of the laboratory dataset maybe obviously smaller than that of the real-world dataset for the three Python idioms although the number of added elements is large. 

List comprehension: On the laboratory dataset, when the the number of added elements is larger than 1,000, the performance improvement of code in the global scope and in the local scope may up to about 5 and 3, repsectively. However, on the real-world dataset, we find the performance improvement maybe not even hit 2 although the number of elements appended to the list of code in function is more than 10,000. For example, the number of added elements is 11,766, the performance improvement is only about 1.03 for the code in the 1st row of Table~\ref{tab:rq3_example}.

Set comprehension: On the laboratory dataset, when the the number of added elements is larger than 1,000, the performance improvement of code in the global scope and in the local scope may up to about 4 and 2.6, repsectively. However, on the real-world dataset, the performance improvement maybe small although the number of added elements is not small. For example, the number of added elements is 44, the performance change is only about 1.008 but the performance change of experimental data could reach about 1.6 although the number of added elements is only 10 for the code in the 2nd row of Table~\ref{tab:rq3_example}.

Dict comprehension: Compared to list comprehension and set comprehension, the performance improvement of dict comprehension is not big on the both of two datasets. For the laboratory dataset, when the the number of added elements is larger than 100, the performance improvement of code in the global scope and in the local scope may up to about 2.2 and 1.2, repsectively. However, on the real-world dataset, the performance of idiomatic code may basically unchanged although the number of elements is not small. For example, the number of added elements is 1,000, the performance change is only about 1.004 (the 3rd row of Table~\ref{tab:rq3_example}).


%%
\noindent\textbf{Chain comparison}.
On the laboratory dataset, the \texttt{scope} is the most important feature. 

\textsf{REL1}: The performance change of the idiomatic refactoring in the global scope is greater than of the idiomatic refactoring in the local scope. Specifically, the idiomatic refactoring in the global scope generally increases the performance but decreases performance in the local scope. The result is consistent with anecdotal evidence on Stackoverflow~\cite{chain_compare_slow_SO}.
%And the number of chained comparison comparators has no statistically significant relationship with performance change.

\noindent\textbf{Difference}: However, on the real-world dataset, although the idiomatic refactoring is in the local scope, the performance may improve. For example, the performance improvement is about 1.3 for the \textsf{``self.maxlen is not None and current\_length >= self.maxlen''} code in the local scope (the 4th row of Table~\ref{tab:rq3_example}).

\noindent\textbf{Truth value test}. 

\textsf{REL1}: On the laboratory dataset, the value of comparator (\textsf{``Fraction(0, 1), Decimal(0), range(0), dict() and set()''}) has a significant relationship with the performance change. For example, If the comparator is \textsf{``Fraction(0, 1)''}, the performance improvement may reach about 7. If the comparator is \textsf{``0, 0.0, `'}, the performance improvement is relatively small, basically less than 1.2. 

\textsf{REL2}: The node kind of operator has no statistically significant relationship with performance change, which is a little unintuitive. For example, for \textsf{``if a != []''} and \textsf{``if a == []''}, their corresponding idiomatic codes are \textsf{``if a''} and \textsf{``if not a''}. Although \textsf{``if not a''} has one more \textsf{``not''} than \textsf{``if a''}, their performance changes are basically the same. %Finally, the parent node to which the comparison node belongs has no statistically significant relationship with performance change. For example, the performance changes of idiomatic refactorings of \textsf{``if a != []''} and \textsf{``while a != []''} basically are same. 

\noindent\textbf{Difference}: On the real-world dataset, we find although the comparator are \textsf{``0, 0.0, `'}, the performance improvement maybe bigger than 7 or the performance regression maybe less than 0.1. For example, for the \textsf{``inter ! = 0''} code in the 5th row of Table~\ref{tab:rq3_example}), the performance change of the idiomatic refactoring is even more than ten times. For another example, for the \textsf{``xpath\_results == []''} code, the performance change of the idiomatic refactoring is less than 0.2.

\noindent\textbf{Loop Else}. 
\textsf{REL1}: On the laboratory dataset, the iterations of loop has a significant relationship with the performance change. As the number of iterations increases, the performance change gradually smaller, and finally it is basically 1. And the performance change is relatively small, the maximum of performance change is less than 2 although the iteration is less than 10 (the sixth-to-last row of Table~\ref{tab:rq3_example}).

\noindent\textbf{Difference}: On the real-world dataset, although the iterations of loop is small, the performance may basically not change. 

% Figure~\ref{fig:distri_rq2} shows the performance change range is about 0.99$\sim$1.9. The deviance explained of the GAM model is about 95.1\%. From the result of the GAM, there are three findings. First, the loop iterations have statistically negative relationship with the performance change. As the number of iterations increases, the performance change decreases. Second, whether the code goes through the break statement have statistically positive relationship with the performance change. The performance change of the code path with the break statement is greater than of the code path without the break statement. Finally, the loop node kind (i.e., for and while node) has no statistically relationship with the performance change. %which are negatively and positively related to performance change. 

\noindent\textbf{Assign Multiple Targets}.

\textsf{REL1}: The most important feature is whether the assignment code is to swap variables or not (\texttt{is\_swap}). The performance change of idiomatic refactorings that swap variables is greater than of code that does not swap variables. For example, when the variable assignment code is only to assign value instead of swapping values, the performance basically decreases. For example, 
the code has four assignment statements in the third-to-last row of Table~\ref{tab:rq3_example}, but the performance change is only 0.78.

\textsf{REL2}: The performance change of code in the global scope is greater than of code in the local scope. For example, when variable assignment code in the global scope is to swap variables, the idiomatic refactorings will improve the performance. However, when the assignment code is to swap only two variables in the local scope, the performance could improve. 

\textsf{REL3}: The performance change of idiomatic refactorings of constants assignment is greater than of code of variables assignment.

\textsf{REL4}: We find the number of assignment node has no significant relationship with the performance change, which is a bit counterintuitive. Since no matter how many assignment statements a non-idiomatic code has, the corresponding idiomatic code has only one assignment statement. It seems the more assignment statements, the greater the performance change but the performance change basically is same. 



\noindent\textbf{Star in Function Calls}. On the laboratory dataset, the top three important features are the number of the subscript node (num\_Subscript), \texttt{scope} and whether the index of the subscript node is constant or not (\texttt{is\_const}). 

\textsf{REL1}: As the number of subscript node increases, the performance change will increase. When the number of subscript node is larger than 4 at least, the performance generally improve. 

\textsf{REL2}: The performance change of code in the global scope is greater than of code in the local scope. 

\textsf{REL3}: The performance change of the constant index of the subscript node is less than of variable index of subscript node. %hen the number of subscript node is larger than 4 at least, the performance can improve.

\noindent\textbf{Difference}: Although the number of subscript node is positively correlated with performance change on the laboratory dataset, we find the number of subscript node has no significant relationship with the performance change on the real-world dataset. For example, for the code in the fourth-to-last row of Table~\ref{tab:rq3_example}, although the number of subscript node is only two, the performance change improves. However, the number of subscript node is three in the third-to-last row of Table~\ref{tab:rq3_example}, the performance change is only about 0.58.

\noindent\textbf{For Multiple Targets}.  On the laboratory dataset, the top three important features are whether the code unpacks all elements at each iteration (\texttt{is\_total\_data}), \texttt{scope} and the number of the subscript node ((num\_Subscript)). 

\textsf{REL1}: The performance change of code to unpack all elements is greater than of code to unpack part elements. And if the code fetches all elements of the iterator, the performance generally improves.

\textsf{REL2}: The performance change of code in the local scope is greater than of code in the global scope. 

\textsf{REL3}: As the number of subscript node in the body of the for node increases, the performance change will increase. 

\noindent\textbf{Difference}: On the real-world dataset, we find although the few subscript nodes used in the code may not cause the obvious performance regression (e.g., <0.5) like on the laboratory dataset. For example, the code with two subscript nodes in the last row of Table~\ref{tab:rq3_example}, the performance change is only 0.33, which is consistent with the result of the laboratory dataset. However, the performance change could be close to 1 (the second-to-last row of Table~\ref{tab:rq3_example}) on the real-world dataset.





%https://www.cnblogs.com/traditional/p/13538919.html 深度剖析Python Interpreter（if/for/exception）
%https://cloud.tencent.com/developer/article/1678615 POP_JUMP_IF_FALSE 指令解析
%https://stackoverflow.com/questions/49735639/in-python-why-is-explicit-bool-much-slower-than-implicit 
\subsection{RQ3: What are the root causes of performance change caused by idiomatic refactorings on the two datasets?}
\subsubsection{Motivation}
 In the previous two research questions, we find that code refactoring with the same Python idiom could improve or decrease performance on the two datasets. And the relationship of code features and performance change of laboratory dataset may not align with that of real-world dataset. Therefore, in this research question, we would like to understand the root causes that different code have different effects on performance change for each Python idiom on the two datasets.% The findings can assist help developers practition- ers in avoiding the use of certain tests in performance assurance activities and in improving tests to serve as performance tests.
\subsubsection{Approach}
To explore the reason of performance change caused by idiomatic refactorings for each Python idiom, it is not reliable to compare the difference of source code between idiomatic code and the corresponding non-idiomatic code because Python interpreter does not directly execute the source code. When the Python code runs, source code first gets compiled into a set of instructions called bytecode. Then the bytecode is executed by the Python interpreter. Therefore, we first get the bytecode instructions of idiomatic code and the corresponding non-idiomatic code for each Python idiom with dis module~\cite{dis_python}. Then we compare their difference of instructions to understand the impact of code features on performance.%The dis module supports the analysis of CPython bytecode by disassembling it.  说明为什么用字节码解释 source code 执行的过程https://legacy.python.org/workshops/1998-11/proceedings/papers/montanaro/montanaro.html，用字节码解释的方法过程 字节码每个meta的概念https://github.com/python/cpython/blob/main/Doc/library/dis.rst

%RQ3 root causes (in both lab and real-world setting, the change by refactoring at the byte-code level are the same, but real-world code involves ……)
% %RQs take-home message and discussion: 
% Refactoring local impact (consider only the code affected by refactoring) are the same in the lab versus real-world setting, but real-world involves many complex context, interweaving ???? which may balance off the improvement by refactoring

% https://towardsdatascience.com/list-comprehensions-vs-for-loops-it-is-not-what-you-think-34071d4d8207
%https://stackoverflow.com/questions/58844643/why-is-my-list-comprehension-function-slower-than-my-list-appending-function-for
%https://www.17tr.com/tool/term/1359708.shtml SOR
\subsubsection{Result}
\noindent\textbf{List/Set/Dict comprehension}. For the list/set comprehension, the idiomatic code replaces the instructions of calling function to append elements with a specific instruction to appending elements. For example, for the idiomatic code of list comprehension, to appending a element to the list, developers replace the instructions of loading the list and calling the append function with the \textsf{``LIST\_APPEND''} (green dotted box in Figure~\ref{fig:bytecode_list_compre}). Each iteration, the non-idiomatic code executes instructions of function call, but the corresponding idiomatic code only needs to execute the \textsf{``LIST\_APPEND''} instruction for appending elements, so as more elements are appended, the greater the performance change. When the number of added element (\texttt{size\_ele}) exceeds a certain value, the performance change basically no longer increases, which is approximately the cost of instructions of function call divided by the cost of the \textsf{``LIST\_APPEND''} instruction. 

For the dict comprehension, the idiomatic code replace the instructions of storing the key-value pair (\textsf{``STORE\_SUBSCR''}) with \textsf{``MAP\_ADD''}. The \textsf{``MAP\_ADD''} achieves the same thing as \textsf{``STORE\_SUBSCR''} but doesn't have to load that the dictionary iterator each time. Therefore, the performance improvement of dict comprehension (maximum is 1.2 when code is in the local cope) is significantly smaller than that of list/set comprehension.
%The reason of the positive relationship of \texttt{size\_ele} with the performance change is that the list/set comprehension replaces the instructions of loading the iterator and calling function with a specific instruction of appending elements. For example, for the idiomatic code of list comprehension, to appending a element to the list, developers replace the instructions of loading the list and calling the append function with the \textsf{``LIST\_APPEND''} (green dotted box in Figure~\ref{fig:bytecode_list_compre}). Each iteration, the non-idiomatic code executes instructions of function call, but the corresponding idiomatic code only needs to execute the \textsf{``LIST\_APPEND''} instruction for appending elements, so as more elements are appended, the greater the performance change. When the number of added element exceeds a certain value, the performance change basically no longer increases, which is approximately the cost of instructions of function call divided by the cost of the \textsf{``LIST\_APPEND''} instruction.

Compared to the non-idiomatic code of list/set/dict comprehension, the idiomatic code adds new instructions. The idiomatic code has instructions of the comprehension-related function call (red dotted box in Figure~\ref{fig:bytecode_list_compre}) but the non-idiomatic code does not have. Before iteration, idiomatic code needs to load and call listcomp function, but non-idiomatic code does need to. Therefore, if there is no element to appended, the performance decreases.


%why generator或者非内置的object slower 有https://www.programiz.com/python-programming/generator
%https://www.programiz.com/python-programming/iterator
\textsf{SOR for Difference}: The cost of \textsf{``FOR\_ITER''} varies with different code. Each iteration, when Python interpreter executes \textsf{``FOR\_ITER''} to get the next item of the iterator, it needs to call \textsf{``\_\_next\_\_()''} method. Therefore, if the iterator is not the Python built-in type and its cost of the self-implemented \textsf{``\_\_next\_\_()''} is large, which may balance off the improvement of list/set/dict comprehension. For example, for the code of the 1st row of Table~\ref{tab:rq3_example}, the \textsf{``reader''} is a reader object from csv library, which overloads the \textsf{``\_\_next\_\_()''} method. Since the cost of \textsf{``\_\_next\_\_()''} is larger than the cost of \textsf{``append''} method of list, the performance improvement is only 1.03.

% For one thing, each iteration, when Python interpreter executes \textsf{``FOR\_ITER''} to get the next item of the iterator , it needs to call \textsf{``\_\_next\_\_()''} method. Therefore, if the iterator is not the Python built-in type and its cost of the self-implemented \textsf{``\_\_next\_\_()''} is large, which could balance off the improvement of list/set/dict comprehension. For example, for the code of the 1st row of Table~\ref{tab:rq3_example}, the \textsf{``reader''} is a reader object from csv library, which overloads the \textsf{``\_\_next\_\_()''} method. Since the cost of \textsf{``\_\_next\_\_()''} is larger than the cost of \textsf{``append''} method of list, the performance improvement is only 1.03.

For another thing, the cost of the object of the added element varies with different code. Different code needs to append different elements to the iterator. If the cost of appended element is larger than of the function call of appending elements, the performance improvement is also small. For example, for the code of the 2nd row of Table~\ref{tab:rq3_example}, the set comprehension adds \textsf{``gen$\wedge$ el''} to the iterator. The \textsf{``gen''} and \textsf{``el''} are self-defined classes and the \textsf{``$\wedge$''} is a overload method, which leads to its cost larger than of  \textsf{``add''} function call, so the performance improvement is only 1.008.
\begin{figure}
  \centering
  \includegraphics[width=3.5in]{./data/rq4_bytecode.png}%performance_rq1_list_compre.pdf
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Bytecode instructions of idiomatic refactorings of list comprehension}
    
    \label{fig:bytecode_list_compre} \vspace{-0.3cm}
    %\vspace{-0.6cm}
\end{figure}


\noindent\textbf{Chain comparison}. The idiomatic code replace the instruction to load the comparator with instructions that create a reference to a comparator (\textsf{``DUP\_TOP''}) and reference shuffling (\textsf{``ROT\_THREE''}). If the comparator is only a variable name, when the comparator is in the local scope, the load instruction is \textsf{``LOAD\_FAST''}, and when the comparator is in the global scope, the load instruction is \textsf{``LOAD\_NAME''}. The cost of \textsf{``LOAD\_FAST''} is smaller than of \textsf{``DUP\_TOP''} and  \textsf{``ROT\_THREE''}, and the cost of \textsf{``DUP\_TOP''}  \textsf{``ROT\_THREE''} is smaller than of  \textsf{``LOAD\_NAME''}. Therefore, the performance improves when the variable is in the local scope, and the performance decreases when the variable is in the global scope. If the comparator is not a variable name but the attribute access or a function call, the cost are generally larger than of \textsf{``DUP\_TOP''} and  \textsf{``ROT\_THREE''}. Therefore, if the comparator is a complex expression such as attribute access or function call, the performance will increases although the comparator is in the local scope. For example, the chained comparator is an access attribute \textsf{``self.maxlen''} whose instructions are \textsf{``LOAD\_FAST''} and  \textsf{``LOAD\_ATTR''} (the 4th row of Table~\ref{tab:rq3_example}). The cost is larger than of \textsf{``DUP\_TOP''} and \textsf{``ROT\_THREE''}, so the performance improves, the performance change is about 1.3. 

\noindent\textbf{Truth value test}. The non-idiomatic code has the instructions of comparison operator and another comparator load, but the idiomatic code does not have. Therefore, the truth value test generally improves the performance. Besides, the cost of loading comparator varies with different comparator, the performance improvement is different. For example, when the comparator is a function call (e.g., \textsf{``Fraction(0,1)''} and \textsf{``dict()''}) instead of primitive data types (e.g., \textsf{``0''} and \textsf{``0.0''}), the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading a variable or constant, so the performance improvement that comparator is the function call is greater than that comparators are primitive data types. %the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants.The greater performance improvement of idiomatic refactorings with function call comparator (e.g., \textsf{``Fraction(0,1)''} and \textsf{``dict()''}) instead of basic data types because the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants.%  instruction rather than instructions of loading variables or constants, the differences in performance change of idiomatic refactorings will be greater, so the performance improvement will be greater. 

% The instructions of \textsf{``if not object''} and \textsf{``if object''} idiomatic codes are almost same because the corresponding instructions are \textsf{``POP\_JUMP\_IF\_FALSE''} and \textsf{``POP\_JUMP\_IF\_TRUE''}, respectively. Therefore,  although the comparison operators \textsf{``==''} and \textsf{``!=''} have no difference is that their instructions are to test the top item of the stack is true or not. Specifically, the instruction \textsf{`object''} of test node is  \textsf{``POP\_JUMP\_IF\_FALSE''}, and for the \textsf{``not object''}, Python interpreter will automatically compiles it \textsf{``POP\_JUMP\_IF\_TRUE''} and does not need to execute extra instructions. Therefore, although the comparison operators \textsf{``==''} and \textsf{``!=''} have different number of tokens, their performance changes are basically the same.

%https://github.com/hemildesai/numpy/blob/6fbbadb676dfa7cee56be3bd17b92bde661f8869/numpy/core/numeric.py#L363-L372 built-in method ``__nonzero__()`` (renamed ``__bool__()`` in python3.x
%https://github.com/lxml/lxml/blob/c742576c105f40fc8b754fcae56fee4aa35840a3/src/lxml/etree.pyx#L2500-L2507
%https://github.com/numpy/numpy/blob/4cbced22a8306d7214a4e18d12e651c034143922/doc/source/reference/arrays.ndarray.rst numpy是因为对==的重载
The cost of instruction of  testing the top item of the stack is true or not (\textsf{``POP\_JUMP\_IF\_TRUE''} or \textsf{``POP\_JUMP\_IF\_FALSE''}) varies with different code largely. When the Python interpreter execute the \textsf{``POP\_JUMP\_IF\_TRUE''}, it calls the \textsf{``\_\_bool\_\_()''} method or \textsf{``\_\_len\_\_()''} method if the object is not bool data type. Therefore, if the object is not Python built-in data type, the implementation of \textsf{``\_\_bool\_\_()''} and \textsf{``\_\_len\_\_()''} may largely impact the performance. For example, the \textsf{``inter''} belongs to array object from numpy library (the 5th row of Table~\ref{tab:rq3_example}), it define the \textsf{``\_\_bool\_\_''} method which make the performance change more than 10. For another example, \href{https://github.com/searx/searx/blob/5b50d7455a719b145be5f90069026a60b480673d/searx/utils.py#L259}{\textsf{``xpath\_results == []''}} code, the \textsf{``xpath\_results''} is \textsf{``HtmlElement''} from lxml library, it define the \textsf{``\_\_bool\_\_''} method ineffectively which make the performance change less than 0.2. And we find that the developers may improve the implementation of  \textsf{``\_\_bool\_\_''} method because its source code has a warning: the method will change in future versions.


\noindent\textbf{Loop Else}. The non-idiomatic code has the instructions of loading, storing and testing the flag variable but the idiomatic code may does not have. Therefore, the for-else could improve the performance. For example, in 7th row of Table~\ref{tab:rq3_example}, the idiomatic code reduces the cost of loading and storing the \textsf{``success\_flag''} variable by removing the \textsf{``success\_flag = True''},  \textsf{``success\_flag = False''}, and \textsf{``if success\_flag''} statements. As the iteration increases, the execution of other instructions may balance off the performance improvement, so the performance change is basically close to 1. 


\noindent\textbf{Assign Multiple Targets}. The idiomatic code generally adds instructions of building a tuple (\textsf{``BUILD\_TUPLE''}) and unpacking the sequence (\textsf{``UNPACK\_SEQUENCE''}) to put values onto the stack right-to-left. Therefore, if the idiomatic code is only to assign variables, it will execute additional instructions, which make the performance decrease. For example, for the code in the 8th row of Table~\ref{tab:rq3_example}, the non-idiomatic code has four assignment node but the idiomatic code only has one assignment node, so it seems that the idiomatic code may improve performance. However, the (\textsf{``=''}) has no real byte code instructions and one assignment statement generally consists of instructions of loading objects and storing objects. The non-idiomatic code loads one object and then stores one object each time execute one assignment statement. While the idiomatic code first loads four objects four times. For assigning values into targets correctly, idiomatic code then executes two extra instructions \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. Finally, the idiomatic code stores four objects four times. Therefore, the performance decreases, the performance change is about 0.78.%Particularly, when there are only two variables, the idiomatic code uses the \textsf{``ROT\_TWO''} instruction to complete the assignment to reduce the performance regression. 

When the assignment code is to swap variables, the idiomatic code generally replaces \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''} with loading and storing temporary objects. Therefore, the performance change of swapping variables is greater than of only assign variables. Particularly, when there are only two variables, the idiomatic code uses the \textsf{``ROT\_TWO''} instruction to complete the assignment to further improve the performance change.%Therefore, the swappuse the The reason of performance regression of variable assignment code refactorings is that the extra cost of instructions of building a tuple for multiple values (\textsf{``BUILD\_TUPLE''}) and unpack the tuple (\textsf{``UNPACK\_SEQUENCE''} ).  For example, for the code in the 8th row of Table~\ref{tab:rq3_example}, the non-idiomatic code has four assignment node but the idiomatic code only has one assignment node, so it seems that the idiomatic code may improve performance. However, the (\textsf{``=''}) has no real byte code instructions and one assignment statement consists of instructions of loading objects and storing objects. The non-idiomatic code loads one object and then stores one object each time. While the idiomatic code first loads four objects four times. For assigning values into targets correctly, idiomatic code then executes two extra instructions \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''} to put values onto the stack right-to-left. Finally, the idiomatic code stores four objects four times. Therefore, the idiomatic refactorings of assign-multiple-targets actually decrease the performance.

% The reason of performance improvement of code of swapping variables in the global scope is that the cost of instructions of loading and storing global temporary variables is larger than instructions of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. However, when variables are in the local scope, the cost of instructions of loading and storing local temporary variables is generally less than of instructions of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. Particularly, when the idiomatic code is to swap two variables in the local scope, the performance improves because Python developers design an instruction \textsf{``ROT\_TWO''} to quickly swap two variables on the stack.

When the code is to assign multiple constants, the idiomatic code replace multiple instructions to load a constant with one instruction to load multiple instructions and \textsf{``UNPACK\_SEQUENCE''}. Since the constant assignment decreases the number of loading objects, its performance change is larger than of variable assignment. For example, for the \textsf{``a, b = 2, 3''} idiomatic code, the load instruction is \textsf{``LOAD\_CONST (2,3)''}, but the corresponding non-idiomatic code has two load instructions: \textsf{``LOAD\_CONST 2''} and \textsf{``LOAD\_CONST 3''}.% The reason of performance improvement of code of constant assignment code with more than about 8 constants is that the idiomatic code directly loads all constants once as a tuple (\textsf{``LOAD\_CONST''}) and then unpacks the tuple (\textsf{``UNPACK\_SEQUENCE''}) rather than loading a constant at a time like the non-idiomatic code. When the number of constants is larger than 8, the cost of \textsf{``UNPACK\_SEQUENCE''} is generally larger than of  8 \textsf{``LOAD\_CONST''} instructions.

\noindent\textbf{Star in Function Calls}. The difference in instructions of non-idiomatic code and idiomatic code is that the non-idiomatic code replace multiple instructions to access an element with specified index (\textsf{``LOAD\_FAST''/``LOAD\_NAME''} and \textsf{``BINARY\_SUBSCR''}) with an instruction to access the element once and an instruction to build a slice (\textsf{``BUILD\_SLICE''}). First, when the code is to fetch all elements of the iterator, the idiomatic code does not need to execute the \textsf{``BUILD\_SLICE''}, so the performance improves. Second, if the code is to fetch part elements, when the number of subscript node increases to a degree (about 4), the cost of \textsf{``BUILD\_SLICE''} is less than that of instructions of accessing elements multiple times. For example, for the \textsf{``points[0], points[1], points[2]''} non-idiomatic code in the third-to-last row of Table~\ref{tab:rq3_example}, it has two more instruction sets (\textsf{``points[0], points[1]''}) than of idiomatic code, but the cost is still less than of \textsf{``BUILD\_SLICE''}, so the performance decreases. %First, when the code is to fetch all elements of the iterator, the idiomatic code does not need to execute the \textsf{``BUILD\_SLICE''}, so the performance improves. Second, 

The instruction cost of loading an object varies with different code. Therefore, the few subscript nodes could improve the performance change on the real-world dataset. For example, in the fourth-to-last row of Table~\ref{tab:rq3_example}, the \textsf{``np\_array.shape''} is a attribute access whose instructions are \textsf{``LOAD\_FAST''} and \textsf{``LOAD\_ATTR''}. The cost is larger than the cost of \textsf{``BUILD\_SLICE''}, so although there are only two subscript nodes, the performance improves.

%The reason of performance change of code in the global scope is greater than of code in the local scope is that the cost of loading global variables is greater than of loading local variables. And the reason of performance change of the variable index is greater than of the constant index is that the cost of loading variables is greater than of loading constants. 
%https://blog.csdn.net/woshaguayi/article/details/108484328
\noindent\textbf{For Multiple Targets}. The non-idiomatic code replace multiple instructions to access elements with specified index (\textsf{``BINARY\_SUBSCR''}) with a instruction to unpack a sequence and instructions of store elements of the iterator  (\textsf{``UNPACK\_EX''}/\textsf{``UNPACK\_SEQUENCE''} and \textsf{``STORE\_FAST''}/\textsf{``STORE\_NAME}). The \textsf{``UNPACK\_EX''} unpacks a more starred target that represents a list of all leftover items than of \textsf{``UNPACK\_SEQUENCE''}. Therefore, as the number of subscript node of non-idiomatic code increases, the times of \textsf{``BINARY\_SUBSCR''} is more, the cost of non-idiomatic code is larger, so performance change increases. If the code fetchs all elements of the iterator, each time the code does not unpack into a starred target, the cost of \textsf{``UNPACK\_SEQUENCE''} and \textsf{``STORE\_FAST''} is less than of (\textsf{``BINARY\_SUBSCR''}), so the performance improves. %If the to The difference in bytecode instructions of idiomatic code and idiomatic code is that the body of non-idiomatic code needs to accessing elements at specified indices (\textsf{``LOAD\_CONST''} and \textsf{``BINARY\_SUBSCR''}) but the idiomatic code does not do it. Therefore, when the code unpacks all elements, the performance will improve the performance. However, if the code unpacks part of elements, each iteration the idiomatic code needs to store an extra variable, e.g., the \textsf{``*x\_len''} variable in the the last row of the Table~\ref{tab:rq3_example}, the performance will decrease.

% The cost of \textsf{``FOR\_ITER''} varies with different code, if the 



==> result_4.tex <==
\subsection{RQ1:What Is the Peformance Impact of Idiomatic Refactoring on the laboratory dataset and field dataset?}
\subsubsection{Motivation}
Section~\ref{motivation} shows that developers are interested in whether Python idioms could improve performance or decrease performance. Furthermore, we find there are some arguments on different code. Therefore, this research question answers the performance impact of the idiomatic refactoring on the laboratory dataset and field dataset.% 
%之后再改
\subsubsection{Approach}
As described in Section~\ref{data}, we collect XXX non-idiomatic and the corresponding idiomatic code pairs for nine Python idioms, and then we compute the performance change on the two datasets based on the approach of Section~\ref{measurement}. We mainly analyze four aspects of Python idioms on two datasets: performance impact (performance improvement/regression/unchanged), the upper bond, lower bond and the range of performance change.  %the differenceschange () % 先计算两组数据的数值，然后XXX If the performance change is larger than 1, the performance improves (i.e., performance improvement). If the performance change is less than 1, the performance decreases (i.e., performance regression). Otherwise, the performance basically is unchanged (i.e., performance unchanged). 

\subsubsection{Result}
Figure~\ref{fig:performance_rq1} shows the distribution of performance change of nine Python idioms on the laboratory dataset and on the real-world dataset. The gray circle represents the outliers of dataset. The upper and lower whiskers represent the maximum and the minimum of performance change of dataset excluding the outliers. The range of the box represents 25th to the 75th percentile of dataset.

\begin{figure}
  \centering
  \includegraphics[width=3.4in]{./data/performance_rq1_compare_boxplot_new_perf_change_speedup_slowdown.pdf}%performance_rq1_compare_boxplot_new_2.pdf. rq1_perf_change_box_plot.png
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Performance change of the idiomatic refactoring on the laboratory data and the real-world data}
    
    \label{fig:performance_rq1} 
    \vspace{-0.3cm}
    %\vspace{-0.6cm}
\end{figure}
\noindent$\bullet$ \textbf{Performance impact of Python idioms on two datasets:} On the laboratory dataset, for seven Python idioms (list/set/dict-comprehension, truth-value-test, loop-else, star-in-func-call and for-multi-targets), the performance of the majority of idiomatic refactorings improves. For remaining two Python idioms (chain-comparison and assign-multi-targets), the performance of the majority of idiomatic refactorings decreases. 

On the field dataset, for the truth-value-test, the performance of the majority of idiomatic refactorings improves. For the set-comprehension and loop-else, the performance of the majority of idiomatic refactorings basically does not change. For the remaining six Python idioms, the performance of the majority of idiomatic refactorings decreases.

Therefore, the performance impact of four Python idioms (truth-value-test, chain-comparison, loop-else and assign-multi-targets) is consistent on the two datasets. For the truth-value-test, it is more likely to improve performance. For the loop-else, the performance basically unchanges or improves small. For the chain-comparison and assign-multi-targets, the performance is more likely to decrease. The remaining five Python idioms exist obvious differences in performance impact on two datasets, which indicates that their performance impacts vary largely for the different code and cannot easily inferred.

\noindent$\bullet$ \textbf{The maximum of performance improvement of Python idioms on two datasets:} On the laboratory dataset, for six Python idioms (list/set/dict-comprehension, truth-value-test, star-in-func-call and for-multi-targets), the maximum of performance improvement is basically bigger than 2 which means that the idiomatic code is 50\% faster than the corresponding non-idiomatic code. On the field dataset, only the truth-value-test makes more than 2X speed up. 

Therefore, the maximum of performance improvement of four Python idioms (truth-value-test, chain-comparison, assign-multi-targets and loop-else) is consistent on two dataset. The maximum performance improvement of truth-value-test generally can be more than 2. The maximum performance improvement of three Python idioms (chain-comparison, assign-multi-targets and loop-else) is likely to be no more than 2. For remaining five Python idioms, their maximum performance improvement is not stable.

\noindent$\bullet$ \textbf{The maximum of performance regression of Python idioms on two datasets:} On the laboratory dataset, for four Python idioms (list-comprehension, truth-value-test, star-in-fun-call and for-multi-targets), the maximum of performance regression is bigger than 2 which means that the idiomatic code is 100\% slower than the non-idiomatic code. However, on the field dataset, for three Python idioms (list-comprehension, star-in-func-call and for-multi-targets), the maximum of performance regression is bigger than 2. 

Therefore, the maximum of performance regression of eight Python idioms are consistent on the two datasets. Among the seven Python idioms, the maximum of performance regression of three Python idioms (list-comprehension, star-in-func-call and for-multi-targets) can be large (>2). For five Python idioms (set-comprehension, dict-comprehension, chain-comparison, loop-else and assign-multi-targets), the maximum of the performance regression is more likely to be no more than 2. For the truth-value-test, the maximum of the performance regression is not stable.


\noindent$\bullet$ \textbf{The range of performance change of Python idioms on two datasets:} On the laboratory dataset, the range of performance change of list-comprehension and for-multi-targets is greater than 2. For three Python idioms (chain-compare, loop-else and assign-multi-targets), the range of performance change is less than 1. For the remaining four Python idioms, the range of performance change is between 1 and 2.

On the field dataset, the range of performance change of truth-value-test and for-multi-targets is greater than 2. For the remaining seven Python idioms, the range of performance change is less than 1.

Therefore, the variation of performance change of three Python idioms (chain-compare, loop-else and assign-multi-targets) is relatively stable on two datasets, where the range of performance change is less than 1. The remaining five Python idioms is relatively unstable (the range of performance change maybe larger than 2).

% For seven Python idioms (list/set-comprehension, chain-comparison, loop-else, assign-multi-targets, star-in-func-call and for-multi-targets), the variation of performance change of laboratory dataset is greater than that of field dataset. For example, for the list comprehension, the ranges of performance change on the laboratory dataset and the field dataset are about 2X slowdown$\sim$2.8X speedup and 1.4X slowdown$\sim$1.2X speedup respectively. 

% For the truth-value-test, the variation of performance change of laboratory dataset is smaller than that of field dataset. The range of performance change of list comprehension is about 1.02X speedup$\sim$2.3X speedup, but the performance change of real-world dataset is about 20X slowdown$\sim$11.9X speedup. 

% For the dict-comprehension, the variation of performance change of laboratory dataset intersects with that of real-world dataset for the dict comprehension, but the performance change of most of idiomatic refactorings of the real-world dataset is less than of laboratory dataset.
% \textbf{Summary:}
% \emph{For nine Python idioms, on the two datasets, the performance change of chain-comparison, the loop-else and assign-multi-targets are relatively stable. The chain-comparison and assign-multi-targets are more likely to decrease performance. The loop-else has little performance impact. The performance change of remaining six Python idioms varies largely, they may increase or decrease the performance based on different code.}
% \vspace{1mm}
\noindent\fbox{\begin{minipage}{8.4cm} \emph{For nine Python idioms, on the two datasets, the performance change of chain-comparison, the loop-else and assign-multi-targets are relatively small. The chain-comparison and assign-multi-targets are more likely to decrease performance. The loop-else has little performance impact. The performance change of remaining six Python idioms vary largely, they may increase or decrease the performance based on different code.} \end{minipage}}

% First, for the laboratory dataset, the upper bond of performance change 

% First, the maximum performance change (11.9) of the truth-value-test of the real-world dataset is larger than of laboratory dataset (7.2). While the maximum of performance improvement of remaining eight Python idioms are less than of real-world dataset.

% All idiomatic refactorings of nine Python idioms can improve or decrease the performance among the two datasets. First, for the performance improvement, among the two datasets, there are six Python idioms (list/set/dict comprehension, star-in-function-call, for-multiple-targets and truth value test) where idiomatic refactoring can make performance changes greater than 2. However, for the remaining three Python idioms, chain-comparison, loop-else and assign-multiple-targets,  their maximums of performance improvement of all idiomatic refactorings on the two datasets are less than 2. Besides, for the performance regression, among the two datasets, there are two Python idioms (for-multiple-targets and truth-value-test) where some idiomatic refactorings make the performance change less than 0.5. For the six Python idioms (list/set/dict-comprehension, chain-comparison, assign-multiple-targets and star-in-func-call), their performance changes of idiomatic refactoring basically are above 0.5. The performance change of idiomatic refactorings of loop-else basically is greater than 0.9.

% There are three differences in the maximum performance change, minimum performance change and the range of performance change on the two datasets.

% First, the maximum performance change (11.9) of the truth-value-test of the real-world dataset is larger than of laboratory dataset (7.2). While the maximum of performance improvement of remaining eight Python idioms are less than of real-world dataset.%have the opposite results from the truth-value-test. 

% Second, for the difference in minimum performance change on the two datasets, the two Python idioms (star-in-fun-call and for-multiple-targets) of the real-world dataset is greater than of laboratory dataset. The remaining six Python idioms have the opposite results to the results of star-in-fun-call and for-multiple-targets. Particularly, the minimum performance change of the truth-value-test is larger than 1 on the laboratory dataset but the minimum of performance change on the real-world dataset only is 0.05.

% Finally, for the difference of the performance change variation of most of idiomatic refactorings for each Python idiom on the two datasets, we could observe the upper and lower whiskers of the Figure~\ref{fig:performance_rq1}. The variation of performance change of laboratory dataset is smaller than that of real-world dataset for the truth-value test idiom. For example, the range of performance change of list comprehension is about 1.02$\sim$2.3, but the performance change of real-world dataset is about 0.05$\sim$11.9. The variation of performance change of laboratory dataset intersects with that of real-world dataset for the dict comprehension, but the performance change of most of idiomatic refactorings of the real-world dataset is less than of laboratory dataset. The variation of performance change of laboratory dataset is relatively greater than that of real-world dataset for the remaining seven Python idioms. For example, for the list comprehension, the ranges of performance change on the laboratory dataset and the real-world dataset are about 0.5$\sim$2.8 and 0.7$\sim$1.2 respectively. 

\subsection{RQ2: What features are related to the performance change on two datasets?}\label{rq2}%WHAT FACTORS AND PROBLEMS ARE RELATED TO THE EFFECTIVENESS OF GFIS? How well the symptom features can explain the performance change of idiomatic refactorings on the laboratory dataset and the real-world dataset
\subsubsection{Motivation}
Section~\ref{sec:motivation} shows that developers are interested in how much idiomatic refactorings can improve or degrade performance. In the research question, investigating the relationship between code features and performance change could help developers use Python idioms better.% and make better choices about how they code, which idioms to prioritize to refactor their code, and how they optimize their code to make Python idioms faster.
\subsubsection{Approach}
%deviance explained
%https://stats.stackexchange.com/questions/519904/how-to-calculate-the-percentage-deviance-explained-wiith-glm-nb
%The answer is your first one (i.e., 2.01). Anyone can easily calculate percent deviance explained of a model by the following codes: 100*with(summary(model), 1 - deviance/null.deviance)
%%Mixed Effects Models and Extensions in Ecology with R---
%We do not have an R2 in GLM models, but the closest we can get is the explained deviance, which is calculated as. So the explanatory variable distance to the park explains 63.51% of the variation in road kills. Dobson (2002) called this proportional increase in explained deviance the pseudo R2--并且介绍了deviance explained的详细计算方法
%https://stats.stackexchange.com/questions/100238/what-is-a-relevant-level-for-percentage-deviance-explained-in-a-glm , % of deviance explained is an effect size measure. Such a measure is not either significant or not sig; it may be important or not important. Unfortunately, any guidelines as to how big a % is how important is going to be context dependent.
% The percentage in the fourth column (shown in parentheses) is the ratio of R2(met. var.) and R2. values between 0.41 and 0.60 indicate that the model explains most of the variation, although considerable variation remains unaccounted for. The percenta-----Using a generalized additive model to quantify the influence of local meteorology on air quality in Zagreb---也包含了VIF
%The proportion of variance explained by the model was 50.0%. The order of importance of the predictors in explaining D. serra recruitment, inferred from the AIC statistics in the stepwise model, Investigating biotic and abiotic factors affecting the recruitment of an intertidal clam on an exposed sandy beach using a generalized additive mode D.S. Schoemana,*, A.J. Richardsonb,1
%https://www.researchgate.net/profile/Ivan-Mateo-2/publication/281939856_A_Comparison_of_Statistical_Methods_to_Standardize_Catch-Per-Unit-Effort_of_the_Alaska_Longline_Sablefish_Fishery/links/55ff47d408aec948c4f9b136/A-Comparison-of-Statistical-Methods-to-Standardize-Catch-Per-Unit-Effort-of-the-Alaska-Longline-Sablefish-Fishery.pdf
% explained deviance is an interpretable measure of the strength of the association. The deviance explained by each variable modelled separately can be contrasted with the total deviance explained by a model that includes all the variables. Thus the proportion of the explainable deviance attributable to each driver alone can be extracted and compared against the total explainable devianc-----Drivers of deforestation in the basin of the Usumacinta River: Inference on process from pattern analysis using generalised additive models
% To assess how well the models fitted the data, percent of deviance explained was used. Percent deviance explained (pseudo-R2) was calculated with the formula 1-(residual deviance/total deviance). To assess the relative importance of different explanatory variables in GLM and GAM models, relative variable importance was calculated by examining changes in improvement of AIC by examining the addition of one variable at a time (CPUE~Year+ βX1). We used this approach because the relative importance of explanatory variables to the model fit can change based on the order the variables are entered into the model. In BRT models, the relative influence of explanatory variables was calculated by how many times that variable was selected for splitting and averaged over all trees compared to the squared improvement to the model fit (Elith et al. 2008). Then, the contribution of each variable is scaled to a total of 100.
%https://bookdown.org/egarpor/PM-UC3M/glm-deviance.html
%https://rdrr.io/cran/modEvA/man/Dsquared.html 
%https://modtools.wordpress.com/2013/08/14/dsquared/
%Linear models come with an R-squared value that measures the proportion of variation that the model accounts for. The R-squared is provided with summary(model) in R. For generalized linear models (GLMs), the equivalent is the amount of deviance accounted for (D-squared; Guisan & Zimmermann 2000). The Dsquared function, now included in the modEvA package (Barbosa et al. 2014), calculates it. There is also an option to calculate the adjusted D-squared, which takes into account the number of observations and the number of model parameters, thus allowing direct comparison among different models (Weisberg 1980, Guisan & Zimmermann 2000). UPDATE: see also further measures in the new RsqGLM function.
%Guisan, A. & Zimmermann, N.E. (2000). Predictive habitat distribution models in ecology. Ecological Modelling 135: 147-186
%

%GAM How Interpretable and Trustworthy are GAMs: 这里说明了GAM的广泛使用
%https://arxiv.org/pdf/2006.06466.pdf
%Generalized Additive Models_ An Introduction with R, Second Edition

%Feature importance
%https://stats.stackexchange.com/questions/454553/what-method-does-varimp-gam-use-in-caret-package-in-r ---- It is used for a quick, somewhat imperfect but relatively well-understood way to measure statistically significance which is itself is a reasonable proxy for variable importance. One can use more sophisticated methods like from the package iml to get more detailed info. 
%https://stats.stackexchange.com/questions/401512/hard-in-calculating-predictor-s-relative-importance-for-gam
%We used “caret” package in R (Kuhn, 2008) to derive the relative variable importance for each of the six growth stages examined.----Evaluation of within-season grapevine evapotranspiration patterns and drivers using generalized additive models
%Appendix C. Measure of relative importance  -- Generalisedadditivemodellingofairpollution,trafficvolume and meteorology MagneAldrin��,IngridHobækHaff
%Measuring Variable Importance in Generalized Linear Models for Modeling Size of Loss Distributions Therefore, the traditional ANOVA method or GAM model may also be appropriate in evaluating variable importance, but subject to its own limitation. Using a generalized additive model to quantify the influence of local meteorology on air quality in Zagreb Variable importance measures are then given by t-values of the coefficients or the reciprocal of the p-value of the t-test in testing the significance of coefficients. They can also be defined using the risk relativity of each factor. Obtaining the risk relativity from GAM is similar to the GLM, discussed in the next section. As we can see from the model setting shown in Equation (3), the GAM method is more appropriate for the numerical type of variable, including the ordinal scale of the numerical factor. This is because of the imposed functionality by fj(·). However, for a categorical variable, we are facing the same problem as the one we will see in the GLM setting. If importance is measured for a factor, we must consider an approach that can summarize the estimate from the factor levels. The common characteristic of the model-based variable importance measure, including the sensitivity measure of the variable and the GAM approach, tries to capture the association between the response variable and a function or a mathematical operation of xj.  ANOVA method or GAM model may also be appropriate in evaluating variable importance, 
%F-----1. Quantifying the influence of local meteorology on air quality using generalized additive models
%John L. Pearce a, *, Jason Beringer a, Neville Nicholls a, Rob J. Hyndman b, Nigel J. Tapper
% F-----2. Using a generalized additive model to quantify the influence of local meteorology on air quality in Zagreb Andreina Belušić, Ivana Herceg-Bulić and Zvjezdana Bencetić Klaić

%Integrating physical and empirical landslide susceptibility models using generalized additive models
%AIC:step wise---Identification of hake distribution pattern and nursery grounds in the Hellenic seas by means of generalized additive models https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.706.9796&rep=rep1&type=pdf 
%step wise---In all GAMs, variable selection proceeded by a stepwise forward entry and the Akaike Information Criterion (AIC) was used to detect the relative importance of each variable in explaining variations and determine the order of those that should be included in the final model. 
%Reconciling Performance and Interpretability in Customer Churn Prediction using Ensemble Learning based on Generalized Additive Models
% Koen W. De Bock* Dirk Van den Poel† AUC-based feature importance
%https://arxiv.org/pdf/2204.09123.pdf 提供了多个gam模型的model interpretability GAM(E) CHANGER OR NOT? AN EVALUATION OF INTERPRETABLE MACHINE LEARNING MODELS BASED ON ADDITIVE MODEL CONSTRAINTS Furthermore, EBM turns out to be the best performing GAM among all interpretable approaches showing the highest prediction qualities in 6 out of 12 datasets. For the regression tasks, it even outperformed all other white-box models and could achieve the best results on 2 out 5 datasets.

%https://shap.readthedocs.io/en/latest/example_notebooks/overviews/An%20introduction%20to%20explainable%20AI%20with%20Shapley%20values.html#Explaining-an-additive-regression-model
%shap: Explaining a generalized additive regression model

% https://ecoforecast.org/workshops/statistical-methods-seminar-series/#simpson
%https://www.youtube.com/watch?v=XQ1vk7wEI7c
%
%yGAM is an extension to linear and generalized linear models, where it could  so it could find a balance between predictive power and interpretability. nonlinear and non-monotonic relationships between the response variable and explanatory variables [21]Since the performance change is a continuous value, and relationships between the performance change and code features are not assumed to be linear, we construct a Generalized additive model (GAM) to analyze their relationships

% Although Aldrin and Haff (2005) inspected colinearity based on cor- relation coefficients solely, in the present study we additionally calculated variance inflation factor (vIF) (Zuur et al., 2009). For all variables vIF values were lower than 3, and they were ranging from about 1.0 for the day of the week (DW) to 2.4 for the relative humidity. Thus, we assumed that variables are not collinear, and that a regression method could be applied.----Using a generalized additive model to quantify the influence of local meteorology on air quality in Zagreb Andreina Belušić, Ivana Herceg-Bulić and Zvjezdana Bencetić Klaić
%Mixed Effects Models and Extensions in Ecology with R-----The resulting VIF values are given in Table 16.2. As explained in Appendix A, a cut-off value of 5 or even 3 can be used to remove collinear variables; we used 3.

To analyze the relationship between the performance change and code features, we construct a Generalized additive model (GAM)~\cite{tan2022exploratory,hastie2017generalized}. The code features come from Section~\ref{data} and the performance changes come from Section~\ref{measurement}. Compared to linear models, it can analyze the nonlinear and non-monotonic relationships between features and the performance change~\cite{hastie2017generalized}. Compared to machine learning algorithms, it is more interpretable~\cite{InterpretableGAM}. So, it could implement a balance between predictive power and interpretability~\cite{serven2018pygam}. Similar to previous studies~\cite{hastie2017generalized}, we first log transform highly skewed performance change and numeric code features. We use the variance inflation factor (VIF) to analyze the multicollinearity of the prediction variables~\cite{mansfield1982detecting}. If the VIF of two features is larger than 5~\cite{JSSv032b01,tan2022exploratory,articleVIFZagreb}, there is significant multicollinearity among the features, we randomly remove a feature. Finally, we build a GAM model with the feature values and performance changes provided by the package ``mgcv'' in R language. The GAM model provide deviance explained and p-values. The deviance explained indicates the goodness-of-fit of model. If the deviance explained is closer to 1, the better the model fits the data. Since the deviance explained indicates the proportion of deviance explained by the model, previous studies generally assume that the model can explain the data well if the deviance explained is greater than 40\%~\cite{tan2022exploratory,SCHOEMAN200267,articleVIFZagreb}. The p-value for each feature tests the null hypothesis that the feature has no correlation with the performance change. If the p-value for a feature is less than 0.05, we think the feature is significant~\cite{tan2022exploratory,SCHOEMAN200267}.
\subsubsection{Result}% Figure 1 shows the distribution of the maximum spread of each benchmark for the study subjects in violin plot notation. To ease visual comprehension, we have limited the y-axis to 1.00 for Java and 0.5 for Go, even though some projects have a small number of outlier benchmarks with even higher maxSpread.展示 deviance explained 
\begin{table}[tbp]
%\vspace{-0.2cm}
\scriptsize\caption{The interpretability of symptom features to performance change on two datasets}
  \label{tab:relation_code_performance}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l |c | c｜c | c } 
\hline
\multirow{2}{*}{Idiom}                                    & \multicolumn{2}{c|}{laboratory data} & \multicolumn{2}{c}{Field data}\\
\cline{2-5} &\begin{tabular}[c]{@{}l@{}}DE (\%) \end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}important\\ features\end{tabular}}&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}DE (\%) \end{tabular}} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}l@{}}important\\ features\end{tabular}}\\\hline

\begin{tabular}[c]{@{}l@{}}List-Com\\prehension\end{tabular}}  &90.3 &\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}\\
\texttt{scope}\\
num\_If\\num\_If\_Else\end{tabular}}
& \multicolumn{1}{c|}{28.3} & \begin{tabular}[c]{@{}l@{}}-
\end{tabular}
\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Set-Comp\\rehension\end{tabular}  & 88.1&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}\\
\texttt{scope}\\
num\_For\\num\_If\\num\_If\_Else\end{tabular}} &  \multicolumn{1}{c|}{8.8} &\begin{tabular}[c]{@{}l@{}}-
\end{tabular}\\
\hline%1292
\begin{tabular}[c]{@{}l@{}}Dict-Comp\\rehension\end{tabular}  & 91.2&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}\\
\texttt{scope}\\
num\_For\\num\_If\\num\_If\_Else\end{tabular}}   & \multicolumn{1}{c|}{29.3}&\begin{tabular}[c]{@{}l@{}}-
\end{tabular}\\ 
\hline

\begin{tabular}[c]{@{}l@{}}Chain\\Comparison\end{tabular}   & 55.4&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
\texttt{scope}\\
\texttt{num\_compop}\\
\texttt{is\_true}\\\end{tabular}}   & \multicolumn{1}{c|}{19.8} &\begin{tabular}[c]{@{}l@{}}-
\end{tabular}\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Truth\\Value\\Test\end{tabular}   & 99.6&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
\texttt{scope}\\
\texttt{empty\_set}\end{tabular}}   & \multicolumn{1}{c|}{32}&\begin{tabular}[c]{@{}l@{}}-
\end{tabular}
\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Loop\\Else\end{tabular}    & 95.1&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
\texttt{size\_ele}\end{tabular}} & \multicolumn{1}{c|}{53.4} &\texttt{size\_ele}\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Assign\\Multi\\Targets\end{tabular}    & 68.6 &\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
\texttt{is\_swap}\\\texttt{scope}\\\texttt{is\_const}
\end{tabular}} & \multicolumn{1}{c|}{55.1}& \begin{tabular}[c]{@{}l@{}}num\_Assign\\
\texttt{is\_const}
\end{tabular}\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Star-in\\Func-Call\end{tabular}  & 90.9&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
num\_Subscript\\\texttt{scope}\\\texttt{is\_const}\\\texttt{has\_Subscript}\\\texttt{has\_Step}\\\texttt{has\_Upper}\\\texttt{has\_Lower}
\end{tabular}}   & \multicolumn{1}{c|}{31.9} &\begin{tabular}[c]{@{}l@{}}-\end{tabular}\\ 
\hline
\begin{tabular}[c]{@{}l@{}}For\\Multi\\Targets\end{tabular} & 88.3&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
\texttt{has\_Starred}\\
\texttt{scope}\\
num\_Subscript\\\texttt{size\_ele}
\end{tabular}}  & \multicolumn{1}{c|}{67.8}&\begin{tabular}[c]{@{}l@{}} 
num\_Subscript\\\texttt{size\_ele}
\end{tabular}\\
\hline
\end{tabular}

\vspace{-0.3cm}
\end{table}


%https://www.statology.org/interpret-prt-regression-output-r/ p-value 
%https://stats.stackexchange.com/questions/400933/which-index-is-preferred-in-gam-r-sq-or-deviance-explained use deviance explained
Table~\ref{tab:relation_code_performance} shows the deviance explained (i.e., \% column) and important features of on laboratory dataset and field dataset.

%On the laboratory dataset,  the symptom features are enough to reflect performance change on the laboratory dataset (the deviance explained is above 50\%). However, On the real-world dataset, for the six Python idioms (list/set/dict-comprehension, chain-comparison, truth-value-test and star-in-func-call), the symptom features alone cannot reflect the performance change on the real-world dataset, which indicates many other complex factors that affect the performance change. For the loop-else, assign-multiple-targets and for-multiple-targets, the symptom features can reflect the performance change well. However, for the loop-else and for-multiple-targets, their differences in deviance explained are larger than 20\% on the two datasets, which reflect some idiomatic refactorings maybe influenced by other symptom features. 

\noindent\FiveStar \textbf{The relationship between features and performance change on the laboratory dataset:} On the laboratory dataset, we find the symptom features are enough to reflect performance change well (the deviance explained is above 50\%). There are some features are significant features in all four dimensions (i.e., node, context, data and state).  The relationships between the features and the performance change are expressed as follows:

\noindent\textbf{Relationship (REL) in node}:

\textbf{REL1-num\_node}: For the list/set/dict-comprehension, we find as the numbers of For, If, If-Else nodes increase, the performance change becomes smaller. 

For the star-in-func-call and the for-multi-targets, as the number of Subscript node increases, the performance change becomes bigger.

\textbf{REL2-\texttt{node\_set}}: For the truth-value-test, the value of comparator (\textsf{``Fraction(0, 1), Decimal(0), range(0), dict() and set()''}) has a significant relationship with the performance change. For example, If the comparator is \textsf{``Fraction(0, 1)''}, the performance improvement may reach about 7. If the comparator is \textsf{``0, 0.0, `'}, the performance improvement is relatively small, basically less than 1.2. 


\textbf{REL3-\texttt{has\_node}}: For the star-in-func-call, the \texttt{has\_Subscript}, \texttt{has\_Step},  \texttt{has\_Upper} and \texttt{has\_Lower} is negatively related to the performance change. For example, for the non-idiomatic code ``\textsf{func(e\_list[0], e\_list[1])}'', if the ``\textsf{e\_list}'' has more than two elements, the corresponding idiomatic code is ``\textsf{func(*e\_list[:2])}'' that has the subscript node ``\textsf{[:2]}'' (i.e., \texttt{has\_Subscript} is 0). However, if the ``\textsf{e\_list}'' has two elements, the corresponding idiomatic code is ``\textsf{func(*e\_list)}'' that does not have the subscript node(i.e., \texttt{has\_Subscript} is 0). The performance change of the idiomatic refactoring with Subscript node is less than of without the Subscript node.%For the non-idiomatic code ``\textsf{func(e\_list[0], e\_list[1])}'', the corresponding idiomatic code is ``\textsf{func(*e\_list[:2])}'' that does not have a Lower node (i.e., \texttt{has\_Lower} is 0). The performance change of the idiomatic refactoring with Lower node is less than of without Lower node.

For the for-multi-targets, the \texttt{has\_Starred} is negatively related to the performance change. For example, if each element of the ``\textsf{e\_list}'' has two items, after refactoring the non-idiomatic code, the part of idiomatic code is ``\textsf{for e\_0, e\_1 in e\_list}''. However, if the element of the ``\textsf{e\_list}'' has three items, the idiomatic code needs a Starred node to denote the remaining items of the element, so the idiomatic code is ``\textsf{for e\_0, e\_1, *e\_len in e\_list}''. The performance change of the idiomatic refactoring of code with Starred node is less than that of code without Starred node. Particularly, we observe that if there is no starred node in the idiomatic code which means that the code fetch all items of each element of the iterator, the performance generally improves. Otherwise, the performance generally decreases.

\noindent\textbf{Relationship (REL) in context}: For the seven Python idioms ( i.e., the list/set/dict-comprehension, chain-comparison, loop-else, assign-multi-targets and star-in-func-call), the performance change in the global scope is greater than of performance change in the local scope. For the remaining two Python idioms (i.e., truth-value-test and for-multiple-targets), the performance change in the global scope is less than of performance change in the local scope.

\noindent\textbf{Relationship (REL) in data}:

\textbf{REL1-\texttt{size\_ele}}: For the list/set/dict-comprehension, the \texttt{size\_ele} is the most important feature. The performance change increases as the number of added elements increases, whereas when the number of elements appended reaches a certain degree, the value of performance change remains stable. Particularly, the performance decreases if there is no element appended to the object. 

For the loop-else, the \texttt{size\_ele} represents the number of iterations. As the number of iterations increases, the performance improvement gradually becomes smaller, and finally the performance change is close to 1, which is basically unchanged.

\textbf{REL2-\texttt{is\_swap}}: For the assign-multi-targets, the performance change of the idiomatic refactoring for swapping variables is greater than of idiomatic refactoring for not swapping variables.

\textbf{REL3-\texttt{is\_const}}: For the star-in-fun-call, the performance change of constant index of Subscript node is greater than of non-constant index of Subscript node. For example, the index is constant for the code ``\textsf{func(e\_list[0], e\_list[1])}'', and the index is non-constant for the code  ``\textsf{func(e\_list[i], e\_list[i+1])}''. After code refactoring, the performance change of code of constant index is greater than of code of non-constant index.

For the assign-multi-targets, the performance change of the idiomatic refactoring of constants assignment is greater than of the idiomatic refactoring of variables assignment. 

\noindent\textbf{Relationship (REL) in state}:

\textbf{REL1-\texttt{is\_true}}: For the chain-compare, the \texttt{is\_true} is positively related to the performance change. The performance change of the true value for the compare node is greater than of false value for the compare node. For example, if ``\textsf{n, o, p}=1, 2, 3'', the value of ``\textsf{n <= o and o > p}'' is ``\textsf{True}'' (code1). However, if ``\textsf{n, o, p}=3, 1, 2'', the value of ``\textsf{n <= o and o > p}'' is ``\textsf{False}''. After refactoring the code, the performance change of the code1 is greater than of the code2. 


% \noindent\FiveStar \textbf{Unintuitive features: }Although some features have no significant relationship with the performance change, we find they are unintuitive. These features are in one dimension: node.

% \textbf{REL1-num\_Assign:} We find the number of assignment node has no significant relationship with the performance change, which is a bit counterintuitive. Since no matter how many assignment statements a non-idiomatic code has, the corresponding idiomatic code has only one assignment statement. It seems the more assignment statements, the greater the performance change but we find their performance changes basically are the same. 

% \textbf{REL2-{eq\_set}:} For the truth-value-test, the node kind of operator has no statistically significant relationship with performance change, which is a little unintuitive. For example, for two non-idiomatic code fragments: \textsf{``if a != []''} and \textsf{``if a == []''}, their corresponding idiomatic codes are \textsf{``if a''} and \textsf{``if not a''}. Although \textsf{``if not a''} has one more \textsf{``not''} than \textsf{``if a''}, their performance changes are basically the same.

 %We observe that if the code is to swap variables in the global scope, the performance basically improves. If the code is to swap variables in the local scope, when swapping two variables, the performance basically improves, otherwise the performance decreases. If the code is only assign the variables instead of swap variables, the performance basically decreases.

\noindent\FiveStar \textbf{The relationship between features and performance change on the field dataset:} On the real-world dataset, the models of the three Python idioms (i.e., loop-else, assign-multiple-targets and for-multiple-targets) could fit the data well. Their important features are also the important features on the laboratory dataset. For the \texttt{scope}, \texttt{is\_swap} and \texttt{has\_Starred} are not the important features on the field dataset because their features are the same on the codes of field dataset. For the \texttt{scope}, all variables on the field dataset are in the local scope. For the \texttt{is\_swap} of assign-multi-targets, all codes of assign-multi-targets are to assign values instead of swapping the variables. For the \texttt{has\_Starred} of for-multi-targets, since the length of iterator cannot be known through static analysis, to ensure the correctness of code refactoring, all idiomatic codes on the field dataset have the Starred node.

For the six Python idioms (list/set/dict-comprehension, chain-comparison, truth-value-test and star-in-func-call), we find their models cannot fit the data well which indicates that symptom features alone cannot reflect the performance change and many other complex factors may affect the performance change on the field dataset. Table\ref{tab:rq3_example} shows examples for the six Python idioms.

For example, for the list-comrehension, although the \texttt{size\_ele} is the most significant feature on the laboratory datasets, the number of elements can also has little effect on performance change. At the list-comprehension row of Table~\ref{tab:rq3_example}, the two code pairs of two datasets basically have the same features such as number of For node and number of added elements. However, the performance improvement on the laboratory dataset (2.87) is significantly larger than of field data (1.03).performance improvement one the field data is only 1.03 but the performance improvement on the laboratory data is 2.87. 

For another example, for the truth-value-test, the ``\textsf{0}'' is not a significant feature on the laboratory dataset. At the truth-value-test row of Table~\ref{tab:rq3_example}, the two code pairs on two datasets is basically same, but the performance improvement on the laboratory dataset (1.05) is significantly less than of field data (11.8).

 
%For the loop-else, assign-multiple-targets and for-multiple-targets, the symptom features can reflect the performance change well. However, for the loop-else and for-multiple-targets, their differences in deviance explained are larger than 20\% on the two datasets, which reflect some idiomatic refactorings maybe influenced by other symptom features. 







%https://www.cnblogs.com/traditional/p/13538919.html 深度剖析Python Interpreter（if/for/exception）
%https://cloud.tencent.com/developer/article/1678615 POP_JUMP_IF_FALSE 指令解析
%https://stackoverflow.com/questions/49735639/in-python-why-is-explicit-bool-much-slower-than-implicit 
\subsection{RQ3: What are the root causes of performance change caused by idiomatic refactorings on the two datasets?}
\subsubsection{Motivation}
 In the previous two research questions, we find that code refactoring with the same Python idiom could improve or decrease performance on the two datasets. And the relationship of code features and performance change of laboratory dataset may not align with that of real-world dataset. Therefore, in this research question, we would like to understand the root causes that different code have different effects on performance change for each Python idiom on the two datasets.% The findings can assist help developers practition- ers in avoiding the use of certain tests in performance assurance activities and in improving tests to serve as performance tests.
\subsubsection{Approach}
To explore the reason of performance change caused by idiomatic refactorings for each Python idiom, it is not reliable to compare the difference of source code between idiomatic code and the corresponding non-idiomatic code because Python interpreter does not directly execute the source code. When the Python code runs, source code first gets compiled into a set of instructions called bytecode. Then the bytecode is executed by the Python interpreter. Therefore, we first get the bytecode instructions of idiomatic code and the corresponding non-idiomatic code for each Python idiom with dis module~\cite{dis_python}. The dis module supports the analysis of CPython bytecode by disassembling it. Then we compare their difference of instructions to understand the impact of code features on performance.
%说明为什么用字节码解释 source code 执行的过程https://legacy.python.org/workshops/1998-11/proceedings/papers/montanaro/montanaro.html，用字节码解释的方法过程 字节码每个meta的概念https://github.com/python/cpython/blob/main/Doc/library/dis.rst

%RQ3 root causes (in both lab and real-world setting, the change by refactoring at the byte-code level are the same, but real-world code involves ……)
% %RQs take-home message and discussion: 
% Refactoring local impact (consider only the code affected by refactoring) are the same in the lab versus real-world setting, but real-world involves many complex context, interweaving ???? which may balance off the improvement by refactoring

% https://towardsdatascience.com/list-comprehensions-vs-for-loops-it-is-not-what-you-think-34071d4d8207
%https://stackoverflow.com/questions/58844643/why-is-my-list-comprehension-function-slower-than-my-list-appending-function-for
%https://www.17tr.com/tool/term/1359708.shtml SOR
\subsubsection{Result}

\noindent\FiveStar \textbf{The bytecodes of idiomatic code and non-idiomatic code are different}. Four differences in bytecodes of the idiomatic refactoring as follows:

\begin{table*}[htbp]
%\vspace{-0.2cm}
\caption{the performance change of code examples of nine Python idioms in the field code}
  \label{tab:rq3_example}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l| l| l| c| c} 
\hline
Idiom&non-idiomatic code  & idiomatic code   & code feature &X\\ \hline

\multirow[b]{2}{*}{\href{https://github.com/kellyjonbrazil/jc/blob/e2f1b16cb9e920968c093bd1f371b191aa7107bf/jc/parsers/csv.py#L145-L146}{list-compre}} & \begin{tabular}[c]{@{}l@{}} raw\_output=[]\\for row in reader:\\    \ \  raw\_output.append(row)\end{tabular} & \begin{tabular}[c]{@{}l@{}}raw\_output = [row \\for row in reader]\end{tabular} &\texttt{size\_ele}:11,766& 1.03\\ 
\cline{2-5} & \begin{tabular}[c]{@{}l@{}} l=[]\\for e\_0 in x\_0:\\    \ \  l.append(e\_0)\end{tabular} & \begin{tabular}[c]{@{}l@{}}l=[e\_0 for e\_0 in x\_0]\end{tabular} &\texttt{size\_ele}:10,000& 2.87\\ \hline
% \href{https://github.com/sympy/sympy/blob/82f264c62db6382fd3545bb43f57584b0f4e27c2/sympy/combinatorics/testutil.py#L195-L197}{set-compre} & \begin{tabular}[c]{@{}l@{}} conjugates = set()\\for el in group.generate\_dimino():
% \\   \ \ for gen in subgr\_gens:
% \\   \ \    \ \      conjugates.add(gen $\wedge$ el)\end{tabular} & \begin{tabular}[c]{@{}l@{}}conjugates = \{gen $\wedge$ el\\ for el in group.generate\_dimino() \\for gen in subgr\_gens\}\end{tabular} &\texttt{size\_ele}:44& 1.008\\ \hline
\multirow[b]{2}{*}{\href{https://github.com/sympy/sympy/blob/429f5be2be5bdc5ee8d717ff857a3268b9c91e40/sympy/ntheory/residue_ntheory.py#L885-L887}{set-compre}} & \begin{tabular}[c]{@{}l@{}} r = set()\\for i in range(p // 2 + 1):\\
    \ \ r.add(pow(i, 2, p))
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
r = \{pow(i, 2, p) for i in range(p // 2 + 1)\}\end{tabular} &\texttt{size\_ele}: 10& 1.04\\ 
\cline{2-5}&\begin{tabular}[c]{@{}l@{}} l = set()\\
for e\_0 in x\_0:\\
    \ \ l.add(e\_0)
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
l = \{e\_0 for e\_0 in x\_0\}\end{tabular} &\texttt{size\_ele}: 10&  1.60\\ 

\hline


\href{https://github.com/networkx/networkx/blob/7b30f1a814d6b7f1b3c4311d19c251b8098d1407/networkx/algorithms/community/quality.py#L299-L302}{dict-compre} & \begin{tabular}[c]{@{}l@{}} rv = \{\}\\for (k, v) in d.items():\\
\  \    rv[k] = v.\_\_self\_\_\end{tabular} & \begin{tabular}[c]{@{}l@{}}rv = \{k: v.\_\_self\_\_ for (k, v) in d.items()\}\end{tabular} &\texttt{size\_ele}:1,000& 1.004\\ 
\cline{2-5} & \begin{tabular}[c]{@{}l@{}} l = dict()\\
l = {e\_0: e\_0 for e\_0 in x\_0}\end{tabular} & \begin{tabular}[c]{@{}l@{}}
l = \{e\_0: e\_0 for e\_0 in x\_0\}\end{tabular} &\texttt{size\_ele}:1,000& 1.09\\
\hline

\multirow[b]{2}{*}{\href{https://github.com/brainix/pottery/blob/c7be6f1f25c5404a460b676cc60d4e6a931f8ee7/pottery/deque.py#L56}{chain-comparison}} & \begin{tabular}[c]{@{}l@{}} self.maxlen is not None and \\ current\_length >= self.maxlen\end{tabular} & \begin{tabular}[c]{@{}l@{}}None is not self.maxlen <= current\_length\end{tabular} & \texttt{scope}: in the function& 1.3\\ 
\cline{2-5} & \begin{tabular}[c]{@{}l@{}} n != o and o >= p\end{tabular} & \begin{tabular}[c]{@{}l@{}}n != o >= p\end{tabular} & \texttt{scope}: in the function& 0.97\\
\hline

\multirow[b]{2}{*}{\href{https://github.com/nipy/nibabel/blob/225892af18d82b9a91ab63a9d072b894588b670e/nibabel/volumeutils.py#L940}{truth-value-test}} & \begin{tabular}[c]{@{}l@{}} if inter != 0:\end{tabular} & \begin{tabular}[c]{@{}l@{}}if inter:\end{tabular} &comparator:0& 11.8\\

\cline{2-5} & \begin{tabular}[c]{@{}l@{}} if a != 0:\end{tabular} & \begin{tabular}[c]{@{}l@{}}if a:\end{tabular} &comparator:0& 1.05\\\hline

% \href{https://github.com/quantumlib/OpenFermion/blob/5ef58b507270f18627ec563a43001c404cf5e6c1/src/openfermion/measurements/fermion_partitioning.py#L276-L282}{loop-else} & \begin{tabular}[c]{@{}l@{}} success\_flag = True\\
%     for divisor in range(2, num\_bins - 1):\\
%     \ \     if trial\_size \% divisor == 0:\\
%         \ \ \ \     success\_flag = False\\
%         \ \ \ \     break\\
%     if success\_flag:\\
%       \ \  return trial\_size\end{tabular} & \begin{tabular}[c]{@{}l@{}}
%     for divisor in range(2, num\_bins - 1):\\
%     \ \     if trial\_size \% divisor == 0:\\
%         \ \ \ \     break\\
%     else:\\
%       \ \  return trial\_size\end{tabular} &iterations:<10& 1.3\\ \hline
       
% \href{https://github.com/Erotemic/ubelt/blob/cdb6aa9dea7567ce742ee6a11d8a1ca4ac89f342/ubelt/util_cache.py#L497-L501}{assign-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
% cfgstr = self.\_rectify\_cfgstr(cfgstr)\\
% dpath = self.dpath\\
% fname = self.fname\\
% verbose = self.verbose
% \end{tabular} & \begin{tabular}[c]{@{}l@{}}
%     cfgstr , dpath , fname , verbose  = \\ self.\_rectify\_cfgstr(cfgstr), self.dpath,\\ self.fname, self.verbose\end{tabular} &num\_assign:4& 0.78\\ \hline

\multirow[b]{2}{*}{\href{https://github.com/maxpumperla/elephas/blob/c474bb4f2565185dfd89fd06a8fe467fa9c64b2b/elephas/mllib/adapter.py#L13-L14}{star-in-func-call}} & \begin{tabular}[c]{@{}l@{}} 
func(np\_array.shape[0], np\_array.shape[1])
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    func(*np\_array.shape[:2])\end{tabular} &num\_subscript:2& 1.004\\ 
  \cline{2-5}
% \href{https://github.com/gugarosa/opytimizer/blob/f3e110cdc7fb8557d7e041737d3c9fd63f375c1e/opytimizer/visualization/surface.py#L39}{star-in-func-call} 
& \begin{tabular}[c]{@{}l@{}} 
func(e\_list[0], e\_list[1])
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
 func(*e\_list[:2])\end{tabular} &num\_subscript:2& 0.77\\ \hline

% \href{https://github.com/networkx/networkx/blob/e0c055a3524f583b60c89ea5d72a3b624212f357/networkx/algorithms/community/quality.py#L327}{for-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
% for e in G.edges():\\
% \ \     e[0]\\
% \ \     e[1]
% \end{tabular} & \begin{tabular}[c]{@{}l@{}}
%     for  (e\_0, e\_1, *e\_len) in G.edges():\\
% \ \     e\_0\\
% \ \     e\_1\end{tabular} &num\_subscript:2& 0.9\\ \hline

% \href{https://github.com/alichtman/shallow-backup/blob/d71b903dacd5eeea9d0be68ef3022817f9bac601/shallow_backup/backup.py#L81-L84}{for-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
% for pacman\_option in \\pacman\_options.values():\\
% \ \     pacman\_option[0]\\
% \ \     pacman\_option[1]
% \end{tabular} & \begin{tabular}[c]{@{}l@{}}
%     for  (pacman\_option\_0, pacman\_option\_1, *pac-\\man\_option\_len)  in pacman\_options.values():\\
% \ \     pacman\_option\_0\\
% \ \     pacman\_option\_1\end{tabular} &num\_subscript:2& 0.33\\ \hline
\end{tabular}
\vspace{-0.3cm}
\end{table*}


\textbf{Python idioms add new bytecodes} which could decrease the performance. There are list/set/dict comprehension and assign-multi-targets. 

For the list/set/dict comprehension, they need to additionally execute instructions of calling comprehension code object before code iteration (red dotted box in Figure~\ref{fig:bytecode_list_compre}). 

For the assign-multi-targets, the ``\textsf{=}'' actually does not have the corresponding bytecodes, so the more assign statements will not add costs. Furthermore, if there are multiple values for one assign statement, to assign each value to the corresponding target it needs to additionally execute instructions of building a tuple (\textsf{``BUILD\_TUPLE''}) and unpacking the sequences (\textsf{``UNPACK\_SEQUENCE''}) to put values onto the stack right-to-left. Therefore, if the assign-multi-targets are only to assign variables, the performance decreases. And as the number of assign nodes increases, the \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''} needs to operate more values, the slower performance. 

\begin{figure}
  \centering
  \includegraphics[width=3.5in]{./data/rq4_bytecode.png}%performance_rq1_list_compre.pdf
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Bytecode instructions of idiomatic refactorings of list comprehension}
    
    \label{fig:bytecode_list_compre} \vspace{-0.3cm}
    %\vspace{-0.6cm}
\end{figure}
\textbf{Python idioms use the unique bytecode to replace a series of bytecodes of non-idiomatic code} which could improve the performance. For the list/set/dict comprehension, they use the specialized add instructions
to reduce the cost of a series of instructions of loading objects and calling function. For example, for the list-comprehension, to append elements with a specific instruction to appending elements. For example, for the list comprehension (green dotted box in Figure~\ref{fig:bytecode_list_compre}), to append elements each iteration, the idiomatic code only need execute the ``LIST\_APPEND'' instruction to append the element, but the non-idiomatic code needs to execute ``\textsf{LOAD\_*}'' instructions to push data into the stack and then call function to append the element. Since the cost of ``\textsf{LIST\_APPEND}'' is less than that of a series instructions especially the expensive the function call instruction for the non-idiomatic code, the performance improves. As the number of added elements (\texttt{size\_ele}) increases, the greater the difference in cost of bytecodes instruction, the performance change will increase. When the \texttt{size\_ele} increases to a certain value, the performance change will stop 
growing because it makes the cost of bytecodes before iterating trivial and approximately equals the cost of for body of the non-idiomatic code divided by the cost of for body of the idiomatic code. 


Different from the list/set-comprehension, for the dict comprehension, the non-idiomatic code does not need to execute the instruction of function call. Although the \textsf{``MAP\_ADD''} of dict-comprehension reduce the cost of loading the dictionary iterable, the \textsf{``MAP\_ADD''} achieves basically the same thing as \textsf{``STORE\_SUBSCR''} (storing the key-value pair) of non-idiomatic code. Therefore, the performance improvement of dict comprehension (the maximum is 1.2 when code is in the local cope) is significantly smaller than that of list/set comprehension. 

\textbf{Python idioms replace bytecodes of non-idiomatic codes with other bytecodes} which could improve performance or decrease performance depend on the specific code. There are chain-compare, star-in-fun-call, for-multi-targets and assign-multi-targets.

For the chain-compare, it replaces one instruction to load the comparator of non-idiomatic code with the instructions to create a reference to a comparator (\textsf{``DUP\_TOP''}) and reference shuffling (\textsf{``ROT\_THREE''}). Saving an extra reference to the comparator for the chained comparison isn't literally free, it is the slightly cheaper operation of loading a local variable. Therefore, if the comparator is in the local scope, the performance decreases (the 1st row in the chain-compare row of Table~\ref{tab:rq3_example}). Otherwise, the performance improves. And if the comparator is more complex such as the attribute access, the greater performance improvement (the 2nd row in the chain-compare row of Table~\ref{tab:rq3_example}).

For the star-in-fun-call that only accesses part of elements, the non-idiomatic code replaces the instructions to load the iterable and access elements with specified index (\textsf{``BINARY\_SUBSCR''}) with the instructions to build the slice (\textsf{``BUILD\_SLICE''}). Since the cost of \textsf{``BUILD\_SLICE''} is larger than of \textsf{``BINARY\_SUBSCR''}, only if the number of Subscript nodes of non-idiomatic code increases to a certain value, the performance probably improve. 

For the for-multi-targets, the non-idiomatic code replaces the instructions of \textsf{``BINARY\_SUBSCR''} with the instruction to 
unpacking the object. Since the cost of unpacking the object is larger than of \textsf{``BINARY\_SUBSCR''}, only if the number of Subscript nodes of non-idiomatic code increases to a certain value (about 5), the performance probably improve.


For the assign-multi-targets, if it is to assign constant values or to swap variables, they replace bytecodes of loading objects with bytecodes of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. For the constant assignment, the idiom could uses one ``\textsf{LOAD\_CONST}'' to load the multiple constants. For the swapping variables, the idiom reduces the bytecodes of loading and storing temporary variables. However, the idioms needs to build the tuple and unpacking the sequence for all values, which are more expensive than of cost of loading more variables for the non-idiomatic code. to reduce such cost of the idiom, for swapping two variables, it executes the cheaper instruction (\textsf{``ROT\_TWO''}) to directly swap variables instead of building and unpacking the tuple, so swapping two variables can improve performance. Otherwise, the performance generally decreases.

\textbf{Python idioms remove byte codes of loading objects non-idiomatic codes} which could improve the performance. There are truth-value-test, loop-else and star-in-fun-call. The truth-value-test reduces the cost of objects from \texttt{empty\_set} and improves the performance. The loop-else reduces the cost of assigning the flagging variables and improves the performance. For the star-in-fun-call that accesses all items of the object, it removes the cost of loading the object multiple times and accessing an element with the index, which improves performance.
%Otherwise, there is no obvious %but the non-idiomatic code(>8) uses each ``\textsf{LOAD\_CONST}'' to load a constant each time. Therefore, the performance change of the constant assignment is greater than that of variable assignment. Howeverit replaces instructions of loading multiple constants with  In the case,  Therefore, the performance change of the constant assignment is greater than that of variable assignment.  Since the cost of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''} is larger than of ``\textsf{LOAD\_CONST}'', as the number of values increases to a certain value (>8), the cost can balance off the cost of  of assign-multi-targets and makes the assign-multi-targets performance improve. If it is to swap variables, it replaces  and star-in-func-call, it reduces the cost of 








%The reason of the positive relationship of \texttt{size\_ele} with the performance change is that the list/set comprehension replaces the instructions of loading the iterator and calling function with a specific instruction of appending elements. For example, for the idiomatic code of list comprehension, to appending a element to the list, developers replace the instructions of loading the list and calling the append function with the \textsf{``LIST\_APPEND''} (green dotted box in Figure~\ref{fig:bytecode_list_compre}). Each iteration, the non-idiomatic code executes instructions of function call, but the corresponding idiomatic code only needs to execute the \textsf{``LIST\_APPEND''} instruction for appending elements, so as more elements are appended, the greater the performance change. When the number of added element exceeds a certain value, the performance change basically no longer increases, which is approximately the cost of instructions of function call divided by the cost of the \textsf{``LIST\_APPEND''} instruction.


\noindent\FiveStar \textbf{Reasons of the nonalignment of performance change on two datsets} as follows:

\begin{itemize}[fullwidth]
\item \textbf{External objects (non-Python built-in objects) overloads Python built-in methods that executed by bytecodes, which make the cost of bytecodes become large}. There are three bytecodes: iterating elements (\textsf{FOR\_ITER}), compare operation (\textsf{COMPARE\_OP}) and testing the truthiness (\textsf{POP\_JUMP\_IF\_TRUE} or \textsf{POP\_JUMP\_IF\_FALSE}). 

\ \ The cost of \textsf{``FOR\_ITER''} varies with different code. Each iteration, when Python interpreter executes \textsf{``FOR\_ITER''} to get the next item of the iterator, it needs to call \textsf{``\_\_next\_\_()''} method. Therefore, if the iterator is not the Python built-in type and its cost of the self-implemented \textsf{``\_\_next\_\_()''} is large, which may balance off the improvement of Python idioms. For example, at the 1st row of list-comprehension row Table~\ref{tab:rq3_example}, the \textsf{``reader''} is a reader object from csv library, which overloads the \textsf{``\_\_next\_\_()''} method. Since the cost of \textsf{``\_\_next\_\_()''} is larger than the cost of \textsf{``append''} method of list, the performance improvement is only 1.03.

% \ \  For the truth-value-test, developers overload the methods of the compare operation (``\textsf{COMPARE\_OP}'') or the instruction of  testing the top item of the stack is true or not (\textsf{``POP\_JUMP\_IF\_TRUE''} or \textsf{``POP\_JUMP\_IF\_FALSE''}), which make performance may improve or decreases. 

\ \  For the compare operation, library developers usually make the cost larger than of Python implementation for special reasons (e.g., multiple elements comparison), which may make performance largerly improves. For example, the 1st row of truth-value-test row in Table~\ref{tab:rq3_example}, the \textsf{``inter''} is array object of numpy library, since the numpy overload the compare operation and needs to do a series of dispatching, type conversion, and wrapper object allocation  that doesn't happen when working with Python built-in objects such as list, the large cost of the compare operation make the performance improves a lot and more than ten times. 

\ \  When Python interpreter executes the instruction to  test the truthiness of value, it calls the \textsf{``\_\_bool\_\_()''} method or \textsf{``\_\_len\_\_()''} method if the object is not bool data type. Therefore, if the object is not Python built-in data type, the implementation of \textsf{``\_\_bool\_\_()''} and \textsf{``\_\_len\_\_()''} may largely impact the performance. For example, for the \href{https://github.com/searx/searx/blob/5b50d7455a719b145be5f90069026a60b480673d/searx/utils.py#L259}{\textsf{``xpath\_results == []''}} code, the \textsf{``xpath\_results''} is \textsf{``HtmlElement''} from lxml library, it define the \textsf{``\_\_bool\_\_''} method ineffectively which make the performance decreases largely and less than 0.2. And we find that the developers may improve the implementation of  \textsf{``\_\_bool\_\_''} method because its source code has a warning: the method will change in future versions. 

\item \textbf{Code on the field dataset uses more complex code (i.e., function calls, attribute access and compounding of expressions and statements) which make performance improve or decrease.} For example, at the 1st row of set-comprehension row in Table~\ref{tab:rq3_example}, instead of simply adding a variable to the ``\textsf{conjugates}'', this code adds a binary operator expression ``\textsf{
gen \^ el}'' that balance off the benefits of set-comprehension. Therefore, the performance improvement is small and less than 1.1. For another example, at the 1st row of the chain-comparison row of Table~\ref{tab:rq3_example}, the chained comparator is not a simple variable but is an attribute access ``\textsf{self.maxlen}''. The cost of creating reference and shuffling reference is less than of  attribute access, which make the performance improvement.


\end{itemize}


%why generator或者非内置的object slower 有https://www.programiz.com/python-programming/generator
%https://www.programiz.com/python-programming/iterator

% For one thing, each iteration, when Python interpreter executes \textsf{``FOR\_ITER''} to get the next item of the iterator , it needs to call \textsf{``\_\_next\_\_()''} method. Therefore, if the iterator is not the Python built-in type and its cost of the self-implemented \textsf{``\_\_next\_\_()''} is large, which could balance off the improvement of list/set/dict comprehension. For example, for the code of the 1st row of Table~\ref{tab:rq3_example}, the \textsf{``reader''} is a reader object from csv library, which overloads the \textsf{``\_\_next\_\_()''} method. Since the cost of \textsf{``\_\_next\_\_()''} is larger than the cost of \textsf{``append''} method of list, the performance improvement is only 1.03.

% \begin{figure}
%   \centering
%   \includegraphics[width=3.5in]{./data/rq4_bytecode.png}%performance_rq1_list_compre.pdf
% \setlength{\abovecaptionskip}{-0.1cm}
%     \caption{Bytecode instructions of idiomatic refactorings of list comprehension}
    
%     \label{fig:bytecode_list_compre} \vspace{-0.3cm}
%     %\vspace{-0.6cm}
% \end{figure}


%the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants.The greater performance improvement of idiomatic refactorings with function call comparator (e.g., \textsf{``Fraction(0,1)''} and \textsf{``dict()''}) instead of basic data types because the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants.%  instruction rather than instructions of loading variables or constants, the differences in performance change of idiomatic refactorings will be greater, so the performance improvement will be greater. 

% The instructions of \textsf{``if not object''} and \textsf{``if object''} idiomatic codes are almost same because the corresponding instructions are \textsf{``POP\_JUMP\_IF\_FALSE''} and \textsf{``POP\_JUMP\_IF\_TRUE''}, respectively. Therefore,  although the comparison operators \textsf{``==''} and \textsf{``!=''} have no difference is that their instructions are to test the top item of the stack is true or not. Specifically, the instruction \textsf{`object''} of test node is  \textsf{``POP\_JUMP\_IF\_FALSE''}, and for the \textsf{``not object''}, Python interpreter will automatically compiles it \textsf{``POP\_JUMP\_IF\_TRUE''} and does not need to execute extra instructions. Therefore, although the comparison operators \textsf{``==''} and \textsf{``!=''} have different number of tokens, their performance changes are basically the same.

%https://github.com/hemildesai/numpy/blob/6fbbadb676dfa7cee56be3bd17b92bde661f8869/numpy/core/numeric.py#L363-L372 built-in method ``__nonzero__()`` (renamed ``__bool__()`` in python3.x
%https://github.com/lxml/lxml/blob/c742576c105f40fc8b754fcae56fee4aa35840a3/src/lxml/etree.pyx#L2500-L2507
%https://github.com/numpy/numpy/blob/4cbced22a8306d7214a4e18d12e651c034143922/doc/source/reference/arrays.ndarray.rst numpy是因为对==的重载
%Particularly, when there are only two variables, the idiomatic code uses the \textsf{``ROT\_TWO''} instruction to complete the assignment to reduce the performance regression. 

%Therefore, the swappuse the The reason of performance regression of variable assignment code refactorings is that the extra cost of instructions of building a tuple for multiple values (\textsf{``BUILD\_TUPLE''}) and unpack the tuple (\textsf{``UNPACK\_SEQUENCE''} ).  For example, for the code in the 8th row of Table~\ref{tab:rq3_example}, the non-idiomatic code has four assignment node but the idiomatic code only has one assignment node, so it seems that the idiomatic code may improve performance. However, the (\textsf{``=''}) has no real byte code instructions and one assignment statement consists of instructions of loading objects and storing objects. The non-idiomatic code loads one object and then stores one object each time. While the idiomatic code first loads four objects four times. For assigning values into targets correctly, idiomatic code then executes two extra instructions \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''} to put values onto the stack right-to-left. Finally, the idiomatic code stores four objects four times. Therefore, the idiomatic refactorings of assign-multiple-targets actually decrease the performance.

% The reason of performance improvement of code of swapping variables in the global scope is that the cost of instructions of loading and storing global temporary variables is larger than instructions of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. However, when variables are in the local scope, the cost of instructions of loading and storing local temporary variables is generally less than of instructions of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. Particularly, when the idiomatic code is to swap two variables in the local scope, the performance improves because Python developers design an instruction \textsf{``ROT\_TWO''} to quickly swap two variables on the stack.

% The reason of performance improvement of code of constant assignment code with more than about 8 constants is that the idiomatic code directly loads all constants once as a tuple (\textsf{``LOAD\_CONST''}) and then unpacks the tuple (\textsf{``UNPACK\_SEQUENCE''}) rather than loading a constant at a time like the non-idiomatic code. When the number of constants is larger than 8, the cost of \textsf{``UNPACK\_SEQUENCE''} is generally larger than of  8 \textsf{``LOAD\_CONST''} instructions.

 %First, when the code is to fetch all elements of the iterator, the idiomatic code does not need to execute the \textsf{``BUILD\_SLICE''}, so the performance improves. Second, 



%The reason of performance change of code in the global scope is greater than of code in the local scope is that the cost of loading global variables is greater than of loading local variables. And the reason of performance change of the variable index is greater than of the constant index is that the cost of loading variables is greater than of loading constants. 
%https://blog.csdn.net/woshaguayi/article/details/108484328
%If the to The difference in bytecode instructions of idiomatic code and idiomatic code is that the body of non-idiomatic code needs to accessing elements at specified indices (\textsf{``LOAD\_CONST''} and \textsf{``BINARY\_SUBSCR''}) but the idiomatic code does not do it. Therefore, when the code unpacks all elements, the performance will improve the performance. However, if the code unpacks part of elements, each iteration the idiomatic code needs to store an extra variable, e.g., the \textsf{``*x\_len''} variable in the the last row of the Table~\ref{tab:rq3_example}, the performance will decrease.

% The cost of \textsf{``FOR\_ITER''} varies with different code, if the 
% !!!!!!!
% !!!!!!!
% !!!!!!!
%set comprehension sympy developers 主动用python idioms重构了代码
% !!!!!!!
% !!!!!!!
% !!!!!!!


==> result_5.tex <==
\subsection{RQ1:What Is the Peformance Impact of Idiomatic Refactoring on the laboratory dataset and field dataset?}
\subsubsection{Motivation}
Section~\ref{motivation} shows that developers are interested in whether Python idioms could improve performance or decrease performance. Furthermore, we find there are some arguments on different code. Therefore, this research question answers the performance impact of the idiomatic refactoring on the laboratory dataset and field dataset.% 
%之后再改
\subsubsection{Approach}
As described in Section~\ref{data}, we collect XXX non-idiomatic and the corresponding idiomatic code pairs for nine Python idioms, and then we compute the performance change on the two datasets based on the approach of Section~\ref{measurement}. We mainly analyze four aspects of Python idioms on two datasets: performance impact (performance improvement/regression/unchanged), the upper bond, lower bond and the range of performance change.  %the differenceschange () % 先计算两组数据的数值，然后XXX If the performance change is larger than 1, the performance improves (i.e., performance improvement). If the performance change is less than 1, the performance decreases (i.e., performance regression). Otherwise, the performance basically is unchanged (i.e., performance unchanged). 

\subsubsection{Result}
Figure~\ref{fig:performance_rq1} shows the distribution of performance change of nine Python idioms on the laboratory dataset and on the real-world dataset. The gray circle represents the outliers of dataset. The upper and lower whiskers represent the maximum and the minimum of performance change of dataset excluding the outliers. The range of the box represents 25th to the 75th percentile of dataset.
%Rplots_spline_change_y.pdf
\begin{figure}
  \centering
  \includegraphics[width=3.4in]{./data/performance_rq1_compare_boxplot_new_perf_change_speedup_slowdown.pdf}%performance_rq1_compare_boxplot_new_2.pdf. rq1_perf_change_box_plot.png
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Performance Change of Idiomatic Code versus Non-idiomatic Code in the Synthetic Dataset and Real-Project Dataset \zc{1) Update legend Synthetic Code, Real-Project Code. 2) y-axis which divided by which equation 3) Is the bottom-left a 20 or 28? may not need 0 point? 4) use - not \_ in idiom name 4) slowdown show more ticks 9/10, 8/10, ...5/10, ... 5) Double check: is the middle line median? median should be in the exact middle of the box. it seems to be the average. 6) x-axix is a bit confusing to read which ticks maps to which names. see if you can improve. 7) Very confusing why speedup 2 is narrower than slowdown 2. Maybe the same scale for speed up and slowdown, use +x for speedup and -x for slowdown.}}
    
    \label{fig:performance_rq1} 
    \vspace{-0.3cm}
    %\vspace{-0.6cm}
\end{figure}
\noindent$\bullet$ \textbf{Performance impact of Python idioms on two datasets:} On the laboratory dataset, for seven Python idioms (list/set/dict-comprehension, truth-value-test, loop-else, star-in-func-call and for-multi-targets), the performance of the majority of idiomatic refactorings improves. For remaining two Python idioms (chain-comparison and assign-multi-targets), the performance of the majority of idiomatic refactorings decreases. 

On the field dataset, for the truth-value-test, the performance of the majority of idiomatic refactorings improves. For the set-comprehension and loop-else, the performance of the majority of idiomatic refactorings basically does not change. For the remaining six Python idioms, the performance of the majority of idiomatic refactorings decreases.

Therefore, the performance impact of four Python idioms (truth-value-test, chain-comparison, loop-else and assign-multi-targets) is consistent on the two datasets. For the truth-value-test, it is more likely to improve performance. For the loop-else, the performance basically unchanges or improves small. For the chain-comparison and assign-multi-targets, the performance is more likely to decrease. The remaining five Python idioms exist obvious differences in performance impact on two datasets, which indicates that their performance impacts vary largely for the different code and cannot easily inferred.

\noindent$\bullet$ \textbf{The maximum of performance improvement of Python idioms on two datasets:} 
%\zc{This part should analyze only those idioms with majority improvements?}
On the laboratory dataset, for six Python idioms (list/set/dict-comprehension, truth-value-test, star-in-func-call and for-multi-targets) \zc{For set-comprehension, dict-comprehension, star-in-func-call, those greater than 2 are mostly outliers. I think we should treat these three separately from list-compprehensioin, truth-value-test, for-multi-targets which have some percentage of instances greater than 2. }, the maximum of performance improvement is basically bigger than 2 which means that the idiomatic code is 50\% faster than the corresponding non-idiomatic code. On the field dataset, only the truth-value-test makes more than 2X speed up. 

Therefore, the maximum of performance improvement of \zc{four ??} Python idioms (truth-value-test, \zc{chain-comparison, assign-multi-targets and loop-else}) is consistent on two dataset. The maximum performance improvement of truth-value-test generally can be more than 2. The maximum performance improvement of three Python idioms (\zc{chain-comparison, assign-multi-targets and loop-else}) is likely to be no more than 2. 
For remaining five Python idioms, their maximum performance improvement is \zc{not stable ??inconsistent between synthetic and real-project code.}.

\noindent$\bullet$ \textbf{The maximum of performance regression of Python idioms on two datasets:} 
%\zc{This part should anlayze only those idioms with majority regression?}
On the laboratory dataset, for four Python idioms (list-comprehension, truth-value-test, star-in-fun-call and for-multi-targets), the maximum of performance regression is \zc{bigger than 2 ??confusing? bigger than 1/2?} which means that the idiomatic code is 100\% slower than the non-idiomatic code. However, on the field dataset, for three Python idioms (\zc{list-comprehension ??only outliers?}, \zc{star-in-func-call ??not bigger than 2} and for-multi-targets), the maximum of performance regression is bigger than 2. 

Therefore, the maximum of performance regression of eight Python idioms are consistent on the two datasets. Among the seven Python idioms, the maximum of performance regression of three Python idioms (list-comprehension, star-in-func-call and for-multi-targets) can be large (>2). For five Python idioms (set-comprehension, dict-comprehension, chain-comparison, loop-else and assign-multi-targets), the maximum of the performance regression is more likely to be no more than 2. For the truth-value-test, the maximum of the performance regression is not stable.


\noindent$\bullet$ \textbf{The range of performance change of Python idioms on two datasets:} On the laboratory dataset, the range of performance change of list-comprehension and for-multi-targets is \zc{greater than 2 ??very confusing! how to compute the range from slowdown 2 to speedup 2? 4? or 2?}. For three Python idioms (chain-compare, loop-else and assign-multi-targets), the range of performance change is less than 1. For the remaining four Python idioms, the range of performance change is between 1 and \zc{2 ??very confusing. which 2? speedup or slowdown?}.

On the field dataset, the range of performance change of truth-value-test and for-multi-targets is greater than 2. For the remaining seven Python idioms, the range of performance change is less than 1.

Therefore, the variation of performance change of three Python idioms (chain-compare, loop-else and assign-multi-targets) is relatively stable on two datasets, where the range of performance change is less than 1. The remaining five Python idioms is relatively unstable (the range of performance change maybe larger than 2).

% For seven Python idioms (list/set-comprehension, chain-comparison, loop-else, assign-multi-targets, star-in-func-call and for-multi-targets), the variation of performance change of laboratory dataset is greater than that of field dataset. For example, for the list comprehension, the ranges of performance change on the laboratory dataset and the field dataset are about 2X slowdown$\sim$2.8X speedup and 1.4X slowdown$\sim$1.2X speedup respectively. 

% For the truth-value-test, the variation of performance change of laboratory dataset is smaller than that of field dataset. The range of performance change of list comprehension is about 1.02X speedup$\sim$2.3X speedup, but the performance change of real-world dataset is about 20X slowdown$\sim$11.9X speedup. 

% For the dict-comprehension, the variation of performance change of laboratory dataset intersects with that of real-world dataset for the dict comprehension, but the performance change of most of idiomatic refactorings of the real-world dataset is less than of laboratory dataset.
% \textbf{Summary:}
% \emph{For nine Python idioms, on the two datasets, the performance change of chain-comparison, the loop-else and assign-multi-targets are relatively stable. The chain-comparison and assign-multi-targets are more likely to decrease performance. The loop-else has little performance impact. The performance change of remaining six Python idioms varies largely, they may increase or decrease the performance based on different code.}
% \vspace{1mm}
\noindent\fbox{\begin{minipage}{8.4cm} \emph{For nine Python idioms, on the two datasets, the performance change of chain-comparison, the loop-else and assign-multi-targets are relatively small. The chain-comparison and assign-multi-targets are more likely to decrease performance. The loop-else has little performance impact. The performance change of remaining six Python idioms vary largely, they may increase or decrease the performance based on different code.} \end{minipage}}

% First, for the laboratory dataset, the upper bond of performance change 

% First, the maximum performance change (11.9) of the truth-value-test of the real-world dataset is larger than of laboratory dataset (7.2). While the maximum of performance improvement of remaining eight Python idioms are less than of real-world dataset.

% All idiomatic refactorings of nine Python idioms can improve or decrease the performance among the two datasets. First, for the performance improvement, among the two datasets, there are six Python idioms (list/set/dict comprehension, star-in-function-call, for-multiple-targets and truth value test) where idiomatic refactoring can make performance changes greater than 2. However, for the remaining three Python idioms, chain-comparison, loop-else and assign-multiple-targets,  their maximums of performance improvement of all idiomatic refactorings on the two datasets are less than 2. Besides, for the performance regression, among the two datasets, there are two Python idioms (for-multiple-targets and truth-value-test) where some idiomatic refactorings make the performance change less than 0.5. For the six Python idioms (list/set/dict-comprehension, chain-comparison, assign-multiple-targets and star-in-func-call), their performance changes of idiomatic refactoring basically are above 0.5. The performance change of idiomatic refactorings of loop-else basically is greater than 0.9.

% There are three differences in the maximum performance change, minimum performance change and the range of performance change on the two datasets.

% First, the maximum performance change (11.9) of the truth-value-test of the real-world dataset is larger than of laboratory dataset (7.2). While the maximum of performance improvement of remaining eight Python idioms are less than of real-world dataset.%have the opposite results from the truth-value-test. 

% Second, for the difference in minimum performance change on the two datasets, the two Python idioms (star-in-fun-call and for-multiple-targets) of the real-world dataset is greater than of laboratory dataset. The remaining six Python idioms have the opposite results to the results of star-in-fun-call and for-multiple-targets. Particularly, the minimum performance change of the truth-value-test is larger than 1 on the laboratory dataset but the minimum of performance change on the real-world dataset only is 0.05.

% Finally, for the difference of the performance change variation of most of idiomatic refactorings for each Python idiom on the two datasets, we could observe the upper and lower whiskers of the Figure~\ref{fig:performance_rq1}. The variation of performance change of laboratory dataset is smaller than that of real-world dataset for the truth-value test idiom. For example, the range of performance change of list comprehension is about 1.02$\sim$2.3, but the performance change of real-world dataset is about 0.05$\sim$11.9. The variation of performance change of laboratory dataset intersects with that of real-world dataset for the dict comprehension, but the performance change of most of idiomatic refactorings of the real-world dataset is less than of laboratory dataset. The variation of performance change of laboratory dataset is relatively greater than that of real-world dataset for the remaining seven Python idioms. For example, for the list comprehension, the ranges of performance change on the laboratory dataset and the real-world dataset are about 0.5$\sim$2.8 and 0.7$\sim$1.2 respectively. 

\subsection{RQ2: What features are related to the performance change on two datasets?}\label{rq2}%WHAT FACTORS AND PROBLEMS ARE RELATED TO THE EFFECTIVENESS OF GFIS? How well the symptom features can explain the performance change of idiomatic refactorings on the laboratory dataset and the real-world dataset
\subsubsection{Motivation}
Section~\ref{sec:motivation} shows that developers are interested in how much idiomatic refactorings can improve or degrade performance. In the research question, investigating the relationship between code features and performance change could help developers use Python idioms better.% and make better choices about how they code, which idioms to prioritize to refactor their code, and how they optimize their code to make Python idioms faster.
\subsubsection{Approach}
%deviance explained
%https://stats.stackexchange.com/questions/519904/how-to-calculate-the-percentage-deviance-explained-wiith-glm-nb
%The answer is your first one (i.e., 2.01). Anyone can easily calculate percent deviance explained of a model by the following codes: 100*with(summary(model), 1 - deviance/null.deviance)
%%Mixed Effects Models and Extensions in Ecology with R---
%We do not have an R2 in GLM models, but the closest we can get is the explained deviance, which is calculated as. So the explanatory variable distance to the park explains 63.51% of the variation in road kills. Dobson (2002) called this proportional increase in explained deviance the pseudo R2--并且介绍了deviance explained的详细计算方法
%https://stats.stackexchange.com/questions/100238/what-is-a-relevant-level-for-percentage-deviance-explained-in-a-glm , % of deviance explained is an effect size measure. Such a measure is not either significant or not sig; it may be important or not important. Unfortunately, any guidelines as to how big a % is how important is going to be context dependent.
% The percentage in the fourth column (shown in parentheses) is the ratio of R2(met. var.) and R2. values between 0.41 and 0.60 indicate that the model explains most of the variation, although considerable variation remains unaccounted for. The percenta-----Using a generalized additive model to quantify the influence of local meteorology on air quality in Zagreb---也包含了VIF
%The proportion of variance explained by the model was 50.0%. The order of importance of the predictors in explaining D. serra recruitment, inferred from the AIC statistics in the stepwise model, Investigating biotic and abiotic factors affecting the recruitment of an intertidal clam on an exposed sandy beach using a generalized additive mode D.S. Schoemana,*, A.J. Richardsonb,1
%https://www.researchgate.net/profile/Ivan-Mateo-2/publication/281939856_A_Comparison_of_Statistical_Methods_to_Standardize_Catch-Per-Unit-Effort_of_the_Alaska_Longline_Sablefish_Fishery/links/55ff47d408aec948c4f9b136/A-Comparison-of-Statistical-Methods-to-Standardize-Catch-Per-Unit-Effort-of-the-Alaska-Longline-Sablefish-Fishery.pdf
% explained deviance is an interpretable measure of the strength of the association. The deviance explained by each variable modelled separately can be contrasted with the total deviance explained by a model that includes all the variables. Thus the proportion of the explainable deviance attributable to each driver alone can be extracted and compared against the total explainable devianc-----Drivers of deforestation in the basin of the Usumacinta River: Inference on process from pattern analysis using generalised additive models
% To assess how well the models fitted the data, percent of deviance explained was used. Percent deviance explained (pseudo-R2) was calculated with the formula 1-(residual deviance/total deviance). To assess the relative importance of different explanatory variables in GLM and GAM models, relative variable importance was calculated by examining changes in improvement of AIC by examining the addition of one variable at a time (CPUE~Year+ βX1). We used this approach because the relative importance of explanatory variables to the model fit can change based on the order the variables are entered into the model. In BRT models, the relative influence of explanatory variables was calculated by how many times that variable was selected for splitting and averaged over all trees compared to the squared improvement to the model fit (Elith et al. 2008). Then, the contribution of each variable is scaled to a total of 100.
%https://bookdown.org/egarpor/PM-UC3M/glm-deviance.html
%https://rdrr.io/cran/modEvA/man/Dsquared.html 
%https://modtools.wordpress.com/2013/08/14/dsquared/
%Linear models come with an R-squared value that measures the proportion of variation that the model accounts for. The R-squared is provided with summary(model) in R. For generalized linear models (GLMs), the equivalent is the amount of deviance accounted for (D-squared; Guisan & Zimmermann 2000). The Dsquared function, now included in the modEvA package (Barbosa et al. 2014), calculates it. There is also an option to calculate the adjusted D-squared, which takes into account the number of observations and the number of model parameters, thus allowing direct comparison among different models (Weisberg 1980, Guisan & Zimmermann 2000). UPDATE: see also further measures in the new RsqGLM function.
%Guisan, A. & Zimmermann, N.E. (2000). Predictive habitat distribution models in ecology. Ecological Modelling 135: 147-186
%

%GAM How Interpretable and Trustworthy are GAMs: 这里说明了GAM的广泛使用
%https://arxiv.org/pdf/2006.06466.pdf
%Generalized Additive Models_ An Introduction with R, Second Edition

%Feature importance
%https://stats.stackexchange.com/questions/454553/what-method-does-varimp-gam-use-in-caret-package-in-r ---- It is used for a quick, somewhat imperfect but relatively well-understood way to measure statistically significance which is itself is a reasonable proxy for variable importance. One can use more sophisticated methods like from the package iml to get more detailed info. 
%https://stats.stackexchange.com/questions/401512/hard-in-calculating-predictor-s-relative-importance-for-gam
%We used “caret” package in R (Kuhn, 2008) to derive the relative variable importance for each of the six growth stages examined.----Evaluation of within-season grapevine evapotranspiration patterns and drivers using generalized additive models
%Appendix C. Measure of relative importance  -- Generalisedadditivemodellingofairpollution,trafficvolume and meteorology MagneAldrin��,IngridHobækHaff
%Measuring Variable Importance in Generalized Linear Models for Modeling Size of Loss Distributions Therefore, the traditional ANOVA method or GAM model may also be appropriate in evaluating variable importance, but subject to its own limitation. Using a generalized additive model to quantify the influence of local meteorology on air quality in Zagreb Variable importance measures are then given by t-values of the coefficients or the reciprocal of the p-value of the t-test in testing the significance of coefficients. They can also be defined using the risk relativity of each factor. Obtaining the risk relativity from GAM is similar to the GLM, discussed in the next section. As we can see from the model setting shown in Equation (3), the GAM method is more appropriate for the numerical type of variable, including the ordinal scale of the numerical factor. This is because of the imposed functionality by fj(·). However, for a categorical variable, we are facing the same problem as the one we will see in the GLM setting. If importance is measured for a factor, we must consider an approach that can summarize the estimate from the factor levels. The common characteristic of the model-based variable importance measure, including the sensitivity measure of the variable and the GAM approach, tries to capture the association between the response variable and a function or a mathematical operation of xj.  ANOVA method or GAM model may also be appropriate in evaluating variable importance, 
%F-----1. Quantifying the influence of local meteorology on air quality using generalized additive models
%John L. Pearce a, *, Jason Beringer a, Neville Nicholls a, Rob J. Hyndman b, Nigel J. Tapper
% F-----2. Using a generalized additive model to quantify the influence of local meteorology on air quality in Zagreb Andreina Belušić, Ivana Herceg-Bulić and Zvjezdana Bencetić Klaić

%Integrating physical and empirical landslide susceptibility models using generalized additive models
%AIC:step wise---Identification of hake distribution pattern and nursery grounds in the Hellenic seas by means of generalized additive models https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.706.9796&rep=rep1&type=pdf 
%step wise---In all GAMs, variable selection proceeded by a stepwise forward entry and the Akaike Information Criterion (AIC) was used to detect the relative importance of each variable in explaining variations and determine the order of those that should be included in the final model. 
%Reconciling Performance and Interpretability in Customer Churn Prediction using Ensemble Learning based on Generalized Additive Models
% Koen W. De Bock* Dirk Van den Poel† AUC-based feature importance
%https://arxiv.org/pdf/2204.09123.pdf 提供了多个gam模型的model interpretability GAM(E) CHANGER OR NOT? AN EVALUATION OF INTERPRETABLE MACHINE LEARNING MODELS BASED ON ADDITIVE MODEL CONSTRAINTS Furthermore, EBM turns out to be the best performing GAM among all interpretable approaches showing the highest prediction qualities in 6 out of 12 datasets. For the regression tasks, it even outperformed all other white-box models and could achieve the best results on 2 out 5 datasets.

%https://shap.readthedocs.io/en/latest/example_notebooks/overviews/An%20introduction%20to%20explainable%20AI%20with%20Shapley%20values.html#Explaining-an-additive-regression-model
%shap: Explaining a generalized additive regression model

% https://ecoforecast.org/workshops/statistical-methods-seminar-series/#simpson
%https://www.youtube.com/watch?v=XQ1vk7wEI7c
%
%yGAM is an extension to linear and generalized linear models, where it could  so it could find a balance between predictive power and interpretability. nonlinear and non-monotonic relationships between the response variable and explanatory variables [21]Since the performance change is a continuous value, and relationships between the performance change and code features are not assumed to be linear, we construct a Generalized additive model (GAM) to analyze their relationships

% Although Aldrin and Haff (2005) inspected colinearity based on cor- relation coefficients solely, in the present study we additionally calculated variance inflation factor (vIF) (Zuur et al., 2009). For all variables vIF values were lower than 3, and they were ranging from about 1.0 for the day of the week (DW) to 2.4 for the relative humidity. Thus, we assumed that variables are not collinear, and that a regression method could be applied.----Using a generalized additive model to quantify the influence of local meteorology on air quality in Zagreb Andreina Belušić, Ivana Herceg-Bulić and Zvjezdana Bencetić Klaić
%Mixed Effects Models and Extensions in Ecology with R-----The resulting VIF values are given in Table 16.2. As explained in Appendix A, a cut-off value of 5 or even 3 can be used to remove collinear variables; we used 3.
% https://stats.stackexchange.com/questions/512834/can-i-have-a-coefficient-like-interpretation-of-my-y-axis-in-a-mgcvgam-plot plot explaination !!!!!!!!!
To analyze the relationship between the performance change and code features, we construct a Generalized additive model (GAM)~\cite{tan2022exploratory,hastie2017generalized}. The code features come from Section~\ref{data} and the performance changes come from Section~\ref{measurement}. Compared to linear models, it can analyze the nonlinear and non-monotonic relationships between features and the performance change~\cite{hastie2017generalized}. Compared to machine learning (ML) algorithms such as Random Forests, it is more interpretable and comparable to the ML algorithms~\cite{InterpretableGAM,GAM30days}. So, it could implement a balance between predictive power and interpretability~\cite{serven2018pygam}. Similar to previous studies~\cite{hastie2017generalized}, we first log transform highly skewed performance change and numeric code features. We use the variance inflation factor (VIF) to analyze the multicollinearity of the prediction variables~\cite{mansfield1982detecting}. If the VIF of two features is larger than 5~\cite{JSSv032b01,tan2022exploratory,articleVIFZagreb}, there is significant multicollinearity among the features, we randomly remove a feature. Finally, we build a GAM model with the feature values and performance changes provided by the package ``mgcv'' in R language. The GAM model provides deviance explained, p-values and the trend plot between the feature and performance change which could help understand whether the relationship between feature and performance change such as positive or negative relationship. The deviance explained indicates the goodness-of-fit of model. If the deviance explained is closer to 1, the better the model fits the data. Since the deviance explained indicates the proportion of deviance explained (DE) by the model, previous studies generally assume that the model can explain the data well if the deviance explained is greater than 40\%~\cite{tan2022exploratory,SCHOEMAN200267,articleVIFZagreb}. The p-value for each feature tests the null hypothesis that the feature has no correlation with the performance change. If the p-value for a feature is less than 0.05, we think the feature is significant~\cite{tan2022exploratory,SCHOEMAN200267}. Since there maybe more than one important features, we need to sort the importance of the feature. Similar to the previous study~\cite{GAM30days} that compares many measurements of feature importance and find that sorting terms works well, so we sort the features by the change of DE by removing one important feature. The rank of features in the Table~\ref{tab:relation_code_performance} presented by the feature importance.%the difference of DE between removing each important feature and a  states that aSince the methods of feature important is many, there is no one measure is correct or best, and followed by the previous studieswe find that a sort that reflects a combination of these metrics seems to work well. 
\subsubsection{Result}% Figure 1 shows the distribution of the maximum spread of each benchmark for the study subjects in violin plot notation. To ease visual comprehension, we have limited the y-axis to 1.00 for Java and 0.5 for Go, even though some projects have a small number of outlier benchmarks with even higher maxSpread.展示 deviance explained 
\begin{table}[tbp]
%\vspace{-0.2cm}
\scriptsize\caption{The interpretability of symptom features to performance change on two datasets}
  \label{tab:relation_code_performance}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l |c | c｜c | c } 
\hline
\multirow{2}{*}{Idiom}                                    & \multicolumn{2}{c|}{laboratory data} & \multicolumn{2}{c}{Field data}\\
\cline{2-5} &\begin{tabular}[c]{@{}l@{}}DE (\%) \end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}important\\ features\end{tabular}}&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}DE (\%) \end{tabular}} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}l@{}}important\\ features\end{tabular}}\\\hline

\begin{tabular}[c]{@{}l@{}}List-Com\\prehension\end{tabular}  &90.3 &\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}\\
\texttt{scope}\\
num\_If\\num\_If\_Else\end{tabular}}
& \multicolumn{1}{c|}{28.3} & \begin{tabular}[c]{@{}l@{}}-
\end{tabular}
\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Set-Comp\\rehension\end{tabular}  & 88.1&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}\\
\texttt{scope}\\
num\_For\\num\_If\\num\_If\_Else\end{tabular}} &  \multicolumn{1}{c|}{8.8} &\begin{tabular}[c]{@{}l@{}}-
\end{tabular}\\
\hline%1292
\begin{tabular}[c]{@{}l@{}}Dict-Comp\\rehension\end{tabular}  & 91.2&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}\\
\texttt{scope}\\
num\_For\\num\_If\\num\_If\_Else\end{tabular}}   & \multicolumn{1}{c|}{29.3}&\begin{tabular}[c]{@{}l@{}}-
\end{tabular}\\ 
\hline

\begin{tabular}[c]{@{}l@{}}Chain\\Comparison\end{tabular}   & 55.4&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
\texttt{scope}\\
\texttt{num\_compop}\\
\texttt{is\_true}\\\end{tabular}}   & \multicolumn{1}{c|}{19.8} &\begin{tabular}[c]{@{}l@{}}-
\end{tabular}\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Truth\\Value\\Test\end{tabular}   & 99.6&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
\texttt{scope}\\
\texttt{empty\_set}\end{tabular}}   & \multicolumn{1}{c|}{32}&\begin{tabular}[c]{@{}l@{}}-
\end{tabular}
\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Loop\\Else\end{tabular}    & 95.1&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
\texttt{size\_ele}\end{tabular}} & \multicolumn{1}{c|}{53.4} &\texttt{size\_ele}\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Assign\\Multi\\Targets\end{tabular}    & 68.6 &\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
\texttt{is\_swap}\\\texttt{scope}\\\texttt{is\_const}
\end{tabular}} & \multicolumn{1}{c|}{55.1}& \begin{tabular}[c]{@{}l@{}}num\_Assign\\
\texttt{is\_const}
\end{tabular}\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Star-in\\Func-Call\end{tabular}  & 90.9&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
num\_Subscript\\\texttt{scope}\\\texttt{is\_const}\\\texttt{has\_Subscript}\\\texttt{has\_Step}\\\texttt{has\_Upper}\\\texttt{has\_Lower}
\end{tabular}}   & \multicolumn{1}{c|}{31.9} &\begin{tabular}[c]{@{}l@{}}-\end{tabular}\\ 
\hline
\begin{tabular}[c]{@{}l@{}}For\\Multi\\Targets\end{tabular} & 88.3&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}
\texttt{has\_Starred}\\
\texttt{scope}\\
num\_Subscript\\\texttt{size\_ele}
\end{tabular}}  & \multicolumn{1}{c|}{67.8}&\begin{tabular}[c]{@{}l@{}} 
num\_Subscript\\\texttt{size\_ele}
\end{tabular}\\
\hline
\end{tabular}

\vspace{-0.3cm}
\end{table}


%https://www.statology.org/interpret-prt-regression-output-r/ p-value 
%https://stats.stackexchange.com/questions/400933/which-index-is-preferred-in-gam-r-sq-or-deviance-explained use deviance explained
Table~\ref{tab:relation_code_performance} shows the deviance explained (i.e., DE (\%) column) and important features of on laboratory dataset and field dataset.

%On the laboratory dataset,  the symptom features are enough to reflect performance change on the laboratory dataset (the deviance explained is above 50\%). However, On the real-world dataset, for the six Python idioms (list/set/dict-comprehension, chain-comparison, truth-value-test and star-in-func-call), the symptom features alone cannot reflect the performance change on the real-world dataset, which indicates many other complex factors that affect the performance change. For the loop-else, assign-multiple-targets and for-multiple-targets, the symptom features can reflect the performance change well. However, for the loop-else and for-multiple-targets, their differences in deviance explained are larger than 20\% on the two datasets, which reflect some idiomatic refactorings maybe influenced by other symptom features. 

\noindent\FiveStar \textbf{The relationship between features and performance change on the laboratory dataset:} On the laboratory dataset, we find the symptom features are enough to reflect performance change well for nine Python idioms. There are some features are significant features in all four dimensions (i.e., node, context, data and state).  The relationships between the features and the performance change are expressed as follows:

\noindent\textbf{Relationship (REL) in AST Nodes}:

\textbf{REL1-numNode}: For the list/set/dict-comprehension, we find as the numbers of For, If, If-Else nodes increase, the performance change becomes smaller. 

For the star-in-func-call and the for-multi-targets, as the number of Subscript node increases, the performance change becomes bigger.

\textbf{REL2-\texttt{nodeSet}}: For the truth-value-test, the value of comparator from \texttt{EmptySet} has a significant relationship with the performance change. For example, If the comparator is \textsf{``Fraction(0, 1)''}, the performance improvement is about 7. If the comparator is \textsf{``0, 0.0, `'}, the performance improvement is relatively small, basically less than 1.2. 


\textbf{REL3-\texttt{hasNode}}: For the star-in-func-call, the \texttt{hasSubscript}, \texttt{hasStep},  \texttt{hasUpper} and \texttt{hasLower} is negatively related to the performance change. For example, for the non-idiomatic code ``\textsf{func(e\_list[0], e\_list[1])}'', if the ``\textsf{e\_list}'' has more than two elements, the corresponding idiomatic code is ``\textsf{func(*e\_list[:2])}'' that has the subscript node ``\textsf{[:2]}'' (i.e., \texttt{hasSubscript} is 0). However, if the ``\textsf{e\_list}'' has two elements, the corresponding idiomatic code is ``\textsf{func(*e\_list)}'' that does not have the subscript node(i.e., \texttt{hasSubscript} is 0). The performance change of the idiomatic refactoring with Subscript node is less than of without the Subscript node.%For the non-idiomatic code ``\textsf{func(e\_list[0], e\_list[1])}'', the corresponding idiomatic code is ``\textsf{func(*e\_list[:2])}'' that does not have a Lower node (i.e., \texttt{has\_Lower} is 0). The performance change of the idiomatic refactoring with Lower node is less than of without Lower node.

For the for-multi-targets, the \texttt{hasStarred} is negatively related to the performance change. For example, if each element of the ``\textsf{e\_list}'' has two items, after refactoring the non-idiomatic code, the part of idiomatic code is ``\textsf{for e\_0, e\_1 in e\_list}''. However, if the element of the ``\textsf{e\_list}'' has three items, the idiomatic code is ``\textsf{for e\_0, e\_1, *e\_len in e\_list}'', where the Starred node (``\textsf{*e\_len}'') represents the remaining items of the element. The performance change of the idiomatic refactoring of code with Starred node is less than that of code without Starred node. Particularly, we observe that if there is no starred node in the idiomatic code which means that the code fetch all items of each element of the iterator, the performance generally improves. Otherwise, the performance generally decreases.

\noindent\textbf{Relationship (REL) in Variable Scope}: For the seven Python idioms ( i.e., the list/set/dict-comprehension, chain-comparison, loop-else, assign-multi-targets and star-in-func-call), the performance change in the global scope is greater than of performance change in the local scope. For the remaining two Python idioms (i.e., truth-value-test and for-multiple-targets), the performance change in the global scope is less than of performance change in the local scope.

\noindent\textbf{Relationship (REL) in Data Properties}:

\textbf{REL1-\texttt{size}}: For the list/set/dict-comprehension and for-multi-targets, the \texttt{size} represents the number of added elements and iterations, respectively. The performance change increases as the \texttt{size} increases, whereas when \texttt{size} reaches a certain degree, the value of performance change stop growing. For example, for the list-comprehension in Figure~\ref{fig:rel_rq2}), when the \texttt{size} reaches about 6 ($2.7^2-1$), the performance improves, and when the \texttt{size} reaches about 147 ($2.7^5-1$), the performance stop growing. %Particularly, the performance decreases if there is no element appended to the object. For the for-multi-targets, the \texttt{size} represents the number of iterations, the performance change increases as the number of iterations increases,  to a certain degree, the performance change remains stable.gradually becomes bigger, and finally the performance change .
%*********R语言plot的figure size set up**********************
%https://stackoverflow.com/questions/2129952/creating-a-plot-window-of-a-particular-size
%https://stackoverflow.com/questions/38112879/how-to-change-the-y-axis-on-mgcv-gam-factor-plots
%*********mgcv gam relationship explaination**********************
%https://stats.stackexchange.com/questions/512834/can-i-have-a-coefficient-like-interpretation-of-my-y-axis-in-a-mgcvgam-plot 
%
%Rplots_spline_change_y.pdf
\begin{figure}
  \centering
  \includegraphics[width=3.4in,height=1.5in]{./data/list_compre_rel_new.png}%performance_rq1_compare_boxplot_new_2.pdf.Rplots_spline_change_y.pdf rq1_perf_change_box_plot.png
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{The relationship between size and performance change for list-comprehension}
    
    \label{fig:rel_rq2} 
    \vspace{-0.6cm}
    %\vspace{-0.6cm}
\end{figure}

For the loop-else, the \texttt{size} represents the number of iterations. As the number of iterations increases, the performance improvement gradually becomes smaller, and finally the performance change stop decreasing and is close to 1, which is basically unchanged.

\textbf{REL2-\texttt{isSwap}}: For the assign-multi-targets, the performance change of idiomatic refactorings for swapping variables is greater than of idiomatic refactorings for not swapping variables.

\textbf{REL3-\texttt{isConst}}: For the star-in-fun-call, the performance change of constant index of Subscript node is greater than of non-constant index of Subscript node. For example, the index is constant for the ``\textsf{func(e\_list[0], e\_list[1])}'' code, and the index is non-constant for the ``\textsf{func(e\_list[i], e\_list[i+1])}'' code. After code refactoring, the performance change of code of constant index is greater than of code of non-constant index.

For the assign-multi-targets, the performance change of the idiomatic refactoring of constants assignment is greater than of the idiomatic refactoring of variables assignment. 

\noindent\textbf{Relationship (REL) in Execution Path}:

\textbf{REL1-\texttt{isTrue}}: For the chain-compare, the \texttt{isTrue} is positively related to the performance change. For example, if ``\textsf{n, o, p}=1, 2, 3'', the value of ``\textsf{n <= o and o > p}'' is ``\textsf{True}'' (code1). However, if ``\textsf{n, o, p}=3, 1, 2'', the value of ``\textsf{n <= o and o > p}'' is ``\textsf{False}''. After refactoring the code, the performance change of the code1 is greater than of the code2. 


% \noindent\FiveStar \textbf{Unintuitive features: }Although some features have no significant relationship with the performance change, we find they are unintuitive. These features are in one dimension: node.

% \textbf{REL1-num\_Assign:} We find the number of assignment node has no significant relationship with the performance change, which is a bit counterintuitive. Since no matter how many assignment statements a non-idiomatic code has, the corresponding idiomatic code has only one assignment statement. It seems the more assignment statements, the greater the performance change but we find their performance changes basically are the same. 

% \textbf{REL2-{eq\_set}:} For the truth-value-test, the node kind of operator has no statistically significant relationship with performance change, which is a little unintuitive. For example, for two non-idiomatic code fragments: \textsf{``if a != []''} and \textsf{``if a == []''}, their corresponding idiomatic codes are \textsf{``if a''} and \textsf{``if not a''}. Although \textsf{``if not a''} has one more \textsf{``not''} than \textsf{``if a''}, their performance changes are basically the same.

 %We observe that if the code is to swap variables in the global scope, the performance basically improves. If the code is to swap variables in the local scope, when swapping two variables, the performance basically improves, otherwise the performance decreases. If the code is only assign the variables instead of swap variables, the performance basically decreases.

\noindent\FiveStar \textbf{The relationship between features and performance change on the field dataset:} On the real-world dataset, the models of the three Python idioms (i.e., loop-else, assign-multiple-targets and for-multiple-targets) could fit the data well. Their important features are also the important features on the laboratory dataset. For the \texttt{scope}, \texttt{isSwap} and \texttt{hasStarred} are not the important features on the field dataset because their features are the same on the codes of field dataset. For the \texttt{scope}, all variables on the field dataset are in the local scope. For the \texttt{isSwap} of assign-multi-targets, all codes of assign-multi-targets are to assign values instead of swapping the variables. For the \texttt{hasStarred} of for-multi-targets, since the length of iterator cannot be known through static analysis, to ensure the correctness of code refactoring, all idiomatic codes on the field dataset have the Starred node. Particularly, for the assign-multi-targets, the \texttt{num\_Assign} is the important feature on the synthetic dataset but is not the important feature on real-project dataset. 

For the six Python idioms (list/set/dict-comprehension, chain-comparison, truth-value-test and star-in-func-call), we find their models cannot fit the data well which indicates that symptom features alone cannot reflect the performance change and many other complex factors may affect the performance change on the field dataset. Table\ref{tab:rq3_example} shows examples for the six Python idioms.

For example, for the list-comrehension, although the \texttt{size} is the most significant feature on the synthetic dataset, the number of elements can also has little effect on performance change. At the list-comprehension row of Table~\ref{tab:rq3_example}, the two code pairs of two datasets basically have the same features such as number of For node and number of added elements. However, the performance improvement on the laboratory dataset (2.87) is significantly larger than of field data (1.03).performance improvement one the field data is only 1.03 but the performance improvement on the laboratory data is 2.87. 

For another example, for the truth-value-test, testing whether a comparator is equal to ``\textsf{0}'' in \texttt{EmptySet} on the synthetic dataset makes the performance improvement is little (<2), but on the real-project dataset, the performance improvement maybe large. At the truth-value-test row of Table~\ref{tab:rq3_example}, the two code pairs on two datasets are basically same, but the performance improvement on the synthetic dataset (1.05) is significantly less than of real-project data (11.8).

 \noindent\fbox{\begin{minipage}{8.4cm} \emph{Among nine Python idioms, for three Python idioms (loop-else, assign-multi-targets and for-multi-targets), the code features can reflect the performance change on two datasets well. Their performance changes are related to features from Data Properties (\texttt{size}, \texttt{IsConst}) and AST Nodes (numSubscript). However, on real-project dataset, the performance of remaining six Python idioms is impacted by other complex factors.} \end{minipage}}
%For the loop-else, assign-multiple-targets and for-multiple-targets, the symptom features can reflect the performance change well. However, for the loop-else and for-multiple-targets, their differences in deviance explained are larger than 20\% on the two datasets, which reflect some idiomatic refactorings maybe influenced by other symptom features. 







%https://www.cnblogs.com/traditional/p/13538919.html 深度剖析Python Interpreter（if/for/exception）
%https://cloud.tencent.com/developer/article/1678615 POP_JUMP_IF_FALSE 指令解析
%https://stackoverflow.com/questions/49735639/in-python-why-is-explicit-bool-much-slower-than-implicit 
\subsection{RQ3: What are the root causes of performance change of idiomatic refactorings on the two datasets?}
\subsubsection{Motivation}
 In the previous two research questions, we find that code refactoring with the same Python idiom could improve or decrease performance on the two datasets. And the relationship of code features and performance change of laboratory dataset may not align with that of real-world dataset. Therefore, in this research question, we would like to understand the root causes that different code have different effects on performance change for each Python idiom on the two datasets.% The findings can assist help developers practition- ers in avoiding the use of certain tests in performance assurance activities and in improving tests to serve as performance tests.
\subsubsection{Approach}
To explore the reason for performance change
caused by idiomatic refactorings for each Python idiom, it is not reliable to compare the difference of source code between idiomatic code and the corresponding non-idiomatic code because Python interpreter does not directly execute the source code. When the Python code runs, source code first gets compiled into a set of instructions called bytecode. Then the bytecode is executed by the Python interpreter. Therefore, we first get the bytecode instructions of idiomatic code and the corresponding non-idiomatic code for each Python idiom with dis module~\cite{dis_python} which supports the analysis of CPython bytecode by disassembling it. Then we compare their difference in instructions to understand the reasons of performance change.
%说明为什么用字节码解释 source code 执行的过程https://legacy.python.org/workshops/1998-11/proceedings/papers/montanaro/montanaro.html，用字节码解释的方法过程 字节码每个meta的概念https://github.com/python/cpython/blob/main/Doc/library/dis.rst

%RQ3 root causes (in both lab and real-world setting, the change by refactoring at the byte-code level are the same, but real-world code involves ……)
% %RQs take-home message and discussion: 
% Refactoring local impact (consider only the code affected by refactoring) are the same in the lab versus real-world setting, but real-world involves many complex context, interweaving ???? which may balance off the improvement by refactoring

% https://towardsdatascience.com/list-comprehensions-vs-for-loops-it-is-not-what-you-think-34071d4d8207
%https://stackoverflow.com/questions/58844643/why-is-my-list-comprehension-function-slower-than-my-list-appending-function-for
%https://www.17tr.com/tool/term/1359708.shtml SOR
\subsubsection{Result}

\noindent\FiveStar \textbf{The bytecodes of idiomatic code and non-idiomatic code are different}. Four differences in bytecodes of the idiomatic refactoring as follows:

\begin{table*}[htbp]
%\vspace{-0.2cm}
\caption{the performance change of code examples of nine Python idioms in the field code}
  \label{tab:rq3_example}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l| l| l| c| c} 
\hline
Idiom&non-idiomatic code  & idiomatic code   & code feature &X\\ \hline

\multirow[b]{2}{*}{\href{https://github.com/kellyjonbrazil/jc/blob/e2f1b16cb9e920968c093bd1f371b191aa7107bf/jc/parsers/csv.py#L145-L146}{list-compre}} & \begin{tabular}[c]{@{}l@{}} raw\_output=[]\\for row in reader:\\    \ \  raw\_output.append(row)\end{tabular} & \begin{tabular}[c]{@{}l@{}}raw\_output = [row \\for row in reader]\end{tabular} &\texttt{size\_ele}:11,766& 1.03\\ 
\cline{2-5} & \begin{tabular}[c]{@{}l@{}} l=[]\\for e\_0 in x\_0:\\    \ \  l.append(e\_0)\end{tabular} & \begin{tabular}[c]{@{}l@{}}l=[e\_0 for e\_0 in x\_0]\end{tabular} &\texttt{size\_ele}:10,000& 2.87\\ \hline
% \href{https://github.com/sympy/sympy/blob/82f264c62db6382fd3545bb43f57584b0f4e27c2/sympy/combinatorics/testutil.py#L195-L197}{set-compre} & \begin{tabular}[c]{@{}l@{}} conjugates = set()\\for el in group.generate\_dimino():
% \\   \ \ for gen in subgr\_gens:
% \\   \ \    \ \      conjugates.add(gen $\wedge$ el)\end{tabular} & \begin{tabular}[c]{@{}l@{}}conjugates = \{gen $\wedge$ el\\ for el in group.generate\_dimino() \\for gen in subgr\_gens\}\end{tabular} &\texttt{size\_ele}:44& 1.008\\ \hline
\multirow[b]{2}{*}{\href{https://github.com/sympy/sympy/blob/429f5be2be5bdc5ee8d717ff857a3268b9c91e40/sympy/ntheory/residue_ntheory.py#L885-L887}{set-compre}} & \begin{tabular}[c]{@{}l@{}} r = set()\\for i in range(p // 2 + 1):\\
    \ \ r.add(pow(i, 2, p))
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
r = \{pow(i, 2, p) for i in range(p // 2 + 1)\}\end{tabular} &\texttt{size\_ele}: 10& 1.04\\ 
\cline{2-5}&\begin{tabular}[c]{@{}l@{}} l = set()\\
for e\_0 in x\_0:\\
    \ \ l.add(e\_0)
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
l = \{e\_0 for e\_0 in x\_0\}\end{tabular} &\texttt{size\_ele}: 10&  1.60\\ 

\hline


\href{https://github.com/networkx/networkx/blob/7b30f1a814d6b7f1b3c4311d19c251b8098d1407/networkx/algorithms/community/quality.py#L299-L302}{dict-compre} & \begin{tabular}[c]{@{}l@{}} rv = \{\}\\for (k, v) in d.items():\\
\  \    rv[k] = v.\_\_self\_\_\end{tabular} & \begin{tabular}[c]{@{}l@{}}rv = \{k: v.\_\_self\_\_ for (k, v) in d.items()\}\end{tabular} &\texttt{size\_ele}:1,000& 1.004\\ 
\cline{2-5} & \begin{tabular}[c]{@{}l@{}} l = dict()\\
l = {e\_0: e\_0 for e\_0 in x\_0}\end{tabular} & \begin{tabular}[c]{@{}l@{}}
l = \{e\_0: e\_0 for e\_0 in x\_0\}\end{tabular} &\texttt{size\_ele}:1,000& 1.09\\
\hline

\multirow[b]{2}{*}{\href{https://github.com/brainix/pottery/blob/c7be6f1f25c5404a460b676cc60d4e6a931f8ee7/pottery/deque.py#L56}{chain-comparison}} & \begin{tabular}[c]{@{}l@{}} self.maxlen is not None and \\ current\_length >= self.maxlen\end{tabular} & \begin{tabular}[c]{@{}l@{}}None is not self.maxlen <= current\_length\end{tabular} & \texttt{scope}: in the function& 1.3\\ 
\cline{2-5} & \begin{tabular}[c]{@{}l@{}} n != o and o >= p\end{tabular} & \begin{tabular}[c]{@{}l@{}}n != o >= p\end{tabular} & \texttt{scope}: in the function& 0.97\\
\hline

\multirow[b]{2}{*}{\href{https://github.com/nipy/nibabel/blob/225892af18d82b9a91ab63a9d072b894588b670e/nibabel/volumeutils.py#L940}{truth-value-test}} & \begin{tabular}[c]{@{}l@{}} if inter != 0:\end{tabular} & \begin{tabular}[c]{@{}l@{}}if inter:\end{tabular} &comparator:0& 11.8\\

\cline{2-5} & \begin{tabular}[c]{@{}l@{}} if a != 0:\end{tabular} & \begin{tabular}[c]{@{}l@{}}if a:\end{tabular} &comparator:0& 1.05\\\hline

% \href{https://github.com/quantumlib/OpenFermion/blob/5ef58b507270f18627ec563a43001c404cf5e6c1/src/openfermion/measurements/fermion_partitioning.py#L276-L282}{loop-else} & \begin{tabular}[c]{@{}l@{}} success\_flag = True\\
%     for divisor in range(2, num\_bins - 1):\\
%     \ \     if trial\_size \% divisor == 0:\\
%         \ \ \ \     success\_flag = False\\
%         \ \ \ \     break\\
%     if success\_flag:\\
%       \ \  return trial\_size\end{tabular} & \begin{tabular}[c]{@{}l@{}}
%     for divisor in range(2, num\_bins - 1):\\
%     \ \     if trial\_size \% divisor == 0:\\
%         \ \ \ \     break\\
%     else:\\
%       \ \  return trial\_size\end{tabular} &iterations:<10& 1.3\\ \hline
       
% \href{https://github.com/Erotemic/ubelt/blob/cdb6aa9dea7567ce742ee6a11d8a1ca4ac89f342/ubelt/util_cache.py#L497-L501}{assign-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
% cfgstr = self.\_rectify\_cfgstr(cfgstr)\\
% dpath = self.dpath\\
% fname = self.fname\\
% verbose = self.verbose
% \end{tabular} & \begin{tabular}[c]{@{}l@{}}
%     cfgstr , dpath , fname , verbose  = \\ self.\_rectify\_cfgstr(cfgstr), self.dpath,\\ self.fname, self.verbose\end{tabular} &num\_assign:4& 0.78\\ \hline

\multirow[b]{2}{*}{\href{https://github.com/maxpumperla/elephas/blob/c474bb4f2565185dfd89fd06a8fe467fa9c64b2b/elephas/mllib/adapter.py#L13-L14}{star-in-func-call}} & \begin{tabular}[c]{@{}l@{}} 
func(np\_array.shape[0], np\_array.shape[1])
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
    func(*np\_array.shape[:2])\end{tabular} &num\_subscript:2& 1.004\\ 
  \cline{2-5}
% \href{https://github.com/gugarosa/opytimizer/blob/f3e110cdc7fb8557d7e041737d3c9fd63f375c1e/opytimizer/visualization/surface.py#L39}{star-in-func-call} 
& \begin{tabular}[c]{@{}l@{}} 
func(e\_list[0], e\_list[1])
\end{tabular} & \begin{tabular}[c]{@{}l@{}}
 func(*e\_list[:2])\end{tabular} &num\_subscript:2& 0.77\\ \hline

% \href{https://github.com/networkx/networkx/blob/e0c055a3524f583b60c89ea5d72a3b624212f357/networkx/algorithms/community/quality.py#L327}{for-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
% for e in G.edges():\\
% \ \     e[0]\\
% \ \     e[1]
% \end{tabular} & \begin{tabular}[c]{@{}l@{}}
%     for  (e\_0, e\_1, *e\_len) in G.edges():\\
% \ \     e\_0\\
% \ \     e\_1\end{tabular} &num\_subscript:2& 0.9\\ \hline

% \href{https://github.com/alichtman/shallow-backup/blob/d71b903dacd5eeea9d0be68ef3022817f9bac601/shallow_backup/backup.py#L81-L84}{for-multi-tars} & \begin{tabular}[c]{@{}l@{}} 
% for pacman\_option in \\pacman\_options.values():\\
% \ \     pacman\_option[0]\\
% \ \     pacman\_option[1]
% \end{tabular} & \begin{tabular}[c]{@{}l@{}}
%     for  (pacman\_option\_0, pacman\_option\_1, *pac-\\man\_option\_len)  in pacman\_options.values():\\
% \ \     pacman\_option\_0\\
% \ \     pacman\_option\_1\end{tabular} &num\_subscript:2& 0.33\\ \hline
\end{tabular}
\vspace{-0.3cm}
\end{table*}


\noindent $\bullet$\textbf{Python idioms add new bytecodes which could decrease the performance.} The corresponding Python idioms are list/set/dict comprehension, star-in-fun-call, for-multi-targets and assign-multi-targets. 

For the list/set/dict comprehension, they need to additionally execute instructions of calling comprehension code object before code iteration (red dotted box in Figure~\ref{fig:bytecode_list_compre}). Therefore, if there is no elements appended, the performance decreases. 
%the ``\textsf{=}'' does not have the corresponding bytecodes, so the more assign statements will not add costs. Furthermore, 
\begin{figure}
  \centering
  \includegraphics[width=3.5in]{./data/rq4_bytecode.png}%performance_rq1_list_compre.pdf
\setlength{\abovecaptionskip}{-0.1cm}
    \caption{Bytecode instructions of idiomatic refactorings of list comprehension}
    
    \label{fig:bytecode_list_compre} \vspace{-0.3cm}
    %\vspace{-0.6cm}
\end{figure}

For the star-in-func-call, if it accesses part of elements of the object, it needs to execute \textsf{``BUILD\_SLICE''} to build slice object.%the non-idiomatic code replaces the multiple use of instructions of accessing the element by index (loading the object and the index, and getting the element) with the instructions of building slice (\textsf{``BUILD\_SLICE''}).

The for-multi-targets needs to execute the unpacking instruction and then multiple instructions of storing unpacked values. % storing multiple values. Since the cost of unpacking the object is larger than of accessing the element by index, only if the number of Subscript nodes of non-idiomatic code increases to a certain value (about 5), the performance probably improve.

For the assign-multi-targets, if there are multiple values for one assign statement, to assign each value to the corresponding target it needs to additionally execute instructions of building a tuple (\textsf{``BUILD\_TUPLE''}) and unpacking the sequences (\textsf{``UNPACK\_SEQUENCE''}) to put values onto the stack right-to-left. Therefore, if the assign-multi-targets are only to assign variables, the performance decreases. And as the number of assign nodes increases, the \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''} needs to operate more values, the slower performance. If the assign-multi-targets is to swap two or three variables, they use \textsf{``ROT\_TWO''} and \textsf{``ROT\_THREE''} to directly swap variables instead of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. 



\noindent $\bullet$\textbf{Python idioms use the specialized bytecode to replace a series of bytecodes of non-idiomatic code which could improve the performance.} They are list/set/dict-comprehension. For the list/set comprehension, they use the specialized add instructions
to reduce the cost of a series of instructions of loading objects and calling function. For example, for the list comprehension (green dotted box in Figure~\ref{fig:bytecode_list_compre}), the non-idiomatic code needs to execute ``\textsf{LOAD\_*}'' instructions to push data into the stack and then call function to append the element, but the idiomatic code only needs to execute the ``LIST\_APPEND'' instruction to append the element. Since the cost of ``\textsf{LIST\_APPEND}'' is less than that of a series instructions especially the expensive function call instruction for the non-idiomatic code, the performance can improve. As the number of added elements (\texttt{size}) increases, the greater the difference in cost of bytecodes instruction, the performance change will increase. When the \texttt{size} increases to a certain value, the performance change will stop 
growing because it makes the cost of code outside the For node (e.g., list creation and data preparation before iterating) trivial and approximately equals the cost of for body of the non-idiomatic code divided by the cost of for body of the idiomatic code. 


Different from the list/set-comprehension, for the dict comprehension, the non-idiomatic code does not need to execute the instruction of function call. Although the \textsf{``MAP\_ADD''} of dict-comprehension reduce the cost of loading the dictionary iterable, the \textsf{``MAP\_ADD''} achieves basically the same thing as the instruction to store key-value pairs of non-idiomatic code. Therefore, the performance improvement of dict comprehension (the maximum of performance improvement is less than 2) is significantly smaller than that of list/set comprehension. %\textsf{``STORE\_SUBSCR''} (

% % There are chain-compare, star-in-fun-call, for-multi-targets.
\noindent $\bullet$\textbf{Python idioms replace bytecodes of non-idiomatic codes with other bytecodes which could improve performance or decrease performance depend on the specific code.} It is the chain-compare which replaces one instruction to load the comparator of non-idiomatic code with the instructions to create a reference to a comparator (\textsf{``DUP\_TOP''}) and reference shuffling (\textsf{``ROT\_THREE''}). Saving an extra reference to the comparator for the chained comparison isn't literally free, it is slightly more expensive than loading a local variable. Therefore, if the comparator is a variable in the local scope, the performance decreases. Otherwise, if the comparator is a global variable, attribute access or the function call, the performance improves. For example, at the the 2nd sub-row of chain-compare of Table~\ref{tab:rq3_example}, ``o'' is a local variable, so the performance decreases by 0.97X. However, the 1st sub-row in the chain-compare of Table~\ref{tab:rq3_example}, \textsf{``self.maxlen''} is an attribute access, the performance improves by 1.3X. 

%https://stackoverflow.com/questions/59056097/is-the-sequence-of-opcodes-binary-subscr-get-iter-somehow-optimized-in-cpytho Indexed access is just slow (loading the sequence, the index, executing a BINARY_SUBSCR over and over, which has to unpack the index each time), and making shallow copies of a list is (comparatively) fast
%https://pyjion.readthedocs.io/en/latest/opt/opt-7.html. BINARY_SUBSCR
%https://stackoverflow.com/questions/52294373/how-to-find-the-implementation-of-1-reversing-list-in-python-in-cpython list[...] is using indexing, or more accurate subscription syntax,
%BUILD_SLICE() bytecode operation takes the top-three elements from the stack (put there by LOAD_CONST operations at indices 2, 4 and 6) to build a slice() object, which is then passed to the list object (next on the stack) with BINARY_SUBSCR. That last bytecode is the Subscript() operation in the AST, and the bytecodes 2-8 are the Slice() object in the AST.
% For the star-in-fun-call, if it accesses part of elements of the object, the non-idiomatic code replaces the multiple use of instructions of accessing the element by index (loading the object and the index, and getting the element) with the instructions of building slice (\textsf{``BUILD\_SLICE''}). The \textsf{``BUILD\_SLICE''} is not cheap (taking the top-three elements from the stack and then build a slice object), which is more expensive than the instruction of accessing the element by index if the object is a variable. Therefore, if the number of Subscript nodes of non-idiomatic is few (<4) and the object is a variable, the performance decreases. Otherwise, the performance improves. For example, the 2nd sub-row in the star-in-fun-call of Table~\ref{tab:rq3_example}, the non-idiomatic code has two Subscript nodes (``\textsf{e\_list[0], e\_list[2]}'') and the ``e\_list'' is a variable, which causes 0.77X regression of performance. However, at 1st sub-row in the star-in-fun-call of Table~\ref{tab:rq3_example}, although the non-idiomatic code has two Subscript nodes but the iterable is an attribute access which is 1.004X faster than the non-idiomatic code. 
%  When the number of Subscript nodes increases to a certain value, the performance could improve. 




% For the assign-multi-targets, if it is to assign constant values or to swap variables, they replace bytecodes of loading objects with bytecodes of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. For the constant assignment, the idiom could uses one ``\textsf{LOAD\_CONST}'' to load the multiple constants. For the swapping variables, the idiom reduces the bytecodes of loading and storing temporary variables. However, the idioms needs to build the tuple and unpacking the sequence for all values, which are more expensive than of cost of loading more variables for the non-idiomatic code. To reduce such cost of the idiom, for swapping two variables, it executes the cheaper instruction (\textsf{``ROT\_TWO''}) to directly swap variables instead of building and unpacking the tuple, so swapping two variables can improve performance. Otherwise, the performance generally decreases.

\textbf{Python idioms remove byte codes non-idiomatic codes which could improve the performance.} There are truth-value-test, loop-else, assign-multi-targets, star-in-fun-call and for-multi-targets. The truth-value-test reduces the cost of loading the object from \texttt{empty\_set} and comparison operation. The loop-else reduces the cost of assigning the flagging variables and comparison operation for the flagging variables. If the assign-multi-targets is to assign constant values, it removes multiple use of instruction to load constant. If the assign-multi-targets is to swap variables, it remove multiple use of instruction to load and store temporary variables. The star-in-fun-call and for-multi-targets remove multiple use of instructions to access an element by the index. %The for-multi-targets removes%Besides, if i that accesses all items of the object, it removes the multiple use of instructions to access an element by the index. For 
%Otherwise, there is no obvious %but the non-idiomatic code(>8) uses each ``\textsf{LOAD\_CONST}'' to load a constant each time. Therefore, the performance change of the constant assignment is greater than that of variable assignment. Howeverit replaces instructions of loading multiple constants with  In the case,  Therefore, the performance change of the constant assignment is greater than that of variable assignment.  Since the cost of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''} is larger than of ``\textsf{LOAD\_CONST}'', as the number of values increases to a certain value (>8), the cost can balance off the cost of  of assign-multi-targets and makes the assign-multi-targets performance improve. If it is to swap variables, it replaces  and star-in-func-call, it reduces the cost of 








%The reason of the positive relationship of \texttt{size\_ele} with the performance change is that the list/set comprehension replaces the instructions of loading the iterator and calling function with a specific instruction of appending elements. For example, for the idiomatic code of list comprehension, to appending a element to the list, developers replace the instructions of loading the list and calling the append function with the \textsf{``LIST\_APPEND''} (green dotted box in Figure~\ref{fig:bytecode_list_compre}). Each iteration, the non-idiomatic code executes instructions of function call, but the corresponding idiomatic code only needs to execute the \textsf{``LIST\_APPEND''} instruction for appending elements, so as more elements are appended, the greater the performance change. When the number of added element exceeds a certain value, the performance change basically no longer increases, which is approximately the cost of instructions of function call divided by the cost of the \textsf{``LIST\_APPEND''} instruction.


\noindent\FiveStar \textbf{Reasons of the nonalignment of performance change on two datsets} as follows:

\begin{itemize}[fullwidth]
\item \textbf{External objects (non-Python built-in objects) overloads Python built-in methods that executed by bytecodes, which make the performance improve or decrease}. There are three bytecodes: iterating elements (\textsf{FOR\_ITER}), compare operation (\textsf{COMPARE\_OP}) and testing the truthiness (\textsf{POP\_JUMP\_IF\_TRUE} or \textsf{POP\_JUMP\_IF\_FALSE}). 

\ \ The cost of \textsf{``FOR\_ITER''} varies with different code. Each iteration, when Python interpreter executes \textsf{``FOR\_ITER''} to get the next item of the object, it needs to call \textsf{``\_\_next\_\_()''} method. Therefore, if the object is not the Python built-in type and its cost of the self-implemented \textsf{``\_\_next\_\_()''} is large, which may balance off the improvement of Python idioms. For example, at the 1st sub-row of list-comprehension Table~\ref{tab:rq3_example}, the \textsf{``reader''} is a reader object from csv library, which overloads the \textsf{``\_\_next\_\_()''} method. Since the cost of \textsf{``\_\_next\_\_()''} is larger than the cost of \textsf{``append''} method of list, the performance improvement is only 1.03.

% \ \  For the truth-value-test, developers overload the methods of the compare operation (``\textsf{COMPARE\_OP}'') or the instruction of  testing the top item of the stack is true or not (\textsf{``POP\_JUMP\_IF\_TRUE''} or \textsf{``POP\_JUMP\_IF\_FALSE''}), which make performance may improve or decreases. 

\ \  For the compare operation, library developers usually make the cost larger than of Python implementation for special reasons (e.g., multiple elements comparison), which may make performance largerly improves. For example, the 1st sub-row of truth-value-test in Table~\ref{tab:rq3_example}, the \textsf{``inter''} is the array object of numpy library, since the numpy overload the compare operation and needs to do a series of dispatching, type conversion, and wrapper object allocation that doesn't happen when working with Python built-in objects such as list, the large cost of the compare operation make the performance improves a lot and more than ten times. 

\ \  When Python interpreter executes the instruction to test the truthiness of value, it calls the \textsf{``\_\_bool\_\_()''} method or \textsf{``\_\_len\_\_()''} method if the object is not bool data type. Therefore, if the object is not Python built-in data type, the implementation of \textsf{``\_\_bool\_\_()''} and \textsf{``\_\_len\_\_()''} may largely impact the performance. For example, for the \href{https://github.com/searx/searx/blob/5b50d7455a719b145be5f90069026a60b480673d/searx/utils.py#L259}{\textsf{``xpath\_results == []''}} code, the \textsf{``xpath\_results''} is \textsf{``HtmlElement''} from lxml library, it defines the \textsf{``\_\_bool\_\_''} method ineffectively which make the performance decreases largely and less than 0.2. And we find that the developers may improve the implementation of  \textsf{``\_\_bool\_\_''} method because its source code has a warning: the method will change in future versions. 

%list/set/dict, for-else
\item \textbf{Code on the real-project dataset uses more complex code (i.e., function calls, attribute access and compounding of expressions and additional statements) which make performance impact small.} For example, at the 1st sub-row of set-comprehension in Table~\ref{tab:rq3_example}, instead of simply adding a variable to the ``\textsf{conjugates}'', this code adds a binary operator expression ``\textsf{
gen \^ el}'' that balance off the benefits of set-comprehension, so the performance improvement is small (<1.04X speedup). %For another example, at the 1st row of the chain-comparison row of Table~\ref{tab:rq3_example}, the chained comparator is not a simple variable but is an attribute access ``\textsf{self.maxlen}''. The cost of creating reference and shuffling reference is less than of  attribute access, which make the performance improvement.


\end{itemize}

 \noindent\fbox{\begin{minipage}{8.4cm} \emph{A Python idiom may improve or decrease performance because it exists both bytecode addition and bytecode remove, the replacement of bytecodes, and overloading methods by developers. The little performance impact of a Python idiom is because using the complex code balances off the performance impact of Python idioms.} \end{minipage}}
%why generator或者非内置的object slower 有https://www.programiz.com/python-programming/generator
%https://www.programiz.com/python-programming/iterator

% For one thing, each iteration, when Python interpreter executes \textsf{``FOR\_ITER''} to get the next item of the iterator , it needs to call \textsf{``\_\_next\_\_()''} method. Therefore, if the iterator is not the Python built-in type and its cost of the self-implemented \textsf{``\_\_next\_\_()''} is large, which could balance off the improvement of list/set/dict comprehension. For example, for the code of the 1st row of Table~\ref{tab:rq3_example}, the \textsf{``reader''} is a reader object from csv library, which overloads the \textsf{``\_\_next\_\_()''} method. Since the cost of \textsf{``\_\_next\_\_()''} is larger than the cost of \textsf{``append''} method of list, the performance improvement is only 1.03.

% \begin{figure}
%   \centering
%   \includegraphics[width=3.5in]{./data/rq4_bytecode.png}%performance_rq1_list_compre.pdf
% \setlength{\abovecaptionskip}{-0.1cm}
%     \caption{Bytecode instructions of idiomatic refactorings of list comprehension}
    
%     \label{fig:bytecode_list_compre} \vspace{-0.3cm}
%     %\vspace{-0.6cm}
% \end{figure}


%the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants.The greater performance improvement of idiomatic refactorings with function call comparator (e.g., \textsf{``Fraction(0,1)''} and \textsf{``dict()''}) instead of basic data types because the cost of \textsf{``CALL\_FUNCTION''} instruction is greater than the cost of loading variables or constants.%  instruction rather than instructions of loading variables or constants, the differences in performance change of idiomatic refactorings will be greater, so the performance improvement will be greater. 

% The instructions of \textsf{``if not object''} and \textsf{``if object''} idiomatic codes are almost same because the corresponding instructions are \textsf{``POP\_JUMP\_IF\_FALSE''} and \textsf{``POP\_JUMP\_IF\_TRUE''}, respectively. Therefore,  although the comparison operators \textsf{``==''} and \textsf{``!=''} have no difference is that their instructions are to test the top item of the stack is true or not. Specifically, the instruction \textsf{`object''} of test node is  \textsf{``POP\_JUMP\_IF\_FALSE''}, and for the \textsf{``not object''}, Python interpreter will automatically compiles it \textsf{``POP\_JUMP\_IF\_TRUE''} and does not need to execute extra instructions. Therefore, although the comparison operators \textsf{``==''} and \textsf{``!=''} have different number of tokens, their performance changes are basically the same.

%https://github.com/hemildesai/numpy/blob/6fbbadb676dfa7cee56be3bd17b92bde661f8869/numpy/core/numeric.py#L363-L372 built-in method ``__nonzero__()`` (renamed ``__bool__()`` in python3.x
%https://github.com/lxml/lxml/blob/c742576c105f40fc8b754fcae56fee4aa35840a3/src/lxml/etree.pyx#L2500-L2507
%https://github.com/numpy/numpy/blob/4cbced22a8306d7214a4e18d12e651c034143922/doc/source/reference/arrays.ndarray.rst numpy是因为对==的重载
%Particularly, when there are only two variables, the idiomatic code uses the \textsf{``ROT\_TWO''} instruction to complete the assignment to reduce the performance regression. 

%Therefore, the swappuse the The reason of performance regression of variable assignment code refactorings is that the extra cost of instructions of building a tuple for multiple values (\textsf{``BUILD\_TUPLE''}) and unpack the tuple (\textsf{``UNPACK\_SEQUENCE''} ).  For example, for the code in the 8th row of Table~\ref{tab:rq3_example}, the non-idiomatic code has four assignment node but the idiomatic code only has one assignment node, so it seems that the idiomatic code may improve performance. However, the (\textsf{``=''}) has no real byte code instructions and one assignment statement consists of instructions of loading objects and storing objects. The non-idiomatic code loads one object and then stores one object each time. While the idiomatic code first loads four objects four times. For assigning values into targets correctly, idiomatic code then executes two extra instructions \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''} to put values onto the stack right-to-left. Finally, the idiomatic code stores four objects four times. Therefore, the idiomatic refactorings of assign-multiple-targets actually decrease the performance.

% The reason of performance improvement of code of swapping variables in the global scope is that the cost of instructions of loading and storing global temporary variables is larger than instructions of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. However, when variables are in the local scope, the cost of instructions of loading and storing local temporary variables is generally less than of instructions of \textsf{``BUILD\_TUPLE''} and \textsf{``UNPACK\_SEQUENCE''}. Particularly, when the idiomatic code is to swap two variables in the local scope, the performance improves because Python developers design an instruction \textsf{``ROT\_TWO''} to quickly swap two variables on the stack.

% The reason of performance improvement of code of constant assignment code with more than about 8 constants is that the idiomatic code directly loads all constants once as a tuple (\textsf{``LOAD\_CONST''}) and then unpacks the tuple (\textsf{``UNPACK\_SEQUENCE''}) rather than loading a constant at a time like the non-idiomatic code. When the number of constants is larger than 8, the cost of \textsf{``UNPACK\_SEQUENCE''} is generally larger than of  8 \textsf{``LOAD\_CONST''} instructions.

 %First, when the code is to fetch all elements of the iterator, the idiomatic code does not need to execute the \textsf{``BUILD\_SLICE''}, so the performance improves. Second, 



%The reason of performance change of code in the global scope is greater than of code in the local scope is that the cost of loading global variables is greater than of loading local variables. And the reason of performance change of the variable index is greater than of the constant index is that the cost of loading variables is greater than of loading constants. 
%https://blog.csdn.net/woshaguayi/article/details/108484328
%If the to The difference in bytecode instructions of idiomatic code and idiomatic code is that the body of non-idiomatic code needs to accessing elements at specified indices (\textsf{``LOAD\_CONST''} and \textsf{``BINARY\_SUBSCR''}) but the idiomatic code does not do it. Therefore, when the code unpacks all elements, the performance will improve the performance. However, if the code unpacks part of elements, each iteration the idiomatic code needs to store an extra variable, e.g., the \textsf{``*x\_len''} variable in the the last row of the Table~\ref{tab:rq3_example}, the performance will decrease.

% The cost of \textsf{``FOR\_ITER''} varies with different code, if the 
% !!!!!!!
% !!!!!!!
% !!!!!!!
%set comprehension sympy developers 主动用python idioms重构了代码
% !!!!!!!
% !!!!!!!
% !!!!!!!


==> set_up_old.tex <==
%\subsection{Research Question}
%https://discuss.python.org/t/hello-where-is-the-source-code-of-list-comprehension-of-python/15312/2
\subsection{Data Collection}\label{data}
Having correct, complete and representative code pairs of non-idiomatic code and idiomatic code for each Python idiom is fundamental for evaluating the performance change of idiomatic refactorings. 
\subsubsection{Laboratory dataset} \textbf{Construction process}: Developers usually write simple code fragments to compare performance change because such code is easy to understand and set up for program execution. However, since manually constructing a large-scale systematic code pairs of non-idiomatic code and idiomatic code is time-consuming and laborious, there is currently no a laboratory benchmark to help developers understand the performance change of idiomatic refactorings. To construct the correct and complete code pairs of idiomatic refactorings, we first design four code dimensions to construct various non-idiomatic code. Then we execute a tool~\cite{zhang2022making} to automatically generate the corresponding idiomatic code. Finally, we manually validate all refactoring instances in the dataset.

\noindent\textbf{Symptoms of labratory dataset}: Previous studies~\cite{chen2020perfjit,Performance_Regression_huang,song2017performance} usually consider static syntax features but ignoring the dynamic features in code execution. In the paper, we design code features in four dimensions with static syntax features and dynamic code features as follows (shown in the Table~\ref{tab:codefeature_lab_dataset}):

\begin{enumerate}[fullwidth,itemindent=0em,leftmargin = 0pt]
	\item[(1)] Node kind: A code fragment with a Python idiom consists of different number of different abstract syntax nodes (ASTs). Any code difference~\cite{chen2020perfjit,Performance_Regression_huang,song2017performance} of code fragment of non-idiomatic code for each Python idiom may affect the performance of the idiomatic refactorings. Therefore, based on the AST node set of each Python idiom, we construct different valid node combinations, and change the number of nodes to analyze performance changes to explore the performance change. For example, the non-idiomatic code of list comprehension is to append elements to a list repeatedly. The code can only contains three AST nodes: For, If and If-Else nodes. Since the code should exist at least one For node, the num\_for does not contain 0. 
	
%https://stackoverflow.com/questions/12590058/performance-with-global-variables-vs-local
%https://wiki.python.org/moin/PythonSpeed/PerformanceTips
	\item[(2)] Context: For Python code, the performance of variables in the local namespace is different from of variables in the global namespace~\cite{python_perf_tips,python_programming}. To explore the impact of the context of variables on performance of the idiomatic refactoring, we wrap the idiomatic code in the function or not in the function as the distinction of the context of the variable.
	\item[(3)] Data instances: After extracting first two static language features, we construct dynamic code features. To construct microbenchmarks~\cite{costa2019s,jmh} to evaluate the performance, developers usually set different data size. Inspired by the practice,  for an iterator data, we will setting different number of elements. For enumerated data, we will enumerate different values. For example, for the non-idiomatic code of list comprehension, the list could append many elements, we set the range of the number of added elements is \texttt{size\_ele}. For another example, the non-idiomatic code of truth value test is to test whether a comparator belongs to \texttt{empty\_set}. 
	\item[(4)] State: A code fragment may exists multiple paths, each time code execute different paths, the code performance may change. Therefore, we construct different paths to explore the impacts of states on performance of idiomatic refactoring. For example, the non-idiomatic code of loop else has two paths: whether executes the break statement or not. 
\end{enumerate}

\begin{table*}[tbp]
\scriptsize
%\vspace{-0.2cm}
\caption{Code features of laboratory dataset}
  \label{tab:codefeature_lab_dataset}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l| c| c| c| c| c| c| c} 
\hline
Symptom&\begin{tabular}[c]{@{}l@{}}List/Set/Dict\\ Comprehension\end{tabular}&	\begin{tabular}[c]{@{}l@{}}chained\\ comparison\end{tabular}&	truth test&	Loop else&	\begin{tabular}[c]{@{}l@{}}assign-multi-tar\end{tabular}&	Star-in-func-call&	\begin{tabular}[c]{@{}l@{}}For-multi-tars\end{tabular}\\ \hline
Node & \begin{tabular}[c]{@{}l@{}} num\_For : 1-4\\
num\_If : 0-4\\
num\_If\_Else : 0-4\end{tabular} & \begin{tabular}[c]{@{}l@{}}num\_comop : 2-5\\ comop : \texttt{compop\_set}\end{tabular} &
\begin{tabular}[c]{@{}l@{}}test:  \texttt{test\_set} \\
comop : \texttt{eq\_set}\end{tabular}& \begin{tabular}[c]{@{}l@{}}\texttt{loop\_set} \\
\texttt{condition\_set}\end{tabular}&
\begin{tabular}[c]{@{}l@{}}num\_assign : 2-10\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
num\_Subscript : 1-30
\\
\texttt{is\_step}\\ 
\texttt{is\_lower}\\
\texttt{is\_upper}\\
\texttt{is\_total\_data}\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
num\_Subscript : 1-30\\
num\_target : 1-5\\
\end{tabular}\\ \hline
context&\texttt{Scope}&\texttt{Scope}&\texttt{Scope}&\texttt{Scope}&\texttt{Scope}&\texttt{Scope}&\texttt{Scope} \\\hline
\begin{tabular}[c]{@{}l@{}}Data\\ Instance\end{tabular}& \begin{tabular}[c]{@{}l@{}}\texttt{size\_ele} \end{tabular}&-& \begin{tabular}[c]{@{}l@{}}\texttt{empty\_set}\end{tabular}&\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}\end{tabular}& \begin{tabular}[c]{@{}l@{}}value : \texttt{data\_type}\\\ \ \texttt{is\_swap} \end{tabular}&\begin{tabular}[c]{@{}l@{}}index: \texttt{data\_type}  \end{tabular}&\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}\\\texttt{is\_total\_data}\end{tabular}\\\hline
State& -&\texttt{is\_true}& \texttt{is\_true}&\texttt{is\_break}& \begin{tabular}[c]{@{}l@{}}-\end{tabular}&-&-\\\hline
\end{tabular}
{\raggedright  num\_$n$ represents the number of the $n$ node; \texttt{test\_set}=\{If, While, Assert\}; \texttt{compop\_set}=\{Eq, NotEq, Lt, LtE, Gt, GtE, Is,  IsNot, In, NotIn\}; \texttt{eq\_set}=\{Eq, NotEq\}; \texttt{loop\_set} =\{For, While\}; \texttt{condition\_set} =\{If, If\_Else\}; \texttt{Scope}=\{in the function,  not in the function\}; \texttt{size\_ele}=\{$0$, $1$, $10$, $10^2$, ...,$10^6$\}; \texttt{empty\_set}=\{None, False, `', 0, 0.0, 0j, Decimal(0), Fraction(0, 1), (), [], \{\}, set(), range(0)\}; \texttt{is\_true}=\{0, 1\}, where 0, 1 represents the value of the code is False or True, respectively; \texttt{is\_break}=\{0, 1\}, where 0, 1 represents the code does not executes the break statement or executes the break statement, respectively; \texttt{is\_swap}=\{0, 1\}, where 0, 1 represents the code is not to swap variables or to swap variables; \texttt{is\_step}=\{0, 1\}, where 0, 1 represents the step of index list is not 1 or is 1, respectively; \texttt{is\_lower}=\{0, 1\}, where 0, 1 represents the index of the first element 
accessed is not 0 or is 0, respectively; \texttt{is\_upper}=\{0, 1\}, where 0, 1 represents the index of the last element 
accessed is not the last element of the list or is the last element of the list, respectively; \texttt{is\_total\_data}=\{0, 1\}, where 0, 1 represents the code fetches part of elements of the iterator or all elements of the iterator, respectively.\par}
\vspace{-0.3cm}
\end{table*}

%We consider the following four dimensions to automatically  programmers set upGenerally Python developers manually write simple code fragments (i.e., microbenchmarks) to compare whether performance improve. for Currently there is no beA code fragment with a Python idiom consists of different number of different abstract syntax nodes (ASTs). Any code changes of code fragment of non-idiomatic code for each Python idiom may affect the performance of the idiomatic refactorings. %Before the code runs, the tokenizer/lexer first convert a stream of characters into a stream of tokens. Then the parser parse the tokens into corresponding abstract syntax nodes (ASTs).
\subsubsection{In-the-field dataset} Although the laboratory data could provide a basic understanding of the impact of code features of the idiomatic refactoring on performance change, real-world project code is complex such as the use of classes and functions from library ecosystem. Similar to the construction of labratory dataset, we also want to contain dynamic features of real-world such as different data instances. Therefore, we use a publicly available test case dataset of idiomatic refactoring pairs~\cite{zhang2022making} from GitHub projects. For each idiomatic refactoring pair, it provides the configured projects to execute code before and after refactoring and a corresponding set of test cases with different data instances. To ensure each test case execute the idiomatic refactoring pair, we instrument print statements around the code to filter out test cases without printing the content we set up. Finally, we consider each data instance as a code refactoring pair.

Table~\ref{tab:statistics_dataset} summarizes the number of idiomatic refactoring in the laboratory dataset and the real-world dataset. 
\begin{table}[tbp]
\scriptsize
%\vspace{-0.2cm}
\caption{The statistics of laboratory data and real-world data}
  \label{tab:statistics_dataset}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l| c| c} 
 \hline
Idiom& laboratory dataset  &real-world dataset\\
 \hline

List Comprehension  & 1600 & 734   \\ 
\hline
Set Comprehension  & 1600 &  282  \\ 
\hline%1292
Dict Comprehension  & 1600   & 2194    \\ 
\hline

Chain Comparison   & 11968  & 2268 \\ 
\hline
Truth Value Test   & 140   & 40116\\ 
\hline
Loop Else    & 112 & 201 \\ 
\hline
Assign Multiple Targets  & 54  & 10583 \\ 
\hline
Star in Func Call  & 3784   & 170 \\ 
\hline
For Multiple Targets & 11760 & 334 \\
\hline
\end{tabular}
\vspace{-0.3cm}
\end{table}
% \begin{table}[tbp]
% \scriptsize
% %\vspace{-0.2cm}
% \caption{The statistics of laboratory data and real-world data}
%   \label{tab:statistics_dataset}
%   %\vspace{-0.4cm}
% \centering
% \begin{tabular}{l| c| c|c| c} 
%  \hline
% Idiom& laboratory dataset &RCIW &real-world dataset&RCIW\\
%  \hline

% List Comprehension  & 1600&0.04   & 734& 0.06    \\ 
% \hline
% Set Comprehension  & 1600&  0.04  & 1292 &    \\ 
% \hline
% Dict Comprehension  & 1600& 0.05   & 2194 & 0.03   \\ 
% \hline

% Chain Comparison   & 11968&0.05  & 2268&0.05 \\ 
% \hline
% Truth Value Test   & 140&0.05    & 40116& 0.05\\ 
% \hline
% Loop Else    & 112&  0.05 & 201& 0.04 \\ 
% \hline
% Assign Multiple Targets  & 54&0.04  & 10583&0.06 \\ 
% \hline
% Star in Func Call  & 3784&  0.04    & 170 & 0.06\\ 
% \hline
% For Multiple Targets & 11760&  0.07  & 334& 0.04 \\
% \hline
% \end{tabular}
% \vspace{-0.3cm}
% \end{table}
% study results
% Project Selection.
% Refactorings and Benchmarks Gathering.
% 2.1.3 Benchmarks Execution/Performance Data Collection. 
\subsection{Performance Measurement}\label{measurement}%Measurement/Evaluation
The measurement of execution time of non-idiomatic code and idiomatic code is far from trivial. There are a number of sources of non-determinism, such as Python Virtual Machine (VM) and the garbage collector~\cite{georges2007statistically}. To overcome the non-determinism, researchers repeatedly execute the code multiple times~\cite{georges2007statistically,chen2020perfjit,traini2021software,ding2020towards,stefan2017unit,laaber2018evaluation,laaber2019software,crape2020rigorous}. Since different VM invocations may result in different code execution time, and multiple executions of the code in a VM invocation may suffer from variability, we repeat each code 35 iterations on 50 invocations. Since first iterations (i.e., warm-up iterations) are subject noise caused by library loading, measurements are only collected in iterations that are subsequent to warm-up. 
We set the warm-up iterations to three which is enough to warmup the benchmark~\cite{traini2021software,pyperf}. 

To represent the performance change before and after idiomatic refactorings, we divide the total of execution time of non-idiomatic code by that of corresponding idiomatic code which indicates how much speedup idiomatic code compared with non-idiomatic code. The formular as follows: $$\rho=\frac{\sum_{i=1}^{n}\sum_{j=1}^{k}m_{i,j}^{before}}{\sum_{i=1}^{n}\sum_{j=1}^{k}m_{i,j}^{after}},$$
where $n$ is the number of VM invocations, $m$ is the number of measurements iterations, and $m_{i,j}$ is the execution time of the $k$th iteration in the $i$th invocation. 

To validate and show the reliability of performance measurement, we apply the approach of quantifying performance changes with effect size proposed by Kalibera et al.~\cite{kalibera2013rigorous,kalibera2020quantifying}. The main benefit of the Kalibera et al. technique is that it provides a clear and rigorous account of the performance change magnitude and of the uncertainty involved. For example, it can indicate that an idiomatic code is slower (or faster) than a non-idiomatic code by X \% ± Y\% with 95\% confidence. Similar to previous studies~\cite{kalibera2013rigorous,kalibera2020quantifying,traini2021software}, to build the confidence interval we use bootstrapping with hierarchical random re-sampling and replacement~\cite{davison1997bootstrap,ren2010nonparametric,traini2021software} on two levels~\cite{traini2021software,kalibera2020quantifying}: VM invocations and iterations. After the termination of 100 bootstrap iterations, we collect and sort a set of simulated realizations of the relative performance change $P = \{\rho_i \mid 1 \le i \le 100\}$ and estimate the lower limit $\rho_l$ and upper limit $\rho_u$ for a 95\% confidence interval. Finally, we compute the relative confidence interval width (RCIW) by the $\frac{\rho_u-\rho_l}{\rho}$ as the uncertainty of performance change of idiomatic refactoring. All the uncertainty of the performance change on the two datasets for each Python idiom is less than 0.05, which shows the reliability of performance measurement. % 这里提供一个时间的不确定说明下时间测量的稳定性
%We relied on steady-state performance~\cite{traini2021software,georges2007statistically}: we repeated a benchmark execution for several iterations and collected measurements only after a steady state had been reached. Indeed, first three iterations (often called warm-up iterations) are subject to noise due to performance variations in transient states, usually caused by library loading. Hence, in our experimental setup, measurements are only collected in iterations that are subsequent to warm-up, namely measurement iterations. Different VM invocations running multiple benchmark iterations may result in different steady-state performance data. For this reason, we also repeated benchmark iterations multiple times on different VM invocations.
%Reliably Detecting Performance Change. For example, it can indicate that a system version is slower (or faster) than another by X \% ± Y \% with 95% confidence. 

==> setup.tex <==
%\subsection{Research Question}
%https://discuss.python.org/t/hello-where-is-the-source-code-of-list-comprehension-of-python/15312/2
\subsection{Data Collection}\label{data}
Having correct, complete and representative code pairs of non-idiomatic code and idiomatic code for Python idioms is fundamental for evaluating the performance change of the idiomatic refactoring. 
\subsubsection{Laboratory dataset} \textbf{Construction process}: Developers usually write simple code fragments to compare performance change because such code is easy to set up for running experiment and understand the performance change. Since manually constructing a correct and large-scale code pairs of non-idiomatic code and idiomatic code is time-consuming and laborious, there is currently no a laboratory dataset. To construct the correct and complete code pairs of idiomatic refactorings, we first design four code dimensions to construct various non-idiomatic code. Then we execute a tool~\cite{zhang2022making} to automatically generate the corresponding idiomatic code. Finally, we manually validate all refactoring instances in the dataset.

\noindent\textbf{Symptoms of labratory dataset}: Previous studies~\cite{chen2020perfjit,Performance_Regression_huang,song2017performance} on performance issues find that source code changes (e.g., the number of loop and condition) may related to performance. They usually consider the programming language syntax but ignore the dynamic features (e.g., different data size and execution paths). In the paper, we design code features in four dimensions with language syntax features and dynamic code features as follows (shown in the Table~\ref{tab:codefeature_lab_dataset}):

\begin{table*}[tbp]
\scriptsize
%\vspace{-0.2cm}
\caption{code features of laboratory dataset}
  \label{tab:codefeature_lab_dataset}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l| c| c| c| c| c| c| c} 
\hline
Symptom&\begin{tabular}[c]{@{}l@{}}list/set/dict\\ comprehension\end{tabular}&	\begin{tabular}[c]{@{}l@{}}chained\\ comparison\end{tabular}&	truth test&	loop else&	\begin{tabular}[c]{@{}l@{}}assign-multi-tar\end{tabular}&	star-in-func-call&	\begin{tabular}[c]{@{}l@{}}For-multi-tars\end{tabular}\\ \hline
Node & \begin{tabular}[c]{@{}l@{}} num\_For : 1-4\\
num\_If : 0-4\\
num\_If\_Else : 0-4\end{tabular} & \begin{tabular}[c]{@{}l@{}}num\_comop : 2-5\\ comop : \texttt{compop\_set}\end{tabular} &
\begin{tabular}[c]{@{}l@{}}test:  \texttt{test\_set} \\
comop : \texttt{eq\_set}\\value : \texttt{empty\_set}\end{tabular}& \begin{tabular}[c]{@{}l@{}}\texttt{loop\_set} \\
\texttt{condition\_set}\end{tabular}&
\begin{tabular}[c]{@{}l@{}}num\_assign : 2-30\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
num\_Subscript : 1-30
\\
\texttt{has\_step}\\ 
\texttt{has\_lower}\\
\texttt{has\_upper}\\
\texttt{has\_Subscript}\end{tabular}&
\begin{tabular}[c]{@{}l@{}}
num\_Subscript : 1-30\\
num\_target : 1-5\\
\texttt{has\_Starred}\\
\end{tabular}\\ \hline
Context&\texttt{Scope}&\texttt{Scope}&\texttt{Scope}&\texttt{Scope}&\texttt{Scope}&\texttt{Scope}&\texttt{Scope} \\\hline
\begin{tabular}[c]{@{}l@{}}Data\end{tabular}& \begin{tabular}[c]{@{}l@{}}\texttt{size\_ele} \end{tabular}&-& \begin{tabular}[c]{@{}l@{}}-\end{tabular}&\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}\end{tabular}& \begin{tabular}[c]{@{}l@{}}value : \texttt{is\_const}\\ \texttt{is\_swap} \end{tabular}&\begin{tabular}[c]{@{}l@{}}index: \texttt{is\_const} \end{tabular}&\begin{tabular}[c]{@{}l@{}}\texttt{size\_ele}\end{tabular}\\\hline
State& -&\texttt{is\_true}& \texttt{is\_true}&\texttt{is\_break}& \begin{tabular}[c]{@{}l@{}}-\end{tabular}&-&-\\\hline
\end{tabular}
% {\raggedright  num\_$n$ represents the number of the $n$ node; \texttt{test\_set}=\{If, While, Assert\}; \texttt{compop\_set}=\{Eq, NotEq, Lt, LtE, Gt, GtE, Is,  IsNot, In, NotIn\}; \texttt{eq\_set}=\{Eq, NotEq\}; \texttt{loop\_set} =\{For, While\}; \texttt{condition\_set} =\{If, If\_Else\}; \texttt{has\_step}=\{0, 1\}, where 0, 1 represents the slice of the idiomatic code does not have the step node or has, respectively; \texttt{has\_lower}=\{0, 1\}, where 0, 1 represents the slice of the idiomatic code does not have the lower node or has, respectively; \texttt{has\_upper}=\{0, 1\}, where 0, 1 represents the slice of the idiomatic code does not have the upper node or has, respectively; \texttt{has\_Subscript}=\{0, 1\}, where 0, 1 represents the idiomatic code does not have the Subscript node or has, respectively; \texttt{has\_Starred}=\{0, 1\}, where 0, 1 represents the idiomatic code does not have the Starred node or has, respectively; \texttt{Scope}=\{in the function,  not in the function\}; \texttt{size\_ele}=\{$0$, $1$, $10$, $10^2$, ...,$10^6$\}; \texttt{empty\_set}=\{None, False, `', 0, 0.0, 0j, Decimal(0), Fraction(0, 1), (), [], \{\}, set(), range(0)\}; \texttt{is\_swap}=\{0, 1\}, where 0, 1 represents the code is not to swap variables or to swap variables, respectively; \texttt{is\_true}=\{0, 1\}, where 0, 1 represents the value of the code is False or True, respectively; \texttt{is\_break}=\{0, 1\}, where 0, 1 represents the code does not executes the break statement or executes the break statement, respectively.\par}
\vspace{-0.3cm}
\end{table*}

% \begin{table*}[tbp]
% \scriptsize
% %\vspace{-0.2cm}
% \caption{code features of laboratory dataset}
%   \label{tab:codefeature_lab_dataset}
%   %\vspace{-0.4cm}
% \centering
% \begin{tabular}{l| c| c| c| c| c| c| c} 
% \hline
% Symptom&\begin{tabular}[c]{@{}l@{}}list/set/dict\\ comprehension\end{tabular}&	\begin{tabular}[c]{@{}l@{}}chained\\ comparison\end{tabular}&	truth test&	loop else&	\begin{tabular}[c]{@{}l@{}}assign-multi-tar\end{tabular}&	star-in-func-call&	\begin{tabular}[c]{@{}l@{}}For-multi-tars\end{tabular}\\ \hline
% Node & \begin{tabular}[c]{@{}l@{}} numFor : 1-4\\
% numIf : 0-4\\
% numIfElse : 0-4\end{tabular} & \begin{tabular}[c]{@{}l@{}}numComop : 2-5\\ comop : \textsf{CompopSet}\end{tabular} &
% \begin{tabular}[c]{@{}l@{}}test:  \textsf{TestSet} \\
% comop : \textsf{EqSet}\\value : \textsf{EmptySet}\end{tabular}& \begin{tabular}[c]{@{}l@{}}\textsf{Loop\_Set} \\
% \textsf{ConditionSet}\end{tabular}&
% \begin{tabular}[c]{@{}l@{}}numAssign : 2-30\end{tabular}&
% \begin{tabular}[c]{@{}l@{}}
% numSubscript : 1-30
% \\
% \texttt{hasStep}\\ 
% \texttt{hasLower}\\
% \texttt{hasUpper}\\
% \texttt{hasSubscript}\end{tabular}&
% \begin{tabular}[c]{@{}l@{}}
% numSubscript : 1-30\\
% numTarget : 1-5\\
% \texttt{hasStarred}\\
% \end{tabular}\\ \hline
% Context&\texttt{scope}&\texttt{scope}&\texttt{scope}&\texttt{scope}&\texttt{scope}&\texttt{scope}&\texttt{scope} \\\hline
% \begin{tabular}[c]{@{}l@{}}Data\end{tabular}& \begin{tabular}[c]{@{}l@{}}\texttt{size} \end{tabular}&-& \begin{tabular}[c]{@{}l@{}}-\end{tabular}&\begin{tabular}[c]{@{}l@{}}\texttt{size}\end{tabular}& \begin{tabular}[c]{@{}l@{}}value : \texttt{isConst}\\ \texttt{isSwap} \end{tabular}&\begin{tabular}[c]{@{}l@{}}index: \texttt{isConst} \end{tabular}&\begin{tabular}[c]{@{}l@{}}\texttt{size}\end{tabular}\\\hline
% State& -&\texttt{isTrue}& \texttt{isTrue}&\texttt{isBreak}& \begin{tabular}[c]{@{}l@{}}-\end{tabular}&-&-\\\hline
% \end{tabular}
% % {\raggedright  num\_$n$ represents the number of the $n$ node; \texttt{test\_set}=\{If, While, Assert\}; \texttt{compop\_set}=\{Eq, NotEq, Lt, LtE, Gt, GtE, Is,  IsNot, In, NotIn\}; \texttt{eq\_set}=\{Eq, NotEq\}; \texttt{loop\_set} =\{For, While\}; \texttt{condition\_set} =\{If, If\_Else\}; \texttt{has\_step}=\{0, 1\}, where 0, 1 represents the slice of the idiomatic code does not have the step node or has, respectively; \texttt{has\_lower}=\{0, 1\}, where 0, 1 represents the slice of the idiomatic code does not have the lower node or has, respectively; \texttt{has\_upper}=\{0, 1\}, where 0, 1 represents the slice of the idiomatic code does not have the upper node or has, respectively; \texttt{has\_Subscript}=\{0, 1\}, where 0, 1 represents the idiomatic code does not have the Subscript node or has, respectively; \texttt{has\_Starred}=\{0, 1\}, where 0, 1 represents the idiomatic code does not have the Starred node or has, respectively; \texttt{Scope}=\{in the function,  not in the function\}; \texttt{size\_ele}=\{$0$, $1$, $10$, $10^2$, ...,$10^6$\}; \texttt{empty\_set}=\{None, False, `', 0, 0.0, 0j, Decimal(0), Fraction(0, 1), (), [], \{\}, set(), range(0)\}; \texttt{is\_swap}=\{0, 1\}, where 0, 1 represents the code is not to swap variables or to swap variables, respectively; \texttt{is\_true}=\{0, 1\}, where 0, 1 represents the value of the code is False or True, respectively; \texttt{is\_break}=\{0, 1\}, where 0, 1 represents the code does not executes the break statement or executes the break statement, respectively.\par}
% \vspace{-0.3cm}
% \end{table*}

\begin{enumerate}[fullwidth,itemindent=0em,leftmargin = 0pt]
	\item[(1)] \textbf{Abstract Syntax Tree (AST) Node:} A code fragment with a Python idiom consists of different abstract syntax nodes (ASTs). Previous studies~\cite{chen2020perfjit,Performance_Regression_huang,song2017performance} on performance issues states that changes on the basic code syntax (e.g., break, loop and condition) may introduce performance regressions. To ensure the completeness of the study, we consider combinations of 
many syntax nodes as much as possible. Based on the set of AST node of non-idiomatic code and idiomatic code, we construct various valid node combinations, and change the number of nodes to analyze the performance change of Python idioms. The feature is shown in the first row of Table~\ref{tab:codefeature_lab_dataset}. The ``num\_*'' represents the number of AST nodes, the ``\texsf{*\_set}'' represents the set of AST nodes of, the ``\texttt{has\_*}'' represents whether Python idioms have the AST node or not where 0 represents the code has the node, 1 represents the code does not have. The details of nine Python idioms as follows:

\noindent $\bullet$ The comprehension idioms are to append elements to an iterable. They must contain For node, and may have If node with else or If node without else. We set up the range of number of For node (num\_For) from 1 to 4, and the range of number of If node with else (num\_If) and If node without else (num\_If\_Else) from 0 to 5. For example, for the list-comprehension code: ``\textsf{l = [e\_0 if e\_0 \% 2 else e\_0 for e\_0 in x\_0 if e\_0 // 1]}'', it has one For node, one If node without else and one If node with else.

\noindent $\bullet$ The chain-comparison is to chain multiple comparison operations, so it has two compare operators at least. We set up the range of num\_compop from two to five. And the compare operator only could from the \texttt{comop\_set}: \{Eq, NotEq, Lt, LtE, Gt, GtE, Is,  IsNot, In, NotIn\}. For example, for the code: ``\textsf{n >= m > l > k}'', it has three compare comparators and their comparators are ``\textsf{>=, >, >}''.

\noindent $\bullet$ The truth-value-test is to test whether an object is equal/not equal to a value, where called test node. The parent node of test node belongs to \texttt{test\_set}: \{For, While, Assert\}, the compare operator belongs to \texttt{eq\_set}\{Eq, NotEq\} (), and the value belongs to \texttt{empty\_set}: \{None, False, `', 0, 0.0, 0j, Decimal(0), Fraction(0, 1), (), [], \{\}, set(), range(0)\}.
	
\noindent $\bullet$ The loop-else is to determine whether execute the else clause after the iterator is exhausted. It contains a For/While node (\texttt{loop\_set}) and an if node without else or an if node (\texttt{condition\_set}) after the loop block.

\noindent $\bullet$ The assign-multiple-targets is to assign multiple values in one assignment statement. We set up the range of the number of assign node from 2$\sim$30.

\noindent $\bullet$ The star-in-func-call is to unpack an iterable to the positional arguments in a function call. The non-idiomatic code consists of Subscript nodes (e.g., e\_list[1]). We set up the range of number of Subscript node (num\_Subscript) from 1 to 30. The corresponding idiomatic code may or may not have the Subscript node \texttt{has\_Subscript}. If it has the Subscript node, it may or may not have the step, lower and upper nodes, where are denoted by \texttt{has\_step}, \texttt{has\_lower} and \texttt{has\_upper}. For example, for the non-idiomatic code: ``\textsf{e\_list[1], e\_list[2], e\_list[3]}'', the num\_Subscript is 3. The corresponding idiomatic code is ``\textsf{*e\_list[1:4]}'', where the \texttt{has\_step}, \texttt{has\_lower}, and \texttt{has\_upper} are 0, 1, 0.

\noindent $\bullet$  The for-multiple-targets is to unpack operators inside an iterable as a flattening operator. It has a For node and Subscript nodes in the body of the For node to use each item. We set up the range of number of Subscript (num\_Subscript) node from 1 to 30. The corresponding idiomatic code may have many target nodes, so we set the range of number target node is from 1 to 5. If the body of For node only accesses part of elements, the idiomatic code may have or not have the a Starred node (\texttt{has\_Starred}). For example, for the non-idiomatic code: ``\textsf{for e in input\_seq: e[0]}'',  the num\_Subscript is 1. If each element of ``\textsf{input\_seq}'' has more than two elements, the idiomatic code fragment is ``\textsf{for (e\_0, *e\_len) in input\_seq: e\_0}'' where the ``\textsf{*e\_len} represents remaining unused items. 

%https://stackoverflow.com/questions/12590058/performance-with-global-variables-vs-local
%https://wiki.python.org/moin/PythonSpeed/PerformanceTips
	\item[(2)] \textbf{Context:} For Python code, the performance of variables in the local namespace is different from of variables in the global namespace~\cite{python_perf_tips,python_programming}. To explore the impact of the context of variables on performance of the idiomatic refactoring, we wrap the idiomatic code in the function or not in the function as the distinction of context. We denote the context by \texttt{scope} in Table~\ref{tab:codefeature_lab_dataset}, where equals to \{local scope, global scope\}.
	\item[(3)] \textbf{Data}: After extracting first two static language features, we construct dynamic code features. When constructing microbenchmarks~\cite{costa2019s,jmh} to evaluate the performance, developers usually set different data size. Inspired by the practice, we set \texttt{size\_ele}=\{$0$, $1$, $10$, $10^2$, ...,$10^6$\} for an iterable. For list/set/dict comprehension, it represents the number of added elements of the iterable. For the loop-else and for-multiple-targets, it represents the number of iterations. The value of assign-multiple-targets maybe a temporary variable or not, which represents whether the funcionality is to swap variables or not (\texttt{is\_swap}). Besides, many researchers states that the constants maybe faster than variables~\cite{const_perf,ismail2018quantitative,barany2014python,rodriguez2016automatic}, since the value of assign-multiple-targets and the index of Subscript of star-in-func-call may be a constant or not, we set \texttt{is\_const} for the two Python idioms.
	%For the star-in-func-call, the index of Subscript also maybe a constant or not a constant (\texttt{is\_const}). And the range of the number of elements of the iterable is from 2 to 30. 
% 	and star-in-func-call, the  For example, for the non-idiomatic code of list comprehension, the list could append many elements, we set the range of the number of added elements is \texttt{size\_ele}. For another example, the non-idiomatic code of truth value test is to test whether a comparator belongs to \texttt{empty\_set}. 
	\item[(4)] \textbf{State}: A code fragment may exist multiple paths, different execution paths may lead to performance change. Therefore, we execute different paths to explore the impact of states on performance of idiomatic refactoring. For the loop-else, it has two paths: whether executes the break statement or not (\texttt{is\_break}). For the chain-comparison, when a compare node is false, it will not test the next compare node and execute the next statement. For the truth-value-test, the true or false of the value jump to different paths. Therefore, we set value of the Python idioms to \texttt{is\_true}, where equals to \{0, 1\}.
\end{enumerate}



%We consider the following four dimensions to automatically  programmers set upGenerally Python developers manually write simple code fragments (i.e., microbenchmarks) to compare whether performance improve. for Currently there is no beA code fragment with a Python idiom consists of different number of different abstract syntax nodes (ASTs). Any code changes of code fragment of non-idiomatic code for each Python idiom may affect the performance of the idiomatic refactorings. %Before the code runs, the tokenizer/lexer first convert a stream of characters into a stream of tokens. Then the parser parse the tokens into corresponding abstract syntax nodes (ASTs).
\subsubsection{In-the-field dataset} Although the laboratory data could provide a basic understanding of the impact of code features of the idiomatic refactoring on performance change, real-world project code is complex such as the use of classes and functions from Python library ecosystem (e.g., numpy and pandas). Similar to the construction of laboratory dataset, we also want to contain dynamic features of real-world such as different data instances. Therefore, we use a publicly available test case dataset of idiomatic refactoring pairs~\cite{zhang2022making} from 270 successfully configured GitHub projects. For each idiomatic refactoring pair, it provides the configured projects to execute code before and after refactoring and a corresponding set of test cases with different data instances. To ensure each test case execute the idiomatic refactoring pair, we instrument print statements around the code to filter out test cases without printing the content we set up. Finally, we consider each data instance as a code refactoring pair. The symptoms of real-world dataset as follows:

\noindent (1) \textbf{Node}: For the Node symptoms of real-world dataset, the ``\texttt{*\_set}'' and ``\texttt{has\_*}'' are the same as that of laboratory dataset. The ``num\_*'' is different from that of laboratory dataset. For the list-comprehension, the range of num\_For, num\_If, num\_If\_Else are 1$\sim$3, 0$\sim$2 and 0$\sim$2, respectively. For the set-comprehension, the range of num\_For, num\_If, num\_If\_Else is 1$\sim$2, 0$\sim$1 and 0. For the dict-comprehension, the range of num\_For, num\_If, num\_If\_Else is 1$\sim$3, 0$\sim$1 and 0$\sim$1. For the chained comparison, the num\_compop is 2. For the assign-multiple-targets, the range of num\_assign is 2$\sim$11. For the star-in-func-call, the range of num\_Subscript is 2$\sim$4. For the for-multiple-targets, the range of num\_Subscript and num\_target are 1$\sim$6 and 1$\sim$3, respectively.

\noindent (2) \textbf{Context}: Since the real-world datasets come from the test cases, all codes are in the local scope.

\noindent (3) \textbf{Data}: The range of \texttt{size\_ele} of real-world dataset is different from that of laboratory dataset. For the list-comprehension, set-comprehension, dict-comprehension, loop-else and for-multiple-targets, their ranges of \texttt{size\_ele} are 0$\sim$11,766, 0$\sim$44, 0$\sim$1,000, 0$\sim$50 and 0$\sim$583, respectively. For the assign-multi-targets, the \texttt{is\_swap} is 0.

\noindent (4) \textbf{State}: The state of real-world dataset is the same as that of laboratory dataset.


Table~\ref{tab:statistics_dataset} summarizes the number of idiomatic refactoring in the laboratory dataset and the real-world dataset. On the laboratory dataset, for the list/set/dict-comprehension, the 1600 is computed by multiplying 4 num\_For, 5 num\_If, 5 num\_If\_Else, 2 values of \texttt{scope} and 8 values of \texttt{size\_ele}. For the chained comparison, the 11968 is computed by multiplying 2992 combinations of 2-5 length subsequences of elements from the \texttt{compop\_set}, 2 values of \texttt{scope} and 2 values of \texttt{is\_true}. For the assign-multiple-targets, when the values are constants, the \texttt{is\_swap} can only be 0, so there are only 174 codes instead of 232 codes.
\begin{table}[tbp]
\scriptsize
\vspace{-0.2cm}
\caption{The statistics of laboratory data and real-world data}
  \label{tab:statistics_dataset}
  %\vspace{-0.4cm}
\centering
\begin{tabular}{l| c| c} 
 \hline
Idiom& laboratory dataset  &real-world dataset\\
 \hline

List Comprehension  & 1600 & 734   \\ 
\hline
Set Comprehension  & 1600 &  282  \\ 
\hline%1292
Dict Comprehension  & 1600   & 2194    \\ 
\hline

Chain Comparison   & 11968  & 2268 \\ 
\hline
Truth Value Test   &336   & 40116\\ 
\hline
Loop Else    & 128 & 201 \\ 
\hline
Assign Multiple Targets  & 174  & 10583 \\ 
\hline
Star in Func Call  & 1920   & 170 \\ 
\hline
For Multiple Targets & 4800 & 334 \\
\hline
\end{tabular}
\vspace{-0.5cm}
\end{table}
% \begin{table}[tbp]
% \scriptsize
% %\vspace{-0.2cm}
% \caption{The statistics of laboratory data and real-world data}
%   \label{tab:statistics_dataset}
%   %\vspace{-0.4cm}
% \centering
% \begin{tabular}{l| c| c|c| c} 
%  \hline
% Idiom& laboratory dataset &RCIW &real-world dataset&RCIW\\
%  \hline

% List Comprehension  & 1600&0.04   & 734& 0.06    \\ 
% \hline
% Set Comprehension  & 1600&  0.04  & 1292 &    \\ 
% \hline
% Dict Comprehension  & 1600& 0.05   & 2194 & 0.03   \\ 
% \hline

% Chain Comparison   & 11968&0.05  & 2268&0.05 \\ 
% \hline
% Truth Value Test   & 140&0.05    & 40116& 0.05\\ 
% \hline
% Loop Else    & 112&  0.05 & 201& 0.04 \\ 
% \hline
% Assign Multiple Targets  & 54&0.04  & 10583&0.06 \\ 
% \hline
% Star in Func Call  & 3784&  0.04    & 170 & 0.06\\ 
% \hline
% For Multiple Targets & 11760&  0.07  & 334& 0.04 \\
% \hline
% \end{tabular}
% \vspace{-0.3cm}
% \end{table}
% study results
% Project Selection.
% Refactorings and Benchmarks Gathering.
% 2.1.3 Benchmarks Execution/Performance Data Collection. 
\subsection{Performance Measurement}\label{measurement}%Measurement/Evaluation
The measurement of execution time of non-idiomatic code and idiomatic code is far from trivial. There are a number of sources of non-determinism, such as Python Virtual Machine (VM) and the garbage collector~\cite{georges2007statistically}. To overcome the non-determinism, researchers repeatedly execute the code multiple times~\cite{georges2007statistically,chen2020perfjit,traini2021software,ding2020towards,stefan2017unit,laaber2018evaluation,laaber2019software,crape2020rigorous}. Since different VM invocations may result in different code execution time, and multiple executions of the code in a VM invocation may suffer from variability, we repeat each code 35 iterations on 50 invocations as done in previous studies~\cite{georges2007statistically,traini2021software,crape2020rigorous,laaber2019software}. Since first iterations (i.e., warm-up iterations) are subject noise caused by library loading, measurements are only collected in iterations that are subsequent to warm-up. 
We set the warm-up iterations to three which is enough to warmup the benchmark~\cite{traini2021software,pyperf}. 

% Kalibera et al.~\cite{kalibera2013rigorous,kalibera2020quantifying} shows that 65 papers of 90 papers quantify a performance change using a ratio of execution times. Similar to them, to represent the performance change before and after idiomatic refactorings, we divide the total of execution time of non-idiomatic code by that of corresponding idiomatic code to indicate how much speedup idiomatic code compared with non-idiomatic code. The formula as follows: $$\rho=\frac{\sum_{i=1}^{n}\sum_{j=1}^{k}m_{i,j}^{before}}{\sum_{i=1}^{n}\sum_{j=1}^{k}m_{i,j}^{after}},$$
% where $n$ is the number of VM invocations, $m$ is the number of measurements iterations, and $m_{i,j}$ is the execution time of the $k$th iteration in the $i$th invocation. 

%https://users.elis.ugent.be/~leeckhou/papers/iiswc20.pdf %PyPy JIT compiler outperforms the CPython interpreter by 1.76× for steady-state while be- ing 2% slower for start-up
%https://kar.kent.ac.uk/33611/45/p63-kaliber.pdf
%https://switowski.com/blog/writing-faster-python-intro
%https://en.wikipedia.org/wiki/Speedup
%https://en.wikipedia.org/wiki/Percentage#Percentage_increase_and_decrease
%https://math.stackexchange.com/questions/1227389/what-is-the-difference-between-faster-by-factor-and-faster-by-percent
%https://kar.kent.ac.uk/33611/45/p63-kaliber.pdf 65 papers Measuring Speedup
%https://math.stackexchange.com/questions/186730/calculate-x-slower-faster

% The more execution time means the slower the speed, if the performance change is larger than 1, the idiomatic code has a $\rho$X speedup (i.e., the idiomatic code is  faster than non-idiomatic code by $(\rho-1)$). If the performance change is less than 1, the idiomatic code has a $\frac{1}{\rho}$X slowdown (i.e., the idiomatic code is $\frac{1}{\rho}$ times as slow as the non-idiomatic code).  Otherwise, the performance of idiomatic code is the same as of non-idiomatic code. For example, if the time of idiomatic code is 2s and the time of non-idiomatic code is 1s, the idiomatic has a 2X speedup or the idiomatic code is 100\% faster than non-idiomatic code.

Kalibera et al.~\cite{kalibera2013rigorous,kalibera2020quantifying} shows that 65 papers of 90 papers quantify a performance change using a ratio of execution times. Similar to them, to represent the performance change before and after idiomatic refactorings, we divide the total of execution time of non-idiomatic code by that of corresponding idiomatic code to indicate how much speedup idiomatic code compared with non-idiomatic code. The formula as follows:
$$\rho=\frac{\sum_{i=1}^{n}\sum_{j=1}^{k}m_{i,j}^{after}}{\sum_{i=1}^{n}\sum_{j=1}^{k}m_{i,j}^{before}},$$
where $n$ is the number of VM invocations, $m$ is the number of measurements iterations, and $m_{i,j}$ is the execution time of the $k$th iteration in the $i$th invocation. 

The more execution time means the slower the speed, if the performance change is larger than 1, the idiomatic code has a $\rho$X slowdown (i.e., the idiomatic code is $\rho-1$ times slower than non-idiomatic code). If the performance change is less than 1, the idiomatic code has a $\frac{1}{\rho}$X speedup (i.e., the idiomatic code is $1-\rho$ times faster than non-idiomatic code). Otherwise, the performance of idiomatic code is the same as of non-idiomatic code. For example, if the time of non-idiomatic code is 2s and the time of idiomatic code is 1s, the idiomatic code has a 2X speedup or the idiomatic code is 50\% faster than non-idiomatic code.

To validate and show the reliability of performance measurement, we apply the approach of quantifying performance changes with effect size proposed by Kalibera et al.~\cite{kalibera2013rigorous,kalibera2020quantifying}. The main benefit of the Kalibera et al. technique is that it provides a clear and rigorous account of the performance change magnitude and of the uncertainty involved. For example, it can indicate that an idiomatic code is slower (or faster) than a non-idiomatic code by X \% ± Y\% with 95\% confidence. Similar to previous studies~\cite{kalibera2013rigorous,kalibera2020quantifying,traini2021software}, to build the confidence interval we use bootstrapping with hierarchical random re-sampling and replacement~\cite{davison1997bootstrap,ren2010nonparametric,traini2021software} on two levels~\cite{traini2021software,kalibera2020quantifying}: VM invocations and iterations. After the termination of 100 bootstrap iterations, we collect and sort a set of simulated realizations of the relative performance change $P = \{\rho_i \mid 1 \le i \le 100\}$ and estimate the lower limit $\rho_l$ and upper limit $\rho_u$ for a 95\% confidence interval. Finally, we compute the relative confidence interval width (RCIW) by the $\frac{\rho_u-\rho_l}{\rho}$ as the uncertainty of performance change of idiomatic refactoring. All the uncertainty of the performance change on the two datasets for each Python idiom is less than 0.05, which shows the reliability of performance measurement. 

% If the performance change is larger than 1, the performance improves (i.e., performance improvement), we say that the performance improvement of idiomatic refactoring is $\rho$. If the performance change is less than 1, the performance decreases (i.e., performance regression), we say that the performance regression of idiomatic refactoring is $\frac{1}{\rho}$. Otherwise, the performance basically is unchanged (i.e., performance unchanged). For each Python idiom, we analyze what kind of performance impact on the two datasets, and compare how well the performance change of the laboratory dataset align with the performance change of real-world dataset from the upper bond, lower bond and the range of performance change.% 这里提供一个时间的不确定说明下时间测量的稳定性
%We relied on steady-state performance~\cite{traini2021software,georges2007statistically}: we repeated a benchmark execution for several iterations and collected measurements only after a steady state had been reached. Indeed, first three iterations (often called warm-up iterations) are subject to noise due to performance variations in transient states, usually caused by library loading. Hence, in our experimental setup, measurements are only collected in iterations that are subsequent to warm-up, namely measurement iterations. Different VM invocations running multiple benchmark iterations may result in different steady-state performance data. For this reason, we also repeated benchmark iterations multiple times on different VM invocations.
%Reliably Detecting Performance Change. For example, it can indicate that a system version is slower (or faster) than another by X \% ± Y \% with 95% confidence. 
